Towards Robust Hyperspectral Unmixing: Mixed Noise Modeling and Image-Domain Regularization

Hyperspectral (HS) unmixing is the process of decomposing an HS image into material-specific spectra (endmembers) and their spatial distributions (abundance maps). Existing unmixing methods have two limitations with respect to noise robustness. First, if the input HS image is highly noisy, even if the balance between sparse and piecewise-smooth regularizations for abundance maps is carefully adjusted, noise may remain in the estimated abundance maps or undesirable artifacts may appear. Second, existing methods do not explicitly account for the effects of stripe noise, which is common in HS measurements, in their formulations, resulting in significant degradation of unmixing performance when such noise is present in the input HS image. To overcome these limitations, we propose a new robust hyperspectral unmixing method based on constrained convex optimization. Our method employs, in addition to the two regularizations for the abundance maps, regularizations for the HS image reconstructed by mixing the estimated abundance maps and endmembers. This strategy makes the unmixing process much more robust in highly-noisy scenarios, under the assumption that the abundance maps used to reconstruct the HS image with desirable spatio-spectral structure are also expected to have desirable properties. Furthermore, our method is designed to accommodate a wider variety of noise including stripe noise. To solve the formulated optimization problem, we develop an efficient algorithm based on a preconditioned primal-dual splitting method, which can automatically determine appropriate stepsizes based on the problem structure. Experiments on synthetic and real HS images demonstrate the advantages of our method over existing methods.

==> fig_tex/fig_Org_HSimages_colored.tex <==
\begin{figure}[t]
	\centering
	\begin{minipage}{0.24\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/original/0.05_0.1_0/Orig_HSI-eps-converted-to.pdf}
		}
		\centerline{(a): \textit{Synth 1}}
	\end{minipage}
	\begin{minipage}{0.05\hsize}
		\centerline{~}
	\end{minipage}
	\begin{minipage}{0.24\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/synth/original/0.05_0.05_0.05/Orig_HSI-eps-converted-to.pdf}}
		\centerline{(b): \textit{Synth 2}}
	\end{minipage}
	\begin{minipage}{0.05\hsize}
		\centerline{~}
	\end{minipage}
	\begin{minipage}{0.24\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre_200_noniid/original/Noniid_0.05_0.05/Orig_HSI-eps-converted-to.pdf}
		}
		\centerline{\textcolor{blue}{(c): \textit{Synth 3}}}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}{0.24\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/real/original/0.1_0_0/Orig_HSI-eps-converted-to.pdf}}
		\centerline{(d): \textit{Jasper Ridge}}
	\end{minipage}
	\begin{minipage}{0.05\hsize}
		\centerline{~}
	\end{minipage}
	\begin{minipage}{0.24\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/real_samson/original/0.1_0.05_0.05/Orig_HSI-eps-converted-to.pdf}}
		\centerline{(e): \textit{Samson}}
	\end{minipage}
	\begin{minipage}{0.05\hsize}
		\centerline{~}
	\end{minipage}
	\begin{minipage}{0.24\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_urban_noniid/original/Noniid_0.05_0.05/Orig_HSI-eps-converted-to.pdf}
		}
		\centerline{\textcolor{blue}{(f): \textit{Urban}}}
	\end{minipage}
	
	\caption{Original HS images.}
	\label{fig:Org_HSimages}
\end{figure}

%\vspace{-10mm}

==> fig_tex/fig_SAD_colord.tex <==
%\begin{figure*}[t]
%	\centering
%	\begin{minipage}{0.24\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/SAD/synth_dataset_Legendre.eps}}
	%		\centerline{(a): \textit{Synth 1}}
	%	\end{minipage}
%	\begin{minipage}{0.10\hsize}
	%	\centerline{~}
	%	\end{minipage}
%	\begin{minipage}{0.24\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/SAD/synth_dataset_new.eps}}
	%		\centerline{(b): \textit{Synth 2}}
	%	\end{minipage}
%	\begin{minipage}{0.10\hsize}
	%	\centerline{~}
	%	\end{minipage}
%	\begin{minipage}{0.24\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/SAD/synth_dataset_200_240.eps}}
	%		\centerline{(c): \textit{Synth 3}}
	%	\end{minipage}
%	
%	\vspace{1mm}
%	
%	\begin{minipage}{0.24\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/SAD/jasper_dataset_20230410.eps}}
	%		\centerline{(d): \textit{Jasper Ridge}}
	%	\end{minipage}
%	\begin{minipage}{0.10\hsize}
	%	\centerline{~}
	%	\end{minipage}
%	\begin{minipage}{0.24\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/SAD/samson_dataset.eps}}
	%		\centerline{(e): \textit{Samson}}
	%	\end{minipage}
%	\begin{minipage}{0.10\hsize}
	%	\centerline{~}
	%	\end{minipage}
%	\begin{minipage}{0.24\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/SAD/urban_dataset.eps}}
	%		\centerline{(f): \textit{Urban}}
	%	\end{minipage}
%	
%	\caption{The distributions of spectral angle distances between the spectra of endmembers present in HS images and the spectra of the other endmembers. Vertical axes indicate the spectral angle ditances. Horizontal axes indicate the indices of the endmembers present in the HS images. The SAD values tends to be the same for all data sets.}
%	\label{fig:SAD}
%\end{figure*}

\begin{figure}[t]
		\color{blue}
	\centering
	\begin{minipage}{0.48\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/SAD/synth_dataset_Legendre.eps}}
		\centerline{(a): \textit{Synth 1}}
	\end{minipage}
	\begin{minipage}{0.48\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/SAD/synth_dataset_new.eps}}
		\centerline{(b): \textit{Synth 2}}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}{0.48\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/SAD/synth_dataset_200_240.eps}}
		\centerline{(c): \textit{Synth 3}}
	\end{minipage}
	\begin{minipage}{0.48\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/SAD/jasper_dataset_20230410.eps}}
		\centerline{(d): \textit{Jasper Ridge}}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}{0.48\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/SAD/samson_dataset.eps}}
		\centerline{(e): \textit{Samson}}
	\end{minipage}
	\begin{minipage}{0.48\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/SAD/urban_dataset.eps}}
		\centerline{(f): \textit{Urban}}
	\end{minipage}
	
	\caption{The distributions of spectral angle distance (SAD) values between the spectra of endmembers present in HS images and the spectra of the other endmembers. Vertical axes indicate the spectral angle ditances. Horizontal axes indicate the indices of the endmembers present in the HS images. The SAD values tend to be the same for all the datasets.}
	\label{fig:SAD}
\end{figure}

%\vspace{-10mm}

==> fig_tex/fig_convergence_analysis_all_colored.tex <==
\begin{figure*}[t]
	\color{blue}
	\centering
	
	\begin{minipage}{0.19\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/jasper_dataset_20230410_Error_Iteration.eps}}
	\end{minipage}
	\begin{minipage}{0.19\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/jasper_dataset_20230410_function_values_Iteration.eps}}
	\end{minipage}
	\begin{minipage}{0.19\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/jasper_dataset_20230410_L2_distance_Iteration.eps}}
	\end{minipage}
	\begin{minipage}{0.19\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/jasper_dataset_20230410_L1_S_Iteration.eps}}
	\end{minipage}
	\begin{minipage}{0.19\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/jasper_dataset_20230410_L1_DvL_Iteration.eps}}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}{0.19\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_Error_Iteration.eps}}
	\end{minipage}
	\begin{minipage}{0.19\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_function_values_Iteration.eps}}
	\end{minipage}
	\begin{minipage}{0.19\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_L2_distance_Iteration.eps}}
	\end{minipage}
	\begin{minipage}{0.19\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_L1_S_Iteration.eps}}
	\end{minipage}
	\begin{minipage}{0.19\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_L1_DvL_Iteration.eps}}
	\end{minipage}
	
	\vspace{1mm}
	
	
	\begin{minipage}{0.19\hsize}
		\centerline{(a)}
	\end{minipage}
	\begin{minipage}{0.19\hsize}
		\centerline{(b)}
	\end{minipage}
	\begin{minipage}{0.19\hsize}
		\centerline{(c)}
	\end{minipage}	
	\begin{minipage}{0.19\hsize}
		\centerline{(d)}
	\end{minipage}
	\begin{minipage}{0.19\hsize}
		\centerline{(e)}
	\end{minipage}
	
	\vspace{-1mm}
	
	\caption{Convergence analysis using the real images. The top row shows the results of experiments using \textit{Jasper Ridge}. The bottom row shows the results of experiments using \textit{Samson}. (a): The relative error of abundance maps $\|\mathbf{X}^{(\NumIter+1)}-\mathbf{X}^{(\NumIter)}\|_F/\|\mathbf{X}^{(\NumIter+1)}\|_F$ versus iteration $\NumIter$. (b): Objective function value $\|\mathbf{X}^{(\NumIter)}\|_{1,2,r}+\lambda_1\|\mathbf{D}(\mathbf{X}^{(\NumIter)})\|_1+\lambda_2\mathcal{R}(\DiffHSIReg(\mathbf{A}\mathbf{X}^{(\NumIter)}))+\lambda_3\|\mathbf{L}^{(\NumIter)}\|_1$ versus iteration $\NumIter$.  (c): The $\ell_{2}$ distance between $\mathbf{Y}$ and $\mathbf{A}\mathbf{X}^{(\NumIter)}+\mathbf{S}^{(\NumIter)}+\mathbf{L}^{(\NumIter)}$ versus iteration $\NumIter$. (d): The $\ell_{1}$ norm of $\mathbf{S}^{(\NumIter)}$ versus iteration $\NumIter$. (e): The mean absolute values (MAV) of $\mathbf{D}_{v}(\mathbf{L}^{(\NumIter)})$ versus iteration $\NumIter$.} 
	\label{fig:convergence_analysis_all}
	\color{black}
\end{figure*}




==> fig_tex/fig_convergence_analysis_jasper.tex <==
\begin{figure}[t]
	\centering
	
	\begin{minipage}{0.32\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/jasper_dataset_20230410_Error_Iteration.eps}}
	\end{minipage}
	\begin{minipage}{0.32\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/jasper_dataset_20230410_function_values_Iteration.eps}}
	\end{minipage}
	\begin{minipage}{0.32\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/jasper_dataset_20230410_L2_distance_Iteration.eps}}
	\end{minipage}

\vspace{1mm}

	\begin{minipage}{0.32\hsize}
		\centerline{(a)}
	\end{minipage}
	\begin{minipage}{0.32\hsize}
		\centerline{(b)}
	\end{minipage}
	\begin{minipage}{0.32\hsize}
		\centerline{(c)}
	\end{minipage}

\vspace{1mm}

	\begin{minipage}{0.32\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/jasper_dataset_20230410_L1_S_Iteration.eps}}
	\end{minipage}
	\begin{minipage}{0.32\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/jasper_dataset_20230410_L1_DvL_Iteration.eps}}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}{0.32\hsize}
		\centerline{(d)}
	\end{minipage}
	\begin{minipage}{0.32\hsize}
		\centerline{(e)}
	\end{minipage}
	
	
	\caption{Convergence analysis using the real image (\textit{Jasper Ridge}). (a): The relative error of abundance maps $\|\mathbf{X}^{(\NumIter+1)}-\mathbf{X}^{(\NumIter)}\|_F/\|\mathbf{X}^{(\NumIter+1)}\|_F$ versus iteration $\NumIter$. (b): Objective function value $\|\mathbf{X}^{(\NumIter)}\|_{1,2,r}+\lambda_1\|\mathbf{D}(\mathbf{X}^{(\NumIter)})\|_1+\lambda_2\mathcal{R}(\DiffHSIReg(\mathbf{A}\mathbf{X}^{(\NumIter)}))+\lambda_3\|\mathbf{L}^{(\NumIter)}\|_1$ versus iteration $\NumIter$.  (c): The $\ell_{2}$ distance between $\mathbf{Y}$ and $\mathbf{A}\mathbf{X}^{(\NumIter)}+\mathbf{S}^{(\NumIter)}+\mathbf{L}^{(\NumIter)}$ versus iteration $\NumIter$. (d): The $\ell_{1}$ norm of $\mathbf{S}^{(\NumIter)}$ versus iteration $\NumIter$. (e): The mean absolute values (MAV) of $\mathbf{D}_{v}(\mathbf{L}^{(\NumIter)})$ versus iteration $\NumIter$.} 
	\label{fig:convergence_analysis_jasper}
\end{figure}


==> fig_tex/fig_convergence_analysis_samson.tex <==
%\begin{figure}[t]
%	\centering
%	\begin{minipage}{0.18\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_function_values_Iteration.eps}}
	%	\end{minipage}
%	\begin{minipage}{0.18\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_L2_distance_Iteration.eps}}
	%	\end{minipage}
%	\begin{minipage}{0.18\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_L1_S_Iteration.eps}}
	%	\end{minipage}
%	\begin{minipage}{0.18\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_L1_DvL_Iteration.eps}}
	%	\end{minipage}
%	\begin{minipage}{0.18\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_Error_Iteration.eps}}
	%	\end{minipage}
%	
%	\begin{minipage}{0.18\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_function_values_Time.eps}}
	%	\end{minipage}
%	\begin{minipage}{0.18\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_L2_distance_Time.eps}}
	%	\end{minipage}
%	\begin{minipage}{0.18\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_L1_S_Time.eps}}
	%	\end{minipage}
%	\begin{minipage}{0.18\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_L1_DvL_Time.eps}}
	%	\end{minipage}
%	\begin{minipage}{0.18\hsize}
	%		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_Error_Time.eps}}
	%	\end{minipage}
%	
%	\begin{minipage}{0.18\hsize}
	%		\centerline{(a)}
	%	\end{minipage}
%	\begin{minipage}{0.18\hsize}
	%		\centerline{(b)}
	%	\end{minipage}
%	\begin{minipage}{0.18\hsize}
	%		\centerline{(c)}
	%	\end{minipage}
%	\begin{minipage}{0.18\hsize}
	%		\centerline{(d)}
	%	\end{minipage}
%	\begin{minipage}{0.18\hsize}
	%		\centerline{(e)}
	%	\end{minipage}
%
%	
%	\caption{Original HS images. (a): A synthetic image generated using a Legendre method. 
	%		(b): A synthetic image generated using a spherical Gaussian method. (c): A real image (\textit{Jasper Ridge}).}
%	\label{fig:Org_HSimages}
%\end{figure}

\begin{figure}[t]
	\centering
	\begin{minipage}{0.32\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_Error_Iteration.eps}}
	\end{minipage}
	\begin{minipage}{0.32\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_function_values_Iteration.eps}}
	\end{minipage}
	\begin{minipage}{0.32\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_L2_distance_Iteration.eps}}
	\end{minipage}
	

\vspace{1mm}
	
	\begin{minipage}{0.32\hsize}
		\centerline{(a)}
	\end{minipage}
	\begin{minipage}{0.32\hsize}
		\centerline{(b)}
	\end{minipage}
	\begin{minipage}{0.32\hsize}
		\centerline{(c)}
	\end{minipage}
	
	\vspace{1mm}
	
	
	\begin{minipage}{0.32\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_L1_S_Iteration.eps}}
	\end{minipage}
	\begin{minipage}{0.32\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/graphs/eps/samson_dataset_L1_DvL_Iteration.eps}}
	\end{minipage}

\vspace{1mm}
	
	\begin{minipage}{0.32\hsize}
		\centerline{(d)}
	\end{minipage}
	\begin{minipage}{0.32\hsize}
		\centerline{(e)}
	\end{minipage}
	
	
	\caption{Convergence analysis using the real image (\textit{Samson}). (a): The relative error of abundance maps $\|\mathbf{X}^{(\NumIter+1)}-\mathbf{X}^{(\NumIter)}\|_F/\|\mathbf{X}^{(\NumIter+1)}\|_F$ versus iteration $\NumIter$. (b): Objective function value $\|\mathbf{X}^{(\NumIter)}\|_{1,2,r}+\lambda_1\|\mathbf{D}(\mathbf{X}^{(\NumIter)})\|_1+\lambda_2\mathcal{R}(\DiffHSIReg(\mathbf{A}\mathbf{X}^{(\NumIter)}))+\lambda_3\|\mathbf{L}^{(\NumIter)}\|_1$ versus iteration $\NumIter$.  (c): The $\ell_{2}$ distance between $\mathbf{Y}$ and $\mathbf{A}\mathbf{X}^{(\NumIter)}+\mathbf{S}^{(\NumIter)}+\mathbf{L}^{(\NumIter)}$ versus iteration $\NumIter$. (d): The $\ell_{1}$ norm of $\mathbf{S}^{(\NumIter)}$ versus iteration $\NumIter$. (e): The mean absolute values (MAV) of $\mathbf{D}_{v}(\mathbf{L}^{(\NumIter)})$ versus iteration $\NumIter$. }
	\label{fig:convergence_analysis_samson}
\end{figure}


==> fig_tex/fig_other_spectra.tex <==
\begin{figure}[t]
	\centering
	\begin{minipage}[t]{0.48\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/experiment/spectral_others_jasper.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.48\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/experiment/spectral_others_samson.eps}
		}
	\end{minipage}
	
	
	\begin{minipage}[t]{0.48\hsize}
		\centerline{
			(a): \textit{Jasper Ridge}
		}
	\end{minipage}
	\begin{minipage}[t]{0.48\hsize}
		\centerline{
			(b): \textit{Samson}
		}
	\end{minipage}
	
	\caption{Spectral signatures added into endmember libraries of real image experiments.}
	\label{fig:other_spectra}
\end{figure}




==> fig_tex/fig_other_spectra_colored.tex <==
\begin{figure}[t]
	\centering
	\begin{minipage}[t]{0.48\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/experiment/spectral_others_jasper.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.48\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/experiment/spectral_others_samson.eps}
		}
	\end{minipage}
	
	
	\begin{minipage}[t]{0.48\hsize}
		\centerline{
			(a): \textit{Jasper Ridge}
		}
	\end{minipage}
	\begin{minipage}[t]{0.48\hsize}
		\centerline{
			(b): \textit{Samson}
		}
	\end{minipage}
	
	\vspace{-1mm}
	
	\caption{\textcolor{blue}{Endmembers added in endmember libraries of real image experiments.}}
	\label{fig:other_spectra}
\end{figure}




==> fig_tex/fig_real_HSI_01_00_00_colored.tex <==
\begin{figure*}[t]
	\color{blue}
	\centering
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/original/0.1_0_0/Orig_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/original/0.1_0_0/Noisy_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/CLSUnSAL/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/JSTV/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/RSSUn-TV/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/LGSU/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/UnDIP/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/EGU_Net/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/RDSWSU/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/MdLRR/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/Reshaped-HTV/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/Reshaped-SSTV/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/Reshaped-HSSTV/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(d)
		}
	\end{minipage}        
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(g)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(h)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			{(i)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			{(j)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(k)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(l)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(m)}
		}
	\end{minipage}
	
	
	\caption{Reconstructed HS image results for the \textit{Jasper Ridge} experiments in Case 2. (a): Original HS image. (b): Noisy image. (c): CLSUnSAL \cite{iordache2014collaborative}.  (d): JSTV~\cite{aggarwal2016hyperspectral}. (e): RSSUn-TV~\cite{wang2019row}. (f): LGSU~\cite{shen2022superpixel}. (g): UnDIP~\cite{UnDIP_RastiB_2022}. (h): EGU-Net~\cite{hong2022endmember}. (i): RDSWSU~\cite{rs_Deng_RobustDual_2023}. (j): MdLRR~\cite{MDLRR_WuLing_2023}. (k): \textbf{\Ourss (HTV)}. (l): \textbf{\Ourss (SSTV)}. (m): \textbf{\Ourss (HSSTV)}.}
	\label{real_HSI_0.1_0_0}
\end{figure*}




==> fig_tex/fig_real_HSI_05_05_05.tex <==
\begin{figure*}[t]
\centering
    \begin{minipage}[t]{0.085\hsize}
        \centerline{
        \includegraphics[width=\hsize]{./fig/real/original/0.05_0.05_0.05/Orig_HSI.eps}
        }
    \end{minipage}
    \begin{minipage}[t]{0.085\hsize}
        \centerline{
        \includegraphics[width=\hsize]{./fig/real/original/0.05_0.05_0.05/Noisy_HSI.eps}
        }
    \end{minipage}
    \begin{minipage}[t]{0.085\hsize}
        \centerline{
        \includegraphics[width=\hsize]{./fig/real/CLSUnSAL_0.0003/0.05_0.05_0.05/Recons_HSI.eps}
        }
    \end{minipage}
    \begin{minipage}[t]{0.085\hsize}
    	\centerline{
    		\includegraphics[width=\hsize]{./fig/real/JSTV_2_0.1_1_/0.05_0.05_0.05/Recons_HSI.eps}
    	}
    \end{minipage}
    \begin{minipage}[t]{0.085\hsize}
    	\centerline{
    		\includegraphics[width=\hsize]{./fig/real/RSSUnTV_0.5_0.001_/0.05_0.05_0.05/Recons_HSI.eps}
    	}
    \end{minipage}
    \begin{minipage}[t]{0.085\hsize}
    	\centerline{
    		\includegraphics[width=\hsize]{./fig/real/lgsu/0.05_0.05_0.05/Recons_HSI.eps}
    	}
    \end{minipage}
	\begin{minipage}[t]{0.085\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/UnDIP/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.085\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/MdLRR/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.085\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/Reshaped_HTV_2_2_1_/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.085\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/Reshaped_SSTV_2_2_1_/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.085\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real/Reshaped_HSSTV_2_2_1_/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
                
    \begin{minipage}[t]{0.085\hsize}
        \centerline{
        (a)
        }
    \end{minipage}
    \begin{minipage}[t]{0.085\hsize}
        \centerline{
        (b)
        }
    \end{minipage}
    \begin{minipage}[t]{0.085\hsize}
        \centerline{
        (c)
        }
    \end{minipage}
    \begin{minipage}[t]{0.085\hsize}
        \centerline{
        (d)
        }
    \end{minipage}
    \begin{minipage}[t]{0.085\hsize}
        \centerline{
        (e)
        }
    \end{minipage}
    \begin{minipage}[t]{0.085\hsize}
        \centerline{
        (f)
        }
    \end{minipage}
    \begin{minipage}[t]{0.085\hsize}
        \centerline{
        (g)
        }
    \end{minipage}
    \begin{minipage}[t]{0.085\hsize}
        \centerline{
        (h)
        }
    \end{minipage}
    \begin{minipage}[t]{0.085\hsize}
        \centerline{
        \textbf{(i)}
        }
    \end{minipage}
	\begin{minipage}[t]{0.085\hsize}
		\centerline{
			\textbf{(j)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.085\hsize}
	\centerline{
		\textbf{(k)}
	}
	\end{minipage}
        

\caption{Reconstructed HS image results for the \textit{Jasper Ridge} experiments in Case 5. (a): Original HS image. (b): Noisy image. (c): CLSUnSAL \cite{iordache2014collaborative}.  (d): JSTV~\cite{aggarwal2016hyperspectral}. (e): RSSUn-TV~\cite{wang2019row}. (f): LGSU~\cite{shen2022superpixel}. (g): UnDIP~\cite{UnDIP_RastiB_2022}. (h): MdLRR~\cite{MDLRR_WuLing_2023}. (i): \textbf{\Ourss (HTV)}. (j): \textbf{\Ourss (SSTV)}. (k): \textbf{\Ourss (HSSTV)}.}
\label{real_HSI_0.05_0.05_0.05}
\end{figure*}



==> fig_tex/fig_real_samson_HSI_01_05_05_colored.tex <==
\begin{figure*}[!h]
	\color{blue}
	\centering
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_samson/original/0.1_0.05_0.05/Orig_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_samson/original/0.1_0.05_0.05/Noisy_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_samson/CLSUnSAL/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_samson/JSTV/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_samson/RSSUn-TV/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_samson/LGSU/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_samson/UnDIP/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_samson/EGU_Net/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_samson/RDSWSU/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_samson/MdLRR/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_samson/Reshaped-HTV/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_samson/Reshaped-SSTV/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_samson/Reshaped-HSSTV/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(g)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(h)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			{(i)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			{(j)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(k)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(l)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(m)}
		}
	\end{minipage}
	
	
	\caption{Reconstructed HS image results for the \textit{samson} experiments in Case 6. (a): Original HS image. (b): Noisy image. (c): CLSUnSAL \cite{iordache2014collaborative}.  (d): JSTV~\cite{aggarwal2016hyperspectral}. (e): RSSUn-TV~\cite{wang2019row}. (f): LGSU~\cite{shen2022superpixel}. (g): UnDIP~\cite{UnDIP_RastiB_2022}. (h): EGU-Net~\cite{hong2022endmember}. (i): RDSWSU~\cite{rs_Deng_RobustDual_2023}. (j): MdLRR~\cite{MDLRR_WuLing_2023}. (k): \textbf{\Ourss (HTV)}. (l): \textbf{\Ourss (SSTV)}. (m): \textbf{\Ourss (HSSTV)}.}
	\label{real_samson_HSI_0.1_0.05_0.05}
\end{figure*}



==> fig_tex/fig_real_urban_HSI_noniid_01_01_colored.tex <==
\begin{figure*}[t]
	\color{blue}
	\centering
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_urban_noniid/original/Noniid_0.05_0.05/Orig_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_urban_noniid/original/Noniid_0.05_0.05/Noisy_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_urban_noniid/CLSUnSAL/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_urban_noniid/JSTV/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_urban_noniid/RSSUn-TV/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_urban_noniid/LGSU/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_urban_noniid/UnDIP/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_urban_noniid/EGU_Net/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_urban_noniid/RDSWSU/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_urban_noniid/MdLRR/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_urban_noniid/Reshaped-HTV/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_urban_noniid/Reshaped-SSTV/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/real_urban_noniid/Reshaped-HSSTV/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(d)
		}
	\end{minipage}        
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(g)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(h)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			{(i)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			{(j)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(k)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(l)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(m)}
		}
	\end{minipage}
	
	
	\caption{Reconstructed HS image results for the \textit{Urban} experiments in Case 8. (a): Original HS image. (b): Noisy image. (c): CLSUnSAL \cite{iordache2014collaborative}.  (d): JSTV~\cite{aggarwal2016hyperspectral}. (e): RSSUn-TV~\cite{wang2019row}. (f): LGSU~\cite{shen2022superpixel}. (g): UnDIP~\cite{UnDIP_RastiB_2022}. (h): EGU-Net~\cite{hong2022endmember}. (i): RDSWSU~\cite{rs_Deng_RobustDual_2023}. (j): MdLRR~\cite{MDLRR_WuLing_2023}. (k): \textbf{\Ourss (HTV)}. (l): \textbf{\Ourss (SSTV)}. (m): \textbf{\Ourss (HSSTV)}.}
	\label{real_urban_noniid_HSI_Noniid_0.05_0.05}
\end{figure*}




==> fig_tex/fig_results_HSI_ablation_jasper.tex <==
\begin{figure}[!h]
	\centering
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/samson_dataset_marked/original/0.1_0.05_0.05/Orig_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/samson_dataset_marked/original/0.1_0.05_0.05/Noisy_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/samson_dataset_marked/ours_ablation/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/samson_dataset_marked/Reshaped_HTV_2_2_1_/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/samson_dataset_marked/Reshaped_SSTV_2_2_1_/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/samson_dataset_marked/Reshaped_HSSTV_2_2_1_/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(f)
		}
	\end{minipage}


\vspace{-1mm}	
	
	
	
	\caption{Reconstructed HS image results for the \textit{Samson} experiments in Case 6. (a): Original HS image. (b): Noisy image. (c): RCHU (--). (d): \textbf{\Ourss (HTV)}. (e): \textbf{\Ourss (SSTV)}. (f): \textbf{\Ourss (HSSTV)}.}
	\label{fig:results_HSI_ablation_samson}
\end{figure}



==> fig_tex/fig_results_HSI_ablation_jasper_blue.tex <==
\begin{figure}[!h]
	\color{blue}
	\centering
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/samson_dataset_marked/original/0.1_0.05_0.05/Orig_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/samson_dataset_marked/original/0.1_0.05_0.05/Noisy_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/samson_dataset_marked/ours_ablation/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/samson_dataset_marked/Reshaped_HTV_2_2_1_/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/samson_dataset_marked/Reshaped_SSTV_2_2_1_/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/samson_dataset_marked/Reshaped_HSSTV_2_2_1_/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	
	
	\vspace{-1mm}	
	
	
	
	\caption{Reconstructed HS image results for the \textit{Samson} experiments in Case 6. (a): Original HS image. (b): Noisy image. (c): RCHU (--). (d): \textbf{\Ourss (HTV)}. (e): \textbf{\Ourss (SSTV)}. (f): \textbf{\Ourss (HSSTV)}.}
	\label{fig:results_HSI_ablation_samson}
	\color{black}
\end{figure}



==> fig_tex/fig_results_HSI_ablation_syn_leg.tex <==
\begin{figure}[t]
	\centering
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_dataset_marked/original/0.1_0.05_0.05/Orig_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_dataset_marked/original/0.1_0.05_0.05/Noisy_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_dataset_marked/ours_ablation/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_dataset_marked/Reshaped_HTV_2_2_1_/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_dataset_marked/Reshaped_SSTV_2_2_1_/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_dataset_marked/Reshaped_HSSTV_2_2_1_/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	
	\vspace{-1mm}
	
	
	
	
	\caption{Reconstructed HS image results for the \textit{Synth 2} experiments in Case 6. (a): Original HS image. (b): Noisy image. (c): RCHU (--). (d): \textbf{\Ourss (HTV)}. (e): \textbf{\Ourss (SSTV)}. (f): \textbf{\Ourss (HSSTV)}.}
	\label{fig:results_HSI_ablation_syn_gau}
\end{figure}



==> fig_tex/fig_results_HSI_ablation_syn_leg_colored.tex <==
\begin{figure}[t]
	\color{blue}
	\centering
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_dataset_marked/original/0.1_0.05_0.05/Orig_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_dataset_marked/original/0.1_0.05_0.05/Noisy_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_dataset_marked/ours_ablation/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_dataset_marked/Reshaped_HTV_2_2_1_/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_dataset_marked/Reshaped_SSTV_2_2_1_/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_dataset_marked/Reshaped_HSSTV_2_2_1_/0.1_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.15\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	
	\vspace{-1mm}
	
	
	
	
	\caption{Reconstructed HS image results for the synthetic HS image 2 experiments in Case 6. (a): Original HS image. (b): Noisy image. (c): RCHU (--). (d): \textbf{\Ourss (HTV)}. (e): \textbf{\Ourss (SSTV)}. (f): \textbf{\Ourss (HSSTV)}.}
	\label{fig:results_HSI_ablation_syn_gau}
	\color{black}
\end{figure}



==> fig_tex/fig_results_ablation_samson.tex <==

\begin{figure}[t]
	\centering
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/original/0.1_0.05_0.05/Orig_3.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/ours_ablation/0.1_0.05_0.05/Recons_3.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/Reshaped_HTV_2_2_1_/0.1_0.05_0.05/Recons_3.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/Reshaped_SSTV_2_2_1_/0.1_0.05_0.05/Recons_3.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/Reshaped_HSSTV_2_2_1_/0.1_0.05_0.05/Recons_3.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.03\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/original/0.1_0.05_0.05/Orig_other_4.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/ours_ablation/0.1_0.05_0.05/Recons_other_4.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/Reshaped_HTV_2_2_1_/0.1_0.05_0.05/Recons_other_4.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/Reshaped_SSTV_2_2_1_/0.1_0.05_0.05/Recons_other_4.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/Reshaped_HSSTV_2_2_1_/0.1_0.05_0.05/Recons_other_4.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.03\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/colorbar_max_0.1.png}
		}
	\end{minipage}
	
	
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.03\hsize}
		\centerline{
			~
		}
	\end{minipage}
	
	\vspace{-1mm}
	
	\caption{Abundance maps of ablation experiments for the \textit{Samson} experiments in Case 6. (a): Original abundance maps.  (b): \Ourss (--). (c): \textbf{\Ourss (HTV)}. (d): \textbf{\Ourss (SSTV)}. (e): \textbf{\Ourss (HSSTV)}.}
	\label{fig:results_ablation_samson}
\end{figure}



==> fig_tex/fig_results_ablation_samson_colored.tex <==

\begin{figure}[t]
	\color{blue}
	\centering
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/original/0.1_0.05_0.05/Orig_3.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/ours_ablation/0.1_0.05_0.05/Recons_3.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/Reshaped_HTV_2_2_1_/0.1_0.05_0.05/Recons_3.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/Reshaped_SSTV_2_2_1_/0.1_0.05_0.05/Recons_3.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/Reshaped_HSSTV_2_2_1_/0.1_0.05_0.05/Recons_3.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.03\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/original/0.1_0.05_0.05/Orig_other_4.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/ours_ablation/0.1_0.05_0.05/Recons_other_4.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/Reshaped_HTV_2_2_1_/0.1_0.05_0.05/Recons_other_4.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/Reshaped_SSTV_2_2_1_/0.1_0.05_0.05/Recons_other_4.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/samson_dataset_marked/Reshaped_HSSTV_2_2_1_/0.1_0.05_0.05/Recons_other_4.png}
		}
	\end{minipage}
	\begin{minipage}[t]{0.03\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/colorbar_max_0.1.png}
		}
	\end{minipage}
	
	
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.03\hsize}
		\centerline{
			~
		}
	\end{minipage}
	
	\vspace{-1mm}
	
	\caption{Abundance maps of ablation experiments for the \textit{Samson} experiments in Case 6. (a): Original abundance maps.  (b): \Ourss (--). (c): \textbf{\Ourss (HTV)}. (d): \textbf{\Ourss (SSTV)}. (e): \textbf{\Ourss (HSSTV)}.}
	\label{fig:results_ablation_samson}
	\color{black}
\end{figure}



==> fig_tex/fig_results_ablation_syn_gau.tex <==

\begin{figure}[t]
	\centering
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/original/0.1_0.05_0.05/Orig_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/ours_ablation/0.1_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/Reshaped_HTV_2_2_1_/0.1_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/Reshaped_SSTV_2_2_1_/0.1_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/Reshaped_HSSTV_2_2_1_/0.1_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.03\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/original/0.1_0.05_0.05/Orig_other_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/ours_ablation/0.1_0.05_0.05/Recons_other_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/Reshaped_HTV_2_2_1_/0.1_0.05_0.05/Recons_other_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/Reshaped_SSTV_2_2_1_/0.1_0.05_0.05/Recons_other_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/Reshaped_HSSTV_2_2_1_/0.1_0.05_0.05/Recons_other_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.03\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/colorbar_max_0.1.png}
		}
	\end{minipage}
	
	
	
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.03\hsize}
		\centerline{
			~
		}
	\end{minipage}
	
	\vspace{-1mm}
	
	\caption{Abundance maps of ablation experiments for the \textit{Synth 2} experiments in Case 6. (a): Original abundance maps.  (b): \Ourss (--). (c): \textbf{\Ourss (HTV)}. (d): \textbf{\Ourss (SSTV)}. (e): \textbf{\Ourss (HSSTV)}.}
	\label{fig:results_ablation_syn_gau}
\end{figure}



==> fig_tex/fig_results_ablation_syn_gau_colored.tex <==

\begin{figure}[t]
	\color{blue}
	\centering
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/original/0.1_0.05_0.05/Orig_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/ours_ablation/0.1_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/Reshaped_HTV_2_2_1_/0.1_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/Reshaped_SSTV_2_2_1_/0.1_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/Reshaped_HSSTV_2_2_1_/0.1_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.03\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/original/0.1_0.05_0.05/Orig_other_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/ours_ablation/0.1_0.05_0.05/Recons_other_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/Reshaped_HTV_2_2_1_/0.1_0.05_0.05/Recons_other_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/Reshaped_SSTV_2_2_1_/0.1_0.05_0.05/Recons_other_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/synth_dataset_marked/Reshaped_HSSTV_2_2_1_/0.1_0.05_0.05/Recons_other_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.03\hsize}
		\centerline{
			\includegraphics[height = 45pt]{./fig/colorbar_max_0.1.png}
		}
	\end{minipage}
	
	
	
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.18\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.03\hsize}
		\centerline{
			~
		}
	\end{minipage}
	
	\vspace{-1mm}
	
	\caption{Abundance maps of ablation experiments for the synthetic HS image 2 experiments in Case 6. (a): Original abundance maps.  (b): \Ourss (--). (c): \textbf{\Ourss (HTV)}. (d): \textbf{\Ourss (SSTV)}. (e): \textbf{\Ourss (HSSTV)}.}
	\label{fig:results_ablation_syn_gau}
	\color{black}
\end{figure}



==> fig_tex/fig_results_real_01_00_00_colored.tex <==
\begin{figure*}[t]
	\color{blue}
	\centering
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/original/0.1_0_0/Orig_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/CLSUnSAL/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/JSTV/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/RSSUn-TV/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/lgsu/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/UnDIP/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/EGU_Net/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/RDSWSU/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/MdLRR/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/Reshaped-HTV/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/Reshaped-SSTV/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/Reshaped-HSSTV/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/original/0.1_0_0/Orig_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/CLSUnSAL/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/JSTV/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/RSSUn-TV/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/LGSU/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/UnDIP/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/EGU_Net/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/RDSWSU/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/MdLRR/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/Reshaped-HTV/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/Reshaped-SSTV/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/Reshaped-HSSTV/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/original/0.1_0_0/Orig_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/CLSUnSAL/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/JSTV/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/RSSUn-TV/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/LGSU/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/UnDIP/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/EGU_Net/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/RDSWSU/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/MdLRR/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/Reshaped-HTV/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/Reshaped-SSTV/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/Reshaped-HSSTV/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/original/0.1_0_0/Orig_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/CLSUnSAL/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/JSTV/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/RSSUn-TV/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/LGSU/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/UnDIP/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/EGU_Net/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/RDSWSU/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/MdLRR/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/Reshaped-HTV/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/Reshaped-SSTV/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real/Reshaped-HSSTV/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(g)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			{(h)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			{(i)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(j)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(k)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(l)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			~
		}
	\end{minipage}
	
	\caption{Unmixing results of abundance maps for the \textit{Jasper Ridge} experiments in Case 2. (a): Original abundance maps. (b): CLSUnSAL~\cite{iordache2014collaborative}. (c): JSTV~\cite{aggarwal2016hyperspectral}. (d): RSSUn-TV~\cite{wang2019row}. (e): LGSU~\cite{shen2022superpixel}. (f): UnDIP~\cite{UnDIP_RastiB_2022}. (g): EGU-Net~\cite{hong2022endmember}. (h): RDSWSU~\cite{rs_Deng_RobustDual_2023}. (i): MdLRR~\cite{MDLRR_WuLing_2023}. (j): \textbf{\Ourss (HTV)}. (k): \textbf{\Ourss (SSTV)}. (l): \textbf{\Ourss (HSSTV)}.}
	\label{real_0.1_0_0}
\end{figure*}







==> fig_tex/fig_results_real_05_05_05.tex <==
\begin{figure*}[!h]
\centering
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/original/0.05_0.05_0.05/Orig_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/CLSUnSAL_0.0003/0.05_0.05_0.05/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/JSTV_2_0.1_1_/0.05_0.05_0.05/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/RSSUnTV_0.5_0.001_/0.05_0.05_0.05/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/lgsu/0.05_0.05_0.05/Recons_1.eps}
            }
        \end{minipage}        
	    \begin{minipage}[t]{0.09\hsize}
	    	\centerline{
	    		\includegraphics[height = 48pt]{./fig/real/UnDIP/0.05_0.05_0.05/Recons_1.eps}
	    	}
	    \end{minipage}        
	    \begin{minipage}[t]{0.09\hsize}
		    \centerline{
		    	\includegraphics[height = 48pt]{./fig/real/MdLRR/0.05_0.05_0.05/Recons_1.eps}
		    }
	    \end{minipage}        
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/Reshaped_HTV_2_2_1_/0.05_0.05_0.05/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/Reshaped_SSTV_2_2_1_/0.05_0.05_0.05/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/Reshaped_HSSTV_2_2_1_/0.05_0.05_0.05/Recons_1.eps}
            }
        \end{minipage}
	    \begin{minipage}[t]{0.02\hsize}
	    	\centerline{
	    		\includegraphics[height = 48pt]{./fig/colorbar_20.png}
	    	}
	    \end{minipage}
    
\vspace{1mm}
        
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/original/0.05_0.05_0.05/Orig_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/CLSUnSAL_0.0003/0.05_0.05_0.05/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/JSTV_2_0.1_1_/0.05_0.05_0.05/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/RSSUnTV_0.5_0.001_/0.05_0.05_0.05/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/lgsu/0.05_0.05_0.05/Recons_2.eps}
            }
        \end{minipage} 
	    \begin{minipage}[t]{0.09\hsize}
	    	\centerline{
	    		\includegraphics[height = 48pt]{./fig/real/UnDIP/0.05_0.05_0.05/Recons_2.eps}
	    	}
	    \end{minipage} 
	    \begin{minipage}[t]{0.09\hsize}
		    \centerline{
		    	\includegraphics[height = 48pt]{./fig/real/MdLRR/0.05_0.05_0.05/Recons_2.eps}
		    }
	    \end{minipage} 
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/Reshaped_HTV_2_2_1_/0.05_0.05_0.05/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/Reshaped_SSTV_2_2_1_/0.05_0.05_0.05/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/Reshaped_HSSTV_2_2_1_/0.05_0.05_0.05/Recons_2.eps}
            }
        \end{minipage}
	    \begin{minipage}[t]{0.02\hsize}
	    	\centerline{
	    		\includegraphics[height = 48pt]{./fig/colorbar_20.png}
	    	}
	    \end{minipage}
    
\vspace{1mm}
        
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/original/0.05_0.05_0.05/Orig_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/CLSUnSAL_0.0003/0.05_0.05_0.05/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/JSTV_2_0.1_1_/0.05_0.05_0.05/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/RSSUnTV_0.5_0.001_/0.05_0.05_0.05/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/lgsu/0.05_0.05_0.05/Recons_3.eps}
            }
        \end{minipage} 
	    \begin{minipage}[t]{0.09\hsize}
	    	\centerline{
	    		\includegraphics[height = 48pt]{./fig/real/UnDIP/0.05_0.05_0.05/Recons_3.eps}
	    	}
	    \end{minipage} 
	    \begin{minipage}[t]{0.09\hsize}
		    \centerline{
		    	\includegraphics[height = 48pt]{./fig/real/MdLRR/0.05_0.05_0.05/Recons_3.eps}
		    }
	    \end{minipage} 
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/Reshaped_HTV_2_2_1_/0.05_0.05_0.05/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/Reshaped_SSTV_2_2_1_/0.05_0.05_0.05/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/Reshaped_HSSTV_2_2_1_/0.05_0.05_0.05/Recons_3.eps}
            }
        \end{minipage}
	    \begin{minipage}[t]{0.02\hsize}
	    	\centerline{
	    		\includegraphics[height = 48pt]{./fig/colorbar_20.png}
	    	}
	    \end{minipage}
    
\vspace{1mm}
        
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/original/0.05_0.05_0.05/Orig_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/CLSUnSAL_0.0003/0.05_0.05_0.05/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/JSTV_2_0.1_1_/0.05_0.05_0.05/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/RSSUnTV_0.5_0.001_/0.05_0.05_0.05/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/lgsu/0.05_0.05_0.05/Recons_4.eps}
            }
        \end{minipage} 
	    \begin{minipage}[t]{0.09\hsize}
	    	\centerline{
	    		\includegraphics[height = 48pt]{./fig/real/UnDIP/0.05_0.05_0.05/Recons_4.eps}
	    	}
	    \end{minipage} 
	    \begin{minipage}[t]{0.09\hsize}
		    \centerline{
		    	\includegraphics[height = 48pt]{./fig/real/MdLRR/0.05_0.05_0.05/Recons_4.eps}
		    }
	    \end{minipage} 
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/Reshaped_HTV_2_2_1_/0.05_0.05_0.05/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/Reshaped_SSTV_2_2_1_/0.05_0.05_0.05/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \includegraphics[height = 48pt]{./fig/real/Reshaped_HSSTV_2_2_1_/0.05_0.05_0.05/Recons_4.eps}
            }
        \end{minipage}
	    \begin{minipage}[t]{0.02\hsize}
	    	\centerline{
	    		\includegraphics[height = 48pt]{./fig/colorbar_20.png}
	    	}
	    \end{minipage}
        
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            (a)
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            (b)
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            (c)
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            (d)
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            (e)
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            (f)
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            (g)
            }
        \end{minipage}
        \begin{minipage}[t]{0.09\hsize}
            \centerline{
            \textbf{(h)}
            }
        \end{minipage}
	    \begin{minipage}[t]{0.09\hsize}
	    	\centerline{
	    		\textbf{(i)}
	    	}
	    \end{minipage}
	    \begin{minipage}[t]{0.09\hsize}
	    \centerline{
	    	\textbf{(j)}
	    }
	    \end{minipage}
	    \begin{minipage}[t]{0.02\hsize}
	    	\centerline{
	    		~
	    	}
	    \end{minipage}

\caption{Unmixing results of abundance maps for the \textit{Jasper Ridge} experiments in Case 5. (a): Original abundance maps. (b): CLSUnSAL \cite{iordache2014collaborative}. (c): JSTV~\cite{aggarwal2016hyperspectral}. (d): RSSUn-TV~\cite{wang2019row}. (e): LGSU~\cite{shen2022superpixel}. (f): UnDIP~\cite{UnDIP_RastiB_2022}. (g): MdLRR~\cite{MDLRR_WuLing_2023}. (h): \textbf{\Ourss (HTV)}. (i): \textbf{\Ourss (SSTV)}. (j): \textbf{\Ourss (HSSTV)}.}
\label{real_0.05_0.05_0.05}
\end{figure*}






==> fig_tex/fig_results_real_samson_01_05_00.tex <==
\begin{figure*}[t]
	\centering
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/original/0.05_0.1_0/Orig_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/CLSUnSAL_0.0003/0.05_0.1_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/JSTV_2_0.1_1_/0.05_0.1_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/RSSUnTV_0.5_0.001_/0.05_0.1_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/lgsu/0.05_0.1_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/UnDIP/0.05_0.1_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/Reshaped_HTV_2_2_1_/0.05_0.1_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/Reshaped_SSTV_2_2_1_/0.05_0.1_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/Reshaped_HSSTV_2_2_1_/0.05_0.1_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/original/0.05_0.1_0/Orig_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/CLSUnSAL_0.0003/0.05_0.1_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/JSTV_2_0.1_1_/0.05_0.1_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/RSSUnTV_0.5_0.001_/0.05_0.1_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/lgsu/0.05_0.1_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/UnDIP/0.05_0.1_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/Reshaped_HTV_2_2_1_/0.05_0.1_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/Reshaped_SSTV_2_2_1_/0.05_0.1_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/Reshaped_HSSTV_2_2_1_/0.05_0.1_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/original/0.05_0.1_0/Orig_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/CLSUnSAL_0.0003/0.05_0.1_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/JSTV_2_0.1_1_/0.05_0.1_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/RSSUnTV_0.5_0.001_/0.05_0.1_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/lgsu/0.05_0.1_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/UnDIP/0.05_0.1_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/Reshaped_HTV_2_2_1_/0.05_0.1_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/Reshaped_SSTV_2_2_1_/0.05_0.1_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/real_samson/Reshaped_HSSTV_2_2_1_/0.05_0.1_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 52pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\textbf{(g)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\textbf{(h)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\textbf{(i)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			~
		}
	\end{minipage}
	
	\caption{Unmixing results of abundance maps for the real samson data in Case 4. (a): Original abundance maps. (b): CLSUnSAL~\cite{iordache2014collaborative}. (c): JSTV~\cite{aggarwal2016hyperspectral}. (d): RSSUn-TV~\cite{wang2019row}. (e): LGSU~\cite{shen2022superpixel}. (f): UnDIP~\cite{UnDIP}. (g): \textbf{\Ourss (HTV)}. (h): \textbf{\Ourss (SSTV)}. (i): \textbf{\Ourss (HSSTV)}.}
	\label{real_samson_0.05_0.1_0}
\end{figure*}







==> fig_tex/fig_results_real_samson_01_05_05_colored.tex <==
\begin{figure*}[t]
	\color{blue}
	\centering
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/original/0.1_0.05_0.05/Orig_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/CLSUnSAL/0.1_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/JSTV/0.1_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/RSSUn-TV/0.1_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/LGSU/0.1_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/UnDIP/0.1_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/EGU_Net/0.1_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/RDSWSU/0.1_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/MdLRR/0.1_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/Reshaped-HTV/0.1_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/Reshaped-SSTV/0.1_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/Reshaped-HSSTV/0.1_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/original/0.1_0.05_0.05/Orig_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/CLSUnSAL/0.1_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/JSTV/0.1_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/RSSUn-TV/0.1_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/LGSU/0.1_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/UnDIP/0.1_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/EGU_Net/0.1_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/RDSWSU/0.1_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/MdLRR/0.1_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/Reshaped-HTV/0.1_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/Reshaped-SSTV/0.1_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/Reshaped-HSSTV/0.1_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/original/0.1_0.05_0.05/Orig_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/CLSUnSAL/0.1_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/JSTV/0.1_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/RSSUn-TV/0.1_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/LGSU/0.1_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/UnDIP/0.1_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/EGU_Net/0.1_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/RDSWSU/0.1_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/MdLRR/0.1_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/Reshaped-HTV/0.1_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/Reshaped-SSTV/0.1_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_samson/Reshaped-HSSTV/0.1_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(g)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			{(h)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			{(i)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(j)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(k)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(l)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			~
		}
	\end{minipage}
	
	\caption{Unmixing results of abundance maps for the \textit{Samson} experiments in Case 6. (a): Original abundance maps. (b): CLSUnSAL~\cite{iordache2014collaborative}. (c): JSTV~\cite{aggarwal2016hyperspectral}. (d): RSSUn-TV~\cite{wang2019row}. (e): LGSU~\cite{shen2022superpixel}. (f): UnDIP~\cite{UnDIP_RastiB_2022}. (g): EGU-Net~\cite{hong2022endmember}. (h): RDSWSU~\cite{rs_Deng_RobustDual_2023}. (i): MdLRR~\cite{MDLRR_WuLing_2023}. (j): \textbf{\Ourss (HTV)}. (k): \textbf{\Ourss (SSTV)}. (l): \textbf{\Ourss (HSSTV)}.}
	\label{real_samson_0.1_0.05_0.05}
\end{figure*}







==> fig_tex/fig_results_real_urban_noniid_01_01_colored.tex <==
\begin{figure*}[!h]
	\color{blue}
	\centering
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/original/Noniid_0.05_0.05/Orig_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/CLSUnSAL/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/JSTV/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/RSSUn-TV/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/lgsu/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/UnDIP/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/EGU_Net/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/RDSWSU/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/MdLRR/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/Reshaped-HTV/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/Reshaped-SSTV/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/Reshaped-HSSTV/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/original/Noniid_0.05_0.05/Orig_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/CLSUnSAL/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/JSTV/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/RSSUn-TV/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/LGSU/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/UnDIP/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/EGU_Net/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/RDSWSU/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/MdLRR/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/Reshaped-HTV/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/Reshaped-SSTV/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/Reshaped-HSSTV/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/original/Noniid_0.05_0.05/Orig_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/CLSUnSAL/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/JSTV/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/RSSUn-TV/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/LGSU/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/UnDIP/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/EGU_Net/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/RDSWSU/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/MdLRR/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/Reshaped-HTV/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/Reshaped-SSTV/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/Reshaped-HSSTV/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/original/Noniid_0.05_0.05/Orig_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/CLSUnSAL/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/JSTV/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/RSSUn-TV/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/LGSU/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/UnDIP/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/EGU_Net/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/RDSWSU/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/MdLRR/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/Reshaped-HTV/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/Reshaped-SSTV/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/real_urban_noniid/Reshaped-HSSTV/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(g)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			{(h)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			{(i)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(j)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(k)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(l)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			~
		}
	\end{minipage}
	
	\caption{Unmixing results of abundance maps for the \textit{Urban} experiments in Case 8. (a): Original abundance maps. (b): CLSUnSAL~\cite{iordache2014collaborative}. (c): JSTV~\cite{aggarwal2016hyperspectral}. (d): RSSUn-TV~\cite{wang2019row}. (e): LGSU~\cite{shen2022superpixel}. (f): UnDIP~\cite{UnDIP_RastiB_2022}. (g): EGU-Net~\cite{hong2022endmember}. (h): RDSWSU~\cite{rs_Deng_RobustDual_2023}. (i): MdLRR~\cite{MDLRR_WuLing_2023}. (j): \textbf{\Ourss (HTV)}. (k): \textbf{\Ourss (SSTV)}. (l): \textbf{\Ourss (HSSTV)}.}
	\label{real_urban_noniid_urban_Noniid_0.05_0.05}
\end{figure*}







==> fig_tex/fig_results_syn_05_01_00.tex <==
\begin{figure*}[t]
\centering
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/original/0.05_0.1_0_0.95_0.9/Orig_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.1_0_0.95_0.9/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/JSTV_2_0.1_1_/0.05_0.1_0_0.95_0.9/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/RSSUnTV_0.5_0.001_/0.05_0.1_0_0.95_0.9/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/lgsu/0.05_0.1_0/Recons1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/Reshaped_HTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/Reshaped_SSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/Reshaped_HSSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_1.eps}
            }
        \end{minipage}
    
\vspace{1mm}
        
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/original/0.05_0.1_0_0.95_0.9/Orig_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.1_0_0.95_0.9/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/JSTV_2_0.1_1_/0.05_0.1_0_0.95_0.9/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/RSSUnTV_0.5_0.001_/0.05_0.1_0_0.95_0.9/Recons_2.eps}
            }
        \end{minipage}        
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/lgsu/0.05_0.1_0/Recons2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/Reshaped_HTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/Reshaped_SSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/Reshaped_HSSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_2.eps}
            }
        \end{minipage}
    
\vspace{1mm}
        
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/original/0.05_0.1_0_0.95_0.9/Orig_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.1_0_0.95_0.9/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/JSTV_2_0.1_1_/0.05_0.1_0_0.95_0.9/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/RSSUnTV_0.5_0.001_/0.05_0.1_0_0.95_0.9/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/lgsu/0.05_0.1_0/Recons3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/Reshaped_HTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/Reshaped_SSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/Reshaped_HSSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_3.eps}
            }
        \end{minipage}
    
\vspace{1mm}
        
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/original/0.05_0.1_0_0.95_0.9/Orig_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.1_0_0.95_0.9/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/JSTV_2_0.1_1_/0.05_0.1_0_0.95_0.9/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/RSSUnTV_0.5_0.001_/0.05_0.1_0_0.95_0.9/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/lgsu/0.05_0.1_0/Recons4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/Reshaped_HTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/Reshaped_SSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth/Reshaped_HSSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_4.eps}
            }
        \end{minipage}
    
\vspace{1mm}
        
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (a)
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (b)
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (c)
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (d)
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (e)
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (f)
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (g)
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (h)
            }
        \end{minipage}

\caption{Unmixing results of abundance maps for the synthetic data in Case 4. (a): Original abundance maps. (b): CLSUnSAL \cite{iordache2013collaborative}. (c): JSTV~\cite{aggarwal2016hyperspectral}. (d): RSSUn-TV~\cite{wang2019row}. (e): LGSU~\cite{shen2022superpixel}. (f): Ours (HTV). (g): Ours (SSTV). (h): Ours (HSSTV).}
\label{synth_0.05_0.1_0}
\end{figure*}

% \begin{figure*}[h]
% \centering
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/original/0.05_0.1_0_0.95_0.9/Orig_1.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.1_0_0.95_0.9/Recons_1.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/JSTV_2_0.1_1_/0.05_0.1_0_0.95_0.9/Recons_1.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/RSSUnTV_0.5_0.001_/0.05_0.1_0_0.95_0.9/Recons_1.eps}
%             }
%         \end{minipage}

%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/original/0.05_0.1_0_0.95_0.9/Orig_2.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.1_0_0.95_0.9/Recons_2.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/JSTV_2_0.1_1_/0.05_0.1_0_0.95_0.9/Recons_2.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/RSSUnTV_0.5_0.001_/0.05_0.1_0_0.95_0.9/Recons_2.eps}
%             }
%         \end{minipage}
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/original/0.05_0.1_0_0.95_0.9/Orig_3.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.1_0_0.95_0.9/Recons_3.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/JSTV_2_0.1_1_/0.05_0.1_0_0.95_0.9/Recons_3.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/RSSUnTV_0.5_0.001_/0.05_0.1_0_0.95_0.9/Recons_3.eps}
%             }
%         \end{minipage}
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/original/0.05_0.1_0_0.95_0.9/Orig_4.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.1_0_0.95_0.9/Recons_4.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/JSTV_2_0.1_1_/0.05_0.1_0_0.95_0.9/Recons_4.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/RSSUnTV_0.5_0.001_/0.05_0.1_0_0.95_0.9/Recons_4.eps}
%             }
%         \end{minipage}
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (a)
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (b)
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (c)
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (d)
%             }
%         \end{minipage}
        
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.1_0_0.95_0.9/Recons_1.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_1.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_SSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_1.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HSSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_1.eps}
%             }
%         \end{minipage}
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.1_0_0.95_0.9/Recons_2.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_2.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_SSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_2.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HSSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_2.eps}
%             }
%         \end{minipage}
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.1_0_0.95_0.9/Recons_3.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_3.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_SSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_3.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HSSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_3.eps}
%             }
%         \end{minipage}
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.1_0_0.95_0.9/Recons_4.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_4.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_SSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_4.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HSSTV_2_2_1_/0.05_0.1_0_0.95_0.9/Recons_4.eps}
%             }
%         \end{minipage}
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (e)
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (f)
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (g)
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (h)
%             }
%         \end{minipage}

% \caption{Unmixing results of abundance maps in the synth data case with noise intensity of $\sigma=0.05, p_{Sp}=0.1, p_{St}=0.0$. (a): Original abundance maps. (b): CLSUnSAL. (c): JSTV. (d): RSSUn-TV. (e): EGU-Net. (f): Ours (HTV). (g): Ours (SSTV). (h): Ours (HSSTV).}
% \label{synth_0.05_0.1_0}
% \end{figure*}






==> fig_tex/fig_results_syn_05_05_05_colored.tex <==
\begin{figure*}[t]
	\color{blue}	
	\centering
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/original/0.05_0.05_0.05/Orig_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/CLSUnSAL/0.05_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/JSTV/0.05_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/RSSUn-TV/0.05_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/LGSU/0.05_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/UnDIP/0.05_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/EGU_Net/0.05_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/RDSWSU/0.05_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/MdLRR/0.05_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/Reshaped-HTV/0.05_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/Reshaped-SSTV/0.05_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/Reshaped-HSSTV/0.05_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/original/0.05_0.05_0.05/Orig_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/CLSUnSAL/0.05_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/JSTV/0.05_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/RSSUn-TV/0.05_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/LGSU/0.05_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/UnDIP/0.05_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/EGU_Net/0.05_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/RDSWSU/0.05_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/MdLRR/0.05_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/Reshaped-HTV/0.05_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/Reshaped-SSTV/0.05_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/Reshaped-HSSTV/0.05_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/original/0.05_0.05_0.05/Orig_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/CLSUnSAL/0.05_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/JSTV/0.05_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/RSSUn-TV/0.05_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/LGSU/0.05_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/UnDIP/0.05_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/EGU_Net/0.05_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/RDSWSU/0.05_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/MdLRR/0.05_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/Reshaped-HTV/0.05_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/Reshaped-SSTV/0.05_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/Reshaped-HSSTV/0.05_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/original/0.05_0.05_0.05/Orig_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/CLSUnSAL/0.05_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/JSTV/0.05_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/RSSUn-TV/0.05_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/LGSU/0.05_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/UnDIP/0.05_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/EGU_Net/0.05_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/RDSWSU/0.05_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/MdLRR/0.05_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/Reshaped-HTV/0.05_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/Reshaped-SSTV/0.05_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth/Reshaped-HSSTV/0.05_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(g)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			{(h)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			{(i)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(j)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(k)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(l)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			~
		}
	\end{minipage}
	
	\vspace{-1mm}
	
	\caption{Unmixing results of abundance maps for the \textit{Synth 2} experiments in Case 5. (a): Original abundance maps. (b): CLSUnSAL~\cite{iordache2014collaborative}. (c): JSTV~\cite{aggarwal2016hyperspectral}. (d): RSSUn-TV~\cite{wang2019row}. (e): LGSU~\cite{shen2022superpixel}. (f): UnDIP~\cite{UnDIP_RastiB_2022}. (g): EGU-Net~\cite{hong2022endmember}. (h): RDSWSU~\cite{rs_Deng_RobustDual_2023}. (i): MdLRR~\cite{MDLRR_WuLing_2023}. (j): \textbf{\Ourss (HTV)}. (k): \textbf{\Ourss (SSTV)}. (l): \textbf{\Ourss (HSSTV)}.}
	\label{synth_0.05_0.05_0.05}
\end{figure*}








==> fig_tex/fig_results_syn_Legendre200_noniid_01_01_colored.tex <==

\begin{figure*}[t]
	\color{blue}
	\centering
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/original/Noniid_0.05_0.05/Orig_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/CLSUnSAL/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/JSTV/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/RSSUn-TV/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/LGSU/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/UnDIP/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/EGU_Net/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/RDSWSU/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/MdLRR/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/Reshaped-HTV/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/Reshaped-SSTV/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/Reshaped-HSSTV/Noniid_0.05_0.05/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/original/Noniid_0.05_0.05/Orig_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/CLSUnSAL/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/JSTV/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/RSSUn-TV/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}        
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/LGSU/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/UnDIP/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/EGU_Net/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/RDSWSU/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/MdLRR/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/Reshaped-HTV/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/Reshaped-SSTV/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/Reshaped-HSSTV/Noniid_0.05_0.05/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/original/Noniid_0.05_0.05/Orig_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/CLSUnSAL/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/JSTV/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/RSSUn-TV/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/LGSU/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/UnDIP/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/EGU_Net/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/RDSWSU/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/MdLRR/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/Reshaped-HTV/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/Reshaped-SSTV/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/Reshaped-HSSTV/Noniid_0.05_0.05/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/original/Noniid_0.05_0.05/Orig_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/CLSUnSAL/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/JSTV/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/RSSUn-TV/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/LGSU/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/UnDIP/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/EGU_Net/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/RDSWSU/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/MdLRR/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/Reshaped-HTV/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/Reshaped-SSTV/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre_200_noniid/Reshaped-HSSTV/Noniid_0.05_0.05/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(g)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			{(h)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			{(i)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(j)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(k)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(l)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			~
		}
	\end{minipage}
	
	\vspace{-1mm}
	
	\caption{Unmixing results of abundance maps for the \textit{Synth 3} experiments in Case 8. (a): Original abundance maps. (b): CLSUnSAL~\cite{iordache2014collaborative}. (c): JSTV~\cite{aggarwal2016hyperspectral}. (d): RSSUn-TV~\cite{wang2019row}. (e): LGSU~\cite{shen2022superpixel}. (f): UnDIP~\cite{UnDIP_RastiB_2022}. (g): EGU-Net~\cite{hong2022endmember}. (h): RDSWSU~\cite{rs_Deng_RobustDual_2023}. (i): MdLRR~\cite{MDLRR_WuLing_2023}. (j): \textbf{\Ourss (HTV)}. (k): \textbf{\Ourss (SSTV)}. (l): \textbf{\Ourss (HSSTV)}.}
	\label{fig:synth_legendre_200_noniid_Noniid_0.05_0.05}
\end{figure*}



==> fig_tex/fig_results_syn_Legendre_01_00_00_colored.tex <==

\begin{figure*}[t]
	\color{blue}
	\centering
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/original/0.1_0_0/Orig_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/CLSUnSAL/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/JSTV/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/RSSUn-TV/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/LGSU/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/UnDIP/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/EGU_Net/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/RDSWSU/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/MdLRR/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HTV/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-SSTV/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HSSTV/0.1_0_0/Recons_1.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/original/0.1_0_0/Orig_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/CLSUnSAL/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/JSTV/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/RSSUn-TV/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}        
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/LGSU/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/UnDIP/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/EGU_Net/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/RDSWSU/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/MdLRR/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HTV/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-SSTV/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HSSTV/0.1_0_0/Recons_2.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/original/0.1_0_0/Orig_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/CLSUnSAL/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/JSTV/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/RSSUn-TV/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/LGSU/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/UnDIP/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/EGU_Net/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/RDSWSU/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/MdLRR/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HTV/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-SSTV/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HSSTV/0.1_0_0/Recons_3.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\vspace{1mm}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/original/0.1_0_0/Orig_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/CLSUnSAL/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/JSTV/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/RSSUn-TV/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/LGSU/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/UnDIP/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/EGU_Net/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/RDSWSU/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/MdLRR/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HTV/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-SSTV/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HSSTV/0.1_0_0/Recons_4.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			\includegraphics[height = 40pt]{./fig/colorbar_20.png}
		}
	\end{minipage}
	
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(d)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			(g)
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			{(h)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			{(i)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(j)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(k)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.075\hsize}
		\centerline{
			\textbf{(l)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.02\hsize}
		\centerline{
			~
		}
	\end{minipage}
	
	\vspace{-1mm}
	
	\caption{Unmixing results of abundance maps for the \textit{Synth 1} experiments in Case 2. (a): Original abundance maps. (b): CLSUnSAL~\cite{iordache2014collaborative}. (c): JSTV~\cite{aggarwal2016hyperspectral}. (d): RSSUn-TV~\cite{wang2019row}. (e): LGSU~\cite{shen2022superpixel}. (f): UnDIP~\cite{UnDIP_RastiB_2022}. (g): EGU-Net~\cite{hong2022endmember}. (h): RDSWSU~\cite{rs_Deng_RobustDual_2023}. (i): MdLRR~\cite{MDLRR_WuLing_2023}. (j): \textbf{\Ourss (HTV)}. (k): \textbf{\Ourss (SSTV)}. (l): \textbf{\Ourss (HSSTV)}.}
	\label{fig:synth_legendre_0.1_0_0}
\end{figure*}



==> fig_tex/fig_results_syn_Legendre_05_01_00.tex <==
\begin{figure*}[!h]
\centering
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/original/0.05_0.1_0/Orig_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/CLSUnSAL/0.05_0.1_0/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/JSTV/0.05_0.1_0/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/RSSUn-TV/0.05_0.1_0/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/LGSU/0.05_0.1_0/Recons_1.eps}
            }
        \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
	    	\centerline{
	    		\includegraphics[height = 40pt]{./fig/synth_legendre/UnDIP/0.05_0.1_0/Recons_1.eps}
	    	}
	    \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
	    \centerline{
	    	\includegraphics[height = 40pt]{./fig/synth_legendre/EGU_Net/0.05_0.1_0/Recons_1.eps}
	    }
	    \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
	    \centerline{
	    	\includegraphics[height = 40pt]{./fig/synth_legendre/RDSWSU/0.05_0.1_0/Recons_1.eps}
	    }
	    \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
		    \centerline{
		    	\includegraphics[height = 40pt]{./fig/synth_legendre/MdLRR/0.05_0.1_0/Recons_1.eps}
		    }
	    \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HTV/0.05_0.1_0/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-SSTV/0.05_0.1_0/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HSSTV/0.05_0.1_0/Recons_1.eps}
            }
        \end{minipage}
	    \begin{minipage}[t]{0.02\hsize}
	    	\centerline{
	    		\includegraphics[height = 40pt]{./fig/colorbar_20.png}
	    	}
	    \end{minipage}
    
    \vspace{1mm}
        
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/original/0.05_0.1_0/Orig_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/CLSUnSAL/0.05_0.1_0/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/JSTV/0.05_0.1_0/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/RSSUn-TV/0.05_0.1_0/Recons_2.eps}
            }
        \end{minipage}        
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/LGSU/0.05_0.1_0/Recons_2.eps}
            }
        \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
	    	\centerline{
	    		\includegraphics[height = 40pt]{./fig/synth_legendre/UnDIP/0.05_0.1_0/Recons_2.eps}
	    	}
	    \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
	    \centerline{
	    	\includegraphics[height = 40pt]{./fig/synth_legendre/EGU_Net/0.05_0.1_0/Recons_2.eps}
	    }
	    \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
	    \centerline{
	    	\includegraphics[height = 40pt]{./fig/synth_legendre/RDSWSU/0.05_0.1_0/Recons_2.eps}
	    }
	    \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
		    \centerline{
		    	\includegraphics[height = 40pt]{./fig/synth_legendre/MdLRR/0.05_0.1_0/Recons_2.eps}
		    }
	    \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HTV/0.05_0.1_0/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-SSTV/0.05_0.1_0/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HSSTV/0.05_0.1_0/Recons_2.eps}
            }
        \end{minipage}
	    \begin{minipage}[t]{0.02\hsize}
	    	\centerline{
	    		\includegraphics[height = 40pt]{./fig/colorbar_20.png}
	    	}
	    \end{minipage}
    
\vspace{1mm}
        
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/original/0.05_0.1_0/Orig_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/CLSUnSAL/0.05_0.1_0/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/JSTV/0.05_0.1_0/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/RSSUn-TV/0.05_0.1_0/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/LGSU/0.05_0.1_0/Recons_3.eps}
            }
        \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
	    	\centerline{
	    		\includegraphics[height = 40pt]{./fig/synth_legendre/UnDIP/0.05_0.1_0/Recons_3.eps}
	    	}
	    \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
	    \centerline{
	    	\includegraphics[height = 40pt]{./fig/synth_legendre/EGU_Net/0.05_0.1_0/Recons_3.eps}
	    }
	    \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
	    \centerline{
	    	\includegraphics[height = 40pt]{./fig/synth_legendre/RDSWSU/0.05_0.1_0/Recons_3.eps}
	    }
	    \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
		    \centerline{
		    	\includegraphics[height = 40pt]{./fig/synth_legendre/MdLRR/0.05_0.1_0/Recons_3.eps}
		    }
	    \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HTV/0.05_0.1_0/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-SSTV/0.05_0.1_0/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HSSTV/0.05_0.1_0/Recons_3.eps}
            }
        \end{minipage}
	    \begin{minipage}[t]{0.02\hsize}
	    	\centerline{
	    		\includegraphics[height = 40pt]{./fig/colorbar_20.png}
	    	}
	    \end{minipage}
    
\vspace{1mm}
        
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/original/0.05_0.1_0/Orig_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/CLSUnSAL/0.05_0.1_0/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/JSTV/0.05_0.1_0/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/RSSUn-TV/0.05_0.1_0/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/LGSU/0.05_0.1_0/Recons_4.eps}
            }
        \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
	    	\centerline{
	    		\includegraphics[height = 40pt]{./fig/synth_legendre/UnDIP/0.05_0.1_0/Recons_4.eps}
	    	}
	    \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
	    \centerline{
	    	\includegraphics[height = 40pt]{./fig/synth_legendre/EGU_Net/0.05_0.1_0/Recons_4.eps}
	    }
	    \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
	    \centerline{
	    	\includegraphics[height = 40pt]{./fig/synth_legendre/RDSWSU/0.05_0.1_0/Recons_4.eps}
	    }
	    \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
		    \centerline{
		    	\includegraphics[height = 40pt]{./fig/synth_legendre/MdLRR/0.05_0.1_0/Recons_4.eps}
		    }
	    \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HTV/0.05_0.1_0/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-SSTV/0.05_0.1_0/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            \includegraphics[height = 40pt]{./fig/synth_legendre/Reshaped-HSSTV/0.05_0.1_0/Recons_4.eps}
            }
        \end{minipage}
	    \begin{minipage}[t]{0.02\hsize}
	    	\centerline{
	    		\includegraphics[height = 40pt]{./fig/colorbar_20.png}
	    	}
	    \end{minipage}
        
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            (a)
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            (b)
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            (c)
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            (d)
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            (e)
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            (f)
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            (g)
            }
        \end{minipage}
        \begin{minipage}[t]{0.075\hsize}
            \centerline{
            {(h)}
            }
        \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
	    	\centerline{
	    		{(i)}
	    	}
	    \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
		    \centerline{
		    	\textbf{(j)}
		    }
	    \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
	    \centerline{
	    	\textbf{(k)}
	    }
	    \end{minipage}
	    \begin{minipage}[t]{0.075\hsize}
	    \centerline{
	    	\textbf{(l)}
	    }
	    \end{minipage}
	    \begin{minipage}[t]{0.02\hsize}
	    	\centerline{
	    		~
	    	}
	    \end{minipage}
	    
	    \vspace{-1mm}

\caption{Unmixing results of abundance maps for the \textit{Synth 1} experiments in Case 4. (a): Original abundance maps. (b): CLSUnSAL~\cite{iordache2014collaborative}. (c): JSTV~\cite{aggarwal2016hyperspectral}. (d): RSSUn-TV~\cite{wang2019row}. (e): LGSU~\cite{shen2022superpixel}. (f): UnDIP~\cite{UnDIP_RastiB_2022}. (g): EGU-Net~\cite{hong2022endmember}. (h): RDSWSU~\cite{rs_Deng_RobustDual_2023}. (i): MdLRR~\cite{MDLRR_WuLing_2023}. (j): \textbf{\Ourss (HTV)}. (k): \textbf{\Ourss (SSTV)}. (l): \textbf{\Ourss (HSSTV)}.}
\label{fig:synth_legendre_0.05_0.1_0}
\end{figure*}








==> fig_tex/fig_results_syn_Legendre_05_05_05.tex <==
\begin{figure*}[!h]
\centering
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/original/0.05_0.05_0.05_0.95_0.9/Orig_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/CLSUnSAL_0.0003/0.05_0.05_0.05_0.95_0.9/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/JSTV_2_0.1_1_/0.05_0.05_0.05_0.95_0.9/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/RSSUnTV_0.5_0.001_/0.05_0.05_0.05_0.95_0.9/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/lgsu/0.05_0.05_0.05_0.95_0.9/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped_HTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped_SSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_1.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped_HSSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_1.eps}
            }
        \end{minipage}
    
\vspace{1mm}
        
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/original/0.05_0.05_0.05_0.95_0.9/Orig_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/CLSUnSAL_0.0003/0.05_0.05_0.05_0.95_0.9/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/JSTV_2_0.1_1_/0.05_0.05_0.05_0.95_0.9/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/RSSUnTV_0.5_0.001_/0.05_0.05_0.05_0.95_0.9/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/lgsu/0.05_0.05_0.05_0.95_0.9/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped_HTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped_SSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_2.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped_HSSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_2.eps}
            }
        \end{minipage}
    
\vspace{1mm}
        
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/original/0.05_0.05_0.05_0.95_0.9/Orig_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/CLSUnSAL_0.0003/0.05_0.05_0.05_0.95_0.9/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/JSTV_2_0.1_1_/0.05_0.05_0.05_0.95_0.9/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/RSSUnTV_0.5_0.001_/0.05_0.05_0.05_0.95_0.9/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/lgsu/0.05_0.05_0.05_0.95_0.9/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped_HTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped_SSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_3.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped_HSSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_3.eps}
            }
        \end{minipage}
    
\vspace{1mm}
        
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/original/0.05_0.05_0.05_0.95_0.9/Orig_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/CLSUnSAL_0.0003/0.05_0.05_0.05_0.95_0.9/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/JSTV_2_0.1_1_/0.05_0.05_0.05_0.95_0.9/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/RSSUnTV_0.5_0.001_/0.05_0.05_0.05_0.95_0.9/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/lgsu/0.05_0.05_0.05_0.95_0.9/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped_HTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped_SSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_4.eps}
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            \includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped_HSSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_4.eps}
            }
        \end{minipage}
    
\vspace{1mm}
        
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (a)
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (b)
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (c)
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (d)
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (e)
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (f)
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (g)
            }
        \end{minipage}
        \begin{minipage}[t]{0.11\hsize}
            \centerline{
            (h)
            }
        \end{minipage}

\caption{Unmixing results of abundance maps for the synthetic data in Case 5. (a): Original abundance maps. (b): CLSUnSAL \cite{iordache2013collaborative}. (c): JSTV~\cite{aggarwal2016hyperspectral}. (d): RSSUn-TV~\cite{wang2019row}. (e): LGSU~\cite{shen2022superpixel}. (f): Ours (HTV). (g): Ours (SSTV). (h): Ours (HSSTV).}
\label{fig:synth_legendre_0.05_0.05_0.05}
\end{figure*}

% \begin{figure*}[h]
% \centering
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/original/0.05_0.05_0.05_0.95_0.9/Orig_1.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.05_0.05_0.95_0.9/Recons_1.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/JSTV_2_0.1_1_/0.05_0.05_0.05_0.95_0.9/Recons_1.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/RSSUnTV_0.5_0.001_/0.05_0.05_0.05_0.95_0.9/Recons_1.eps}
%             }
%         \end{minipage}

%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/original/0.05_0.05_0.05_0.95_0.9/Orig_2.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.05_0.05_0.95_0.9/Recons_2.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/JSTV_2_0.1_1_/0.05_0.05_0.05_0.95_0.9/Recons_2.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/RSSUnTV_0.5_0.001_/0.05_0.05_0.05_0.95_0.9/Recons_2.eps}
%             }
%         \end{minipage}
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/original/0.05_0.05_0.05_0.95_0.9/Orig_3.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.05_0.05_0.95_0.9/Recons_3.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/JSTV_2_0.1_1_/0.05_0.05_0.05_0.95_0.9/Recons_3.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/RSSUnTV_0.5_0.001_/0.05_0.05_0.05_0.95_0.9/Recons_3.eps}
%             }
%         \end{minipage}
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/original/0.05_0.05_0.05_0.95_0.9/Orig_4.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.05_0.05_0.95_0.9/Recons_4.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/JSTV_2_0.1_1_/0.05_0.05_0.05_0.95_0.9/Recons_4.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/RSSUnTV_0.5_0.001_/0.05_0.05_0.05_0.95_0.9/Recons_4.eps}
%             }
%         \end{minipage}
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (a)
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (b)
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (c)
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (d)
%             }
%         \end{minipage}
        
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.05_0.05_0.95_0.9/Recons_1.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_1.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_SSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_1.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HSSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_1.eps}
%             }
%         \end{minipage}
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.05_0.05_0.95_0.9/Recons_2.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_2.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_SSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_2.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HSSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_2.eps}
%             }
%         \end{minipage}
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.05_0.05_0.95_0.9/Recons_3.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_3.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_SSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_3.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HSSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_3.eps}
%             }
%         \end{minipage}
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/CLSUnSAL_0.0003/0.05_0.05_0.05_0.95_0.9/Recons_4.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_4.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_SSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_4.eps}
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             \includegraphics[width=\hsize]{./fig/synth/Reshaped_HSSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_4.eps}
%             }
%         \end{minipage}
        
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (e)
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (f)
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (g)
%             }
%         \end{minipage}
%         \begin{minipage}[t]{0.18\hsize}
%             \centerline{
%             (h)
%             }
%         \end{minipage}

% \caption{Unmixing results of abundance maps in the synth data case with noise intensity of $\sigma=0.05, p_{Sp}=0.1, p_{St}=0.0$. (a): Original abundance maps. (b): CLSUnSAL. (c): JSTV. (d): RSSUn-TV. (e): EGU-Net. (f): Ours (HTV). (g): Ours (SSTV). (h): Ours (HSSTV).}
% \label{synth_0.05_0.05_0.05}
% \end{figure*}





==> fig_tex/fig_synth_HSI_05_01_00.tex <==
\begin{figure*}[t]
\centering
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        \includegraphics[width=\hsize]{./fig/synth/recons_0.05_0.1_0/Orig_HSI.eps}
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        \includegraphics[width=\hsize]{./fig/synth/recons_0.05_0.1_0/Noisy_HSI.eps}
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        \includegraphics[width=\hsize]{./fig/synth/recons_0.05_0.1_0/clsunsal.eps}
        }
    \end{minipage}
 \begin{minipage}[t]{0.10\hsize}
  \centerline{
	    	\includegraphics[width=\hsize]{./fig/synth/recons_0.05_0.1_0/jstv.eps}
  }
	\end{minipage}       
	\begin{minipage}[t]{0.10\hsize}
	\centerline{
		\includegraphics[width=\hsize]{./fig/synth/recons_0.05_0.1_0/rssuntv.eps}
	}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
	\centerline{
		\includegraphics[width=\hsize]{./fig/synth/lgsu/0.05_0.1_0/ReconsHSI.eps}
	}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/recons_0.05_0.1_0/htv.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/recons_0.05_0.1_0/sstv.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/recons_0.05_0.1_0/hsstv.eps}
		}
	\end{minipage}
     
     
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (a)
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (b)
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (c)
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (d)
        }
    \end{minipage}        
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (e)
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (f)
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (g)
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (h)
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (i)
        }
    \end{minipage}
        

\caption{HS image results obtained by mixing endmembers and estimated abundances for the synthetic data in Case 4. (a): Original HS image. (b): Noisy image. (c): CLSUnSAL \cite{iordache2013collaborative}.  (d): JSTV~\cite{aggarwal2016hyperspectral}. (e): RSSUn-TV~\cite{wang2019row}. (f): LGSU~\cite{shen2022superpixel}. (g): Ours (HTV). (h): Ours (SSTV). (i): Ours (HSSTV).}
\label{synth_HSI_0.05_0.1_0}
\end{figure*}



==> fig_tex/fig_synth_HSI_05_05_05_colored.tex <==
\begin{figure*}[!h]
	\color{blue}
	\centering
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/original/0.05_0.05_0.05/Orig_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/original/0.05_0.05_0.05/Noisy_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/CLSUnSAL/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}    
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/JSTV/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}        
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/RSSUn-TV/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}        
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/LGSU/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/UnDIP/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/EGU_Net/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/RDSWSU/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/MdLRR/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/Reshaped-HTV/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/Reshaped-SSTV/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth/Reshaped-HSSTV/0.05_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(d)
		}
	\end{minipage}        
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(g)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(h)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			{(i)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			{(j)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(k)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(l)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(m)}
		}
	\end{minipage}
	
	
	\vspace{-1mm}
	
	\caption{Reconstructed HS image results for
		the \textit{Synth 2} experiments in Case 5. (a): Original HS image. (b): Noisy image. (c): CLSUnSAL \cite{iordache2014collaborative}.  (d): JSTV~\cite{aggarwal2016hyperspectral}. (e): RSSUn-TV~\cite{wang2019row}. (f): LGSU~\cite{shen2022superpixel}. (g): UnDIP~\cite{UnDIP_RastiB_2022}. (h): EGU-Net~\cite{hong2022endmember}. (i): RDSWSU~\cite{rs_Deng_RobustDual_2023}. (j): MdLRR~\cite{MDLRR_WuLing_2023}. (k): \textbf{\Ourss (HTV)}. (l): \textbf{\Ourss (SSTV)}. (m): \textbf{\Ourss (HSSTV)}.}
	\label{synth_HSI_0.05_0.05_0.05}
\end{figure*}




==> fig_tex/fig_synth_Legendre200_noniid_HSI_01_01_colored.tex <==
\begin{figure*}[!h]
	\color{blue}
	\centering
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre_200_noniid/original/Noniid_0.05_0.05/Orig_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre_200_noniid/original/Noniid_0.05_0.05/Noisy_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre_200_noniid/CLSUnSAL/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre_200_noniid/JSTV/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}       
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre_200_noniid/RSSUn-TV/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre_200_noniid/LGSU/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre_200_noniid/UnDIP/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre_200_noniid/EGU_Net/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre_200_noniid/RDSWSU/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre_200_noniid/MdLRR/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre_200_noniid/Reshaped-HTV/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre_200_noniid/Reshaped-SSTV/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre_200_noniid/Reshaped-HSSTV/Noniid_0.05_0.05/Recons_HSI.eps}
		}
	\end{minipage}
	
	
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(d)
		}
	\end{minipage}        
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(g)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(h)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			{(i)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			{(j)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(k)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(l)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(m)}
		}
	\end{minipage}
	
	\vspace{-1mm}
	
	
	\caption{Reconstructed HS image results for the \textit{Synth 3} experiments in Case 8.  (a): Original HS image. (b): Noisy image. (c): CLSUnSAL \cite{iordache2014collaborative}.  (d): JSTV~\cite{aggarwal2016hyperspectral}. (e): RSSUn-TV~\cite{wang2019row}. (f): LGSU~\cite{shen2022superpixel}. (g): UnDIP~\cite{UnDIP_RastiB_2022}. (h): EGU-Net~\cite{hong2022endmember}. (i): RDSWSU~\cite{rs_Deng_RobustDual_2023}. (j): MdLRR~\cite{MDLRR_WuLing_2023}. (k): \textbf{\Ourss (HTV)}. (l): \textbf{\Ourss (SSTV)}. (m): \textbf{\Ourss (HSSTV)}.}
	\label{fig:synth_legendre_200_noniid200_noniid_HSI_0.1_0.1}
\end{figure*}



==> fig_tex/fig_synth_Legendre_HSI_01_00_00_colored.tex <==
\begin{figure*}[!h]
	\color{blue}
	\centering
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/original/0.1_0_0/Orig_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/original/0.1_0_0/Noisy_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/CLSUnSAL/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/JSTV/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}       
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/RSSUn-TV/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/LGSU/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/UnDIP/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/EGU_Net/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/RDSWSU/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/MdLRR/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped-HTV/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped-SSTV/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped-HSSTV/0.1_0_0/Recons_HSI.eps}
		}
	\end{minipage}
	
	
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(a)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(b)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(c)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(d)
		}
	\end{minipage}        
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(e)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(f)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(g)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			(h)
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			{(i)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			{(j)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(k)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(l)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(m)}
		}
	\end{minipage}
	
	\vspace{-1mm}
	
	
	\caption{Reconstructed HS image results for the \textit{Synth 1} experiments in Case 2.  (a): Original HS image. (b): Noisy image. (c): CLSUnSAL \cite{iordache2014collaborative}.  (d): JSTV~\cite{aggarwal2016hyperspectral}. (e): RSSUn-TV~\cite{wang2019row}. (f): LGSU~\cite{shen2022superpixel}. (g): UnDIP~\cite{UnDIP_RastiB_2022}. (h): EGU-Net~\cite{hong2022endmember}. (i): RDSWSU~\cite{rs_Deng_RobustDual_2023}. (j): MdLRR~\cite{MDLRR_WuLing_2023}. (k): \textbf{\Ourss (HTV)}. (l): \textbf{\Ourss (SSTV)}. (m): \textbf{\Ourss (HSSTV)}.}
	\label{fig:synth_legendre_HSI_0.1_0_0}
\end{figure*}



==> fig_tex/fig_synth_Legendre_HSI_05_01_00.tex <==
\begin{figure*}[!h]
\centering
    \begin{minipage}[t]{0.07\hsize}
        \centerline{
        \includegraphics[width=\hsize]{./fig/synth_legendre/original/0.05_0.1_0/Orig_HSI.eps}
        }
    \end{minipage}
    \begin{minipage}[t]{0.07\hsize}
        \centerline{
        \includegraphics[width=\hsize]{./fig/synth_legendre/original/0.05_0.1_0/Noisy_HSI.eps}
        }
    \end{minipage}
    \begin{minipage}[t]{0.07\hsize}
        \centerline{
        \includegraphics[width=\hsize]{./fig/synth_legendre/CLSUnSAL/0.05_0.1_0/Recons_HSI.eps}
        }
    \end{minipage}
 \begin{minipage}[t]{0.07\hsize}
  \centerline{
	    	\includegraphics[width=\hsize]{./fig/synth_legendre/JSTV/0.05_0.1_0/Recons_HSI.eps}
  }
	\end{minipage}       
	\begin{minipage}[t]{0.07\hsize}
	\centerline{
		\includegraphics[width=\hsize]{./fig/synth_legendre/RSSUn-TV/0.05_0.1_0/Recons_HSI.eps}
	}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
	\centerline{
		\includegraphics[width=\hsize]{./fig/synth_legendre/LGSU/0.05_0.1_0/Recons_HSI.eps}
	}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/UnDIP/0.05_0.1_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
	\centerline{
		\includegraphics[width=\hsize]{./fig/synth_legendre/EGU_Net/0.05_0.1_0/Recons_HSI.eps}
	}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
	\centerline{
		\includegraphics[width=\hsize]{./fig/synth_legendre/RDSWSU/0.05_0.1_0/Recons_HSI.eps}
	}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/MdLRR/0.05_0.1_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped-HTV/0.05_0.1_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped-SSTV/0.05_0.1_0/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped-HSSTV/0.05_0.1_0/Recons_HSI.eps}
		}
	\end{minipage}
     
     
    \begin{minipage}[t]{0.07\hsize}
        \centerline{
        (a)
        }
    \end{minipage}
    \begin{minipage}[t]{0.07\hsize}
        \centerline{
        (b)
        }
    \end{minipage}
    \begin{minipage}[t]{0.07\hsize}
        \centerline{
        (c)
        }
    \end{minipage}
    \begin{minipage}[t]{0.07\hsize}
        \centerline{
        (d)
        }
    \end{minipage}        
    \begin{minipage}[t]{0.07\hsize}
        \centerline{
        (e)
        }
    \end{minipage}
    \begin{minipage}[t]{0.07\hsize}
        \centerline{
        (f)
        }
    \end{minipage}
    \begin{minipage}[t]{0.07\hsize}
        \centerline{
        (g)
        }
    \end{minipage}
    \begin{minipage}[t]{0.07\hsize}
        \centerline{
        (h)
        }
    \end{minipage}
    \begin{minipage}[t]{0.07\hsize}
        \centerline{
        {(i)}
        }
    \end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			{(j)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
		\centerline{
			\textbf{(k)}
		}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
	\centerline{
		\textbf{(l)}
	}
	\end{minipage}
	\begin{minipage}[t]{0.07\hsize}
	\centerline{
		\textbf{(m)}
	}
	\end{minipage}
        
        \vspace{-1mm}

\caption{Reconstructed HS image results for the \textit{Synth 1} experiments in Case 4.  (a): Original HS image. (b): Noisy image. (c): CLSUnSAL \cite{iordache2014collaborative}.  (d): JSTV~\cite{aggarwal2016hyperspectral}. (e): RSSUn-TV~\cite{wang2019row}. (f): LGSU~\cite{shen2022superpixel}. (g): UnDIP~\cite{UnDIP_RastiB_2022}. (h): EGU-Net~\cite{hong2022endmember}. (i): RDSWSU~\cite{rs_Deng_RobustDual_2023}. (j): MdLRR~\cite{MDLRR_WuLing_2023}. (k): \textbf{\Ourss (HTV)}. (l): \textbf{\Ourss (SSTV)}. (m): \textbf{\Ourss (HSSTV)}.}
\label{fig:synth_legendre_HSI_0.05_0.1_0}
\end{figure*}



==> fig_tex/fig_synth_Legendre_HSI_05_05_05.tex <==
\begin{figure*}[t]
\centering
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        \includegraphics[width=\hsize]{./fig/synth_legendre/original/0.05_0.05_0.05_0.95_0.9/Orig_HSI.eps}
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        \includegraphics[width=\hsize]{./fig/synth_legendre/original/0.05_0.05_0.05_0.95_0.9/Noisy_HSI.eps}
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        \includegraphics[width=\hsize]{./fig/synth_legendre/CLSUnSAL_0.0003/0.05_0.05_0.05_0.95_0.9/Recons_HSI.eps}
        }
    \end{minipage}    
    \begin{minipage}[t]{0.10\hsize}
    	\centerline{
    		\includegraphics[width=\hsize]{./fig/synth_legendre/JSTV_2_0.1_1_/0.05_0.05_0.05_0.95_0.9/Recons_HSI.eps}
    	}
    \end{minipage}        
    \begin{minipage}[t]{0.10\hsize}
    	\centerline{
    		\includegraphics[width=\hsize]{./fig/synth_legendre/RSSUnTV_0.5_0.001_/0.05_0.05_0.05_0.95_0.9/Recons_HSI.eps}
    	}
    \end{minipage}        
    \begin{minipage}[t]{0.10\hsize}
    	\centerline{
    		\includegraphics[width=\hsize]{./fig/synth_legendre/lgsu/0.05_0.05_0.05_0.95_0.9/Recons_HSI.eps}
    	}
    \end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped_HTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped_SSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_HSI.eps}
		}
	\end{minipage}
	\begin{minipage}[t]{0.10\hsize}
		\centerline{
			\includegraphics[width=\hsize]{./fig/synth_legendre/Reshaped_HSSTV_2_2_1_/0.05_0.05_0.05_0.95_0.9/Recons_HSI.eps}
		}
	\end{minipage}
        
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (a)
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (b)
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (c)
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (d)
        }
    \end{minipage}        
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (e)
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (f)
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (g)
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (h)
        }
    \end{minipage}
    \begin{minipage}[t]{0.10\hsize}
        \centerline{
        (i)
        }
    \end{minipage}
        

\caption{HS image results obtained by mixing endmembers and estimated abundances for
the synthetic data in Case 5. (a): Original HS image. (b): Noisy image. (c): CLSUnSAL \cite{iordache2013collaborative}.  (d): JSTV~\cite{aggarwal2016hyperspectral}. (e): RSSUn-TV~\cite{wang2019row}. (f): LGSU~\cite{shen2022superpixel}. (g): Ours (HTV). (h): Ours (SSTV). (i): Ours (HSSTV).}
\label{fig:synth_legendre_HSI_0.05_0.05_0.05}
\end{figure*}




==> tab_tex/tab_cases.tex <==

\begin{table}[t]
	\caption{Noise Taken Into Account by Each Method.}
	\vspace{-1mm}
	\label{tab:noise}
	\centering
	\color{red}
	\begin{tabular}{cccc}
		\toprule
		Methods & Gaussian noise & Sparse noise & Stripe noise \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-4}
		\vspace{0.5mm}
		CLSUnSAL~\cite{iordache2014collaborative} & \checkmark & - & - \\
		\vspace{0.5mm}
		JSTV~\cite{aggarwal2016hyperspectral} & \checkmark & \checkmark & - \\
		\vspace{0.5mm}
		RSSUn-TV~\cite{wang2019row} & \checkmark & - & - \\
		\vspace{0.5mm}
		LGSU~\cite{shen2022superpixel} & \checkmark & - & - \\
		\vspace{0.5mm}
		UnDIP~\cite{UnDIP_RastiB_2022} & \checkmark & - & - \\
		\vspace{0.5mm}
		EGU-Net~\cite{hong2022endmember} & \checkmark & - & - \\
		\vspace{0.5mm}
		RDSWSU~\cite{rs_Deng_RobustDual_2023} & \checkmark & - & - \\
		\vspace{0.5mm}
		MdLRR~\cite{MDLRR_WuLing_2023} & \checkmark & - & - \\
		%		\cmidrule(lr){1-4}
		\textbf{\Ourss (Ours)} & \checkmark &\checkmark&\checkmark\\
		\bottomrule
	\end{tabular}
	\color{black}
\end{table}


==> tab_tex/tab_computational_compexity_colored.tex <==
\begin{table}[t]
	\color{blue}
	\caption{Computational Complexities of Each Operation.}
	\label{tab:computational_complexity}
	\vspace{-1mm}
	\centering
	\begin{tabular}{cc}
		\toprule
		Operations &  $O$-notation \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-2}
		$\MatEndmember \MatAbun$, 
		($\MatEndmember \in \SetRealNum^{\NumBand \times \NumEndmember}$ 
		and $\MatAbun \in \SetRealNum^{\NumEndmember \times \NumPixel}$) 
		& $O(\NumPixel \NumEndmember \NumBand)$ \\
		
		\addlinespace[5pt]
		$\OpeDiff{\MatAbun}$, 
		($\MatAbun \in \SetRealNum^{\NumEndmember \times \NumPixel}$) 
		& $O(\NumPixel \NumEndmember)$ \\
		
		\addlinespace[5pt]
		$\OpeDiff{\MatHSIGeneral}$, 
		($\MatHSIGeneral \in \SetRealNum^{\NumBand \times \NumPixel}$) 
		& $O(\NumPixel \NumBand)$ \\
		
		\addlinespace[5pt]
		$\DiffHSIReg(\MatHSIGeneral)$, 
		$\begin{cases}
			\DiffHSIReg = \OpeDiffSymb, \: (\MatHSIGeneral \in \SetRealNum^{\NumBand \times \NumPixel}) \\
			\DiffHSIReg = \OpeDiffSymb \circ \OpeDiffbSymb, \: (\MatHSIGeneral \in \SetRealNum^{\NumBand \times \NumPixel}) \\
			\DiffHSIReg = \OpeDiffHSSTVSymb_{\ParamHSSTV}, \: (\MatHSIGeneral \in \SetRealNum^{\NumBand \times \NumPixel})
		\end{cases}$
		& $O(\NumPixel \NumBand)$ \\
		
		\addlinespace[5pt]
		$\textrm{prox}_{\gamma_1 \FuncIndSymb{\SetNNOrthantAbun}}(\MatAbun)$, ($\MatAbun \in \SetRealNum^{\NumEndmember \times \NumPixel}$) 
		& $O(\NumPixel \NumEndmember)$ \\
		
		\addlinespace[5pt]
		$\textrm{prox}_{\gamma_2 \iota_{\SetConsSpar}}(\MatSpar)$, 
		($\MatSpar \in \SetRealNum^{\NumBand \times \NumPixel}$) 
		& $O(\NumPixel \NumBand \log \NumPixel \NumBand)$ \\
		
		\addlinespace[5pt]
		$\textrm{prox}_{\gamma_3\lambda_3\|\cdot\|_1}(\MatStripe)$,
		($\MatStripe \in \SetRealNum^{\NumBand \times \NumPixel}$) 
		& $O(\NumPixel \NumBand)$ \\
		
		\addlinespace[5pt]
		$\textrm{prox}_{\tfrac{1}{\gamma_4}\|\cdot\|_{1,2,r}}(\mathbf{Z}_{1})$,
		($\mathbf{Z}_{1} \in \SetRealNum^{\NumEndmember \times \NumPixel}$) 
		& $O(\NumPixel \NumEndmember)$ \\
		
		\addlinespace[5pt]
		$\textrm{prox}_{\tfrac{\lambda_1}{\gamma_4}\|\cdot\|_1}(\mathbf{Z}_{2})$,
		($ \mathbf{Z}_{2} \in \SetRealNum^{2\NumEndmember \times \NumPixel} $) 
		& $O(\NumPixel \NumEndmember)$ \\
		
		\addlinespace[5pt]
		$\textrm{prox}_{\tfrac{\lambda_2}{\gamma_4}\FuncRegRec}(\mathbf{Z}_{3})$, 
		$\begin{cases}
			\FuncRegRec = \|\cdot\|_{1,2,c}, \: (\mathbf{Z}_{3} \in \SetRealNum^{2\NumBand \times \NumPixel}) \\
			\FuncRegRec = \|\cdot\|_{1}, \: (\mathbf{Z}_{3} \in \SetRealNum^{2\NumBand \times \NumPixel}) \\
			\FuncRegRec = \|\cdot\|_{1}, \: (\mathbf{Z}_{3} \in \SetRealNum^{4\NumBand \times \NumPixel})
		\end{cases}$
		& $O(\NumPixel \NumBand)$ \\
		
		\addlinespace[5pt]
		$\textrm{prox}_{\tfrac{1}{\gamma_{4}} \FuncIndSymb{\SetConsFidel}}(\mathbf{Z}_{4})$,
		($\mathbf{Z}_{4} \in \SetRealNum^{\NumBand \times \NumPixel}$) 
		& $O(\NumPixel \NumBand)$ \\
		\bottomrule
	\end{tabular}
	\color{black}
\end{table}


==> tab_tex/tab_noise_colored.tex <==

\begin{table}[t]
	\caption{Assumption and Types of Noise Considered in Each Method.}
	\vspace{-1mm}
	\label{tab:noise}
	\centering
	\begin{tabular}{ccccc}
		\toprule
		\multirow{2}{*}{Methods} & \multirow{2}{*}{Assumption} & \multicolumn{3}{c}{Noise} \\
		\cmidrule(lr){3-5}
		& & Gaussian & Sparse & Stripe \\
		\cmidrule(lr){1-5}
		\vspace{0.5mm}
		CLSUnSAL~\cite{iordache2014collaborative} & non-blind & \checkmark & - & - \\
		\vspace{0.5mm}
		JSTV~\cite{aggarwal2016hyperspectral} & non-blind & \checkmark & \checkmark & - \\
		\vspace{0.5mm}
		RSSUn-TV~\cite{wang2019row} & non-blind & \checkmark & - & - \\
		\vspace{0.5mm}
		LGSU~\cite{shen2022superpixel} & non-blind & \checkmark & - & - \\
		\vspace{0.5mm}
		UnDIP~\cite{UnDIP_RastiB_2022} & non-blind & \checkmark & - & - \\
		\vspace{0.5mm}
		\color{blue}EGU-Net~\cite{hong2022endmember} & \color{blue}blind & \color{blue}\checkmark & \color{blue}- & \color{blue}- \\
		\vspace{0.5mm}
		\color{blue}RDSWSU~\cite{rs_Deng_RobustDual_2023} & \color{blue}non-blind & \color{blue}\checkmark & \color{blue}- & \color{blue}- \\
		\vspace{0.5mm}
		MdLRR~\cite{MDLRR_WuLing_2023} & non-blind & \checkmark & - & - \\
		%		\cmidrule(lr){1-4}
		\textbf{\Ourss (Ours)} & non-blind & \checkmark &\checkmark&\checkmark\\
		\bottomrule
	\end{tabular}
\end{table}


==> tab_tex/tab_range_params_colored.tex <==

\begin{table}[t]
	\caption{Hyperparameter Settings in Each Method.}
	\vspace{-1mm}
	\label{tab:parameter_settings}
	\centering
	\color{blue}
	\begin{tabular}{cc}
		\toprule
		Methods & Parameter search range \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-2}
		\vspace{0.5mm}
		CLSUnSAL~\cite{iordache2014collaborative} & $\lambda \in \{ 10^{-4}, 10^{-3}, 10^{-2}, 10^{-1}, 10^{0}, 10^{1}, 10^{2} \}$ \\
		\vspace{0.5mm}
		JSTV~\cite{aggarwal2016hyperspectral} & \begin{tabular}{c} $\lambda_{1} \in \{ 10^{-2}, 10^{-1}, 10^{0}, 10^{1} \}$, \\ $\lambda_{2} \in \{ 10^{-2}, 10^{-1}, 10^{0}, 10^{1} \}$, \\ $\lambda_{3} \in \{ 10^{-1}, 10^{0}, 10^{1} \}$ \end{tabular} \\
		\vspace{0.5mm}
		RSSUn-TV~\cite{wang2019row} & \begin{tabular}{c} $\lambda \in \{ 10^{-2}, 10^{-1}, 10^{0}, 10^{1} \}$, \\ $\lambda_{TV} \in \{ 10^{-4}, 10^{-3}, 10^{-2}, 10^{-1} \}$ \end{tabular} \\
		\vspace{0.5mm}
		LGSU~\cite{shen2022superpixel} & \begin{tabular}{c} $\lambda_{g} \in \{ 10^{-3}, 10^{-2}, 10^{-1}, 10^{0}, 10^{1} \}$, \\ $\lambda_{l} \in \{ 10^{-4}, 10^{-3}, 10^{-2}, 10^{-1} \}$ \end{tabular} \\
		\vspace{0.5mm}
		UnDIP~\cite{UnDIP_RastiB_2022} & -- \\
		\vspace{0.5mm}
		EGU-Net~\cite{hong2022endmember} & -- \\
		\vspace{0.5mm}
		RDSWSU~\cite{rs_Deng_RobustDual_2023} & $\lambda \in \{ 10^{-3}, 10^{-2}, 10^{-1}, 10^{0}, 10^{1} \}$ \\
		\vspace{0.5mm}
		MdLRR~\cite{MDLRR_WuLing_2023} & \begin{tabular}{c} $\lambda \in \{ 10^{-3}, 10^{-2}, 10^{-1} \}$, \\ $\tau \in \{ 10^{-3}, 10^{-2}, 10^{-1}, 10^{0} \}$ \end{tabular} \\
		%		\cmidrule(lr){1-4}
		\textbf{\Ourss (Ours)} & \begin{tabular}{c} $\lambda_{1} \in \{ 10^{-2}, 10^{-1}, 10^{0}, 10^{1} \}$, \\ $\lambda_{2} \in \{ 10^{-2}, 10^{-1}, 10^{0}, 10^{1} \}$, \\ $\alpha \in \{ 0.95, 0.98 \}$ \end{tabular} \\
		\bottomrule
	\end{tabular}
	\color{black}
\end{table}



%CLSUnSAL: $\lambda \in \{ 10^{-4}, 10^{-3}, 10^{-2}, 10^{-1}, 10^{0}, 10^{1}, 10^{2} \}$
%JSTV: $\lambda_{1} \in \{ 10^{-2}, 10^{-1}, 10^{0}, 10^{1} \}$, $\lambda_{2} \in \{ 10^{-2}, 10^{-1}, 10^{0}, 10^{1} \}$, $\lambda_{3} \in \{ 10^{-1}, 10^{0}, 10^{1} \}$
%RSSUn-TV: $\lambda \in \{ 10^{-2}, 10^{-1}, 10^{0}, 10^{1} \}$, $\lambda_{TV} \in \{ 10^{-4}, 10^{-3}, 10^{-2}, 10^{-1} \}$
%LGSU: $\lambda_{g} \in \{ 10^{-3}, 10^{-2}, 10^{-1}, 10^{0}, 10^{1} \}$, $\lambda_{l} \in \{ 10^{-4}, 10^{-3}, 10^{-2}, 10^{-1} \}$
%RDSWSU: $\lambda \in \{ 10^{-3}, 10^{-2}, 10^{-1}, 10^{0}, 10^{1} \}$
%MdLRR: $\lambda \in \{ 10^{-3}, 10^{-2}, 10^{-1} \}$, $\tau \in \{ 10^{-3}, 10^{-2}, 10^{-1}, 10^{0} \}$
%Ours: $\lambda_{1} \in \{ 10^{-2}, 10^{-1}, 10^{0}, 10^{1} \}$, $\lambda_{2} \in \{ 10^{-2}, 10^{-1}, 10^{0}, 10^{1} \}$, $\alpha = \{ 0.95, 0.98 \}$.
%UnDIP, EGU-Net have no parameters to adjust, but the experiment process follows these references.



==> tab_tex/tab_result_jasper_colored.tex <==

%\begin{table*}[!h]
%	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM in the Experiments Using \textit{Jasper Ridge}.}
%	\vspace{-1mm}
%	\label{tab:result_jasper}
%	\centering
%%	\scriptsize
%	\scalebox{0.95}{
	%		\begin{tabular}{cccccccccccc} \toprule
		%			\multirow{3}{*}{ Noise } & \multirow{3}{6em}{\centering Evaluation \\ Target}  & \multirow{3}{*}{Measures}& \multicolumn{9}{c}{Methods}\\ 
		%			\cmidrule(lr){4-12}
		%			& & & CLSUnSAL & JSTV & RSSUn-TV & LGSU & UnDIP & MdLRR & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
		%			& & & \cite{iordache2014collaborative} & \cite{aggarwal2016hyperspectral} & \cite{wang2019row} & \cite{shen2022superpixel} & \cite{UnDIP_RastiB_2022} & \cite{MDLRR_WuLing_2023} & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
		%			
		%			\midrule
		%			
		%			\multirow{5}{*}{Case 1} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & \ValSecnd{19.97} & 16.22 & 15.88 & {19.72} & 8.12 & \Valbest{20.23} & 17.72 & 17.07 & 17.06 \\
		%			& & RMSE & \ValSecnd{0.0431} & 0.0664 & 0.0690 & {0.0444} & 0.1688 & \Valbest{0.0412} & 0.0559 & 0.0602 & 0.0603 \\
		%			& & Ps   & 0.42 & 0.40 & 0.40 & 0.40 & 0.31 & \ValSecnd{0.43} & \Valbest{0.44} & 0.42 & \ValSecnd{0.43} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & {37.67} & 36.80 & 36.71 & \Valbest{38.28} & 25.37 & \ValSecnd{37.85} & 37.35 & 37.02 & 36.96 \\
		%			& HS image
		%			& MSSIM & 0.9858 & 0.9821 & 0.9817 & \ValSecnd{0.9866} & 0.9129 & 0.9858 & \Valbest{0.9878} & 0.9857 & 0.9864 \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 2} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 15.24 & 11.11 & 10.95 & 12.92 & 5.64 & 12.44 & \Valbest{16.09} & 15.59 & \ValSecnd{15.62} \\
		%			& & RMSE & 0.0744 & 0.1197 & 0.1218 & 0.0972 & 0.2245 & 0.1011 & \Valbest{0.0674} & 0.0715 & \ValSecnd{0.0712} \\
		%			& & Ps   & 0.37 & 0.34 & 0.34 & 0.34 & 0.31 & 0.36 & \Valbest{0.40} & \Valbest{0.40} & \Valbest{0.40} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 32.01 & 31.08 & 31.04 & 31.92 & 21.07 & 31.43 & \Valbest{33.40} & 32.90 & \ValSecnd{33.29} \\
		%			& HS image
		%			& MSSIM & 0.9538 & 0.9409 & 0.9404 & 0.9477 & 0.8303 & 0.9438 & \Valbest{0.9687} & 0.9629 & \ValSecnd{0.9681} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 3} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 11.74 & 15.48 & 7.62 & 8.12 & 3.65 & 8.38 & \Valbest{17.49} & \ValSecnd{16.85} & 16.83 \\
		%			& & RMSE & 0.1112 & 0.0724 & 0.1789 & 0.1687 & 0.2823 & 0.1652 & \Valbest{0.0574} & \ValSecnd{0.0618} & 0.0619 \\
		%			& & Ps   & 0.33 & 0.40 & 0.32 & 0.32 & 0.20 & 0.33 & \Valbest{0.44} & \ValSecnd{0.43} & \ValSecnd{0.43} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 25.44 & 35.70 & 24.85 & 25.05 & 16.74 & 24.89 & \Valbest{36.59} & \ValSecnd{36.26} & 36.23 \\
		%			& HS image
		%			& MSSIM & 0.8701 & 0.9771 & 0.8442 & 0.8479 & 0.6797 & 0.8460 & \Valbest{0.9851} & 0.9827 & \ValSecnd{0.9837} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 4} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 8.83 & 14.38 & 4.83 & 4.98 & 3.84 & 5.61 & \Valbest{17.77} & \ValSecnd{17.28} & 17.27 \\
		%			& & RMSE & 0.1556 & 0.0821 & 0.2465 & 0.2424 & 0.2762 & 0.2357 & \Valbest{0.0556} & \ValSecnd{0.0588} & 0.0589 \\
		%			& & Ps   & 0.28 & 0.38 & 0.27 & 0.27 & 0.19 & 0.28 & \Valbest{0.43} & \ValSecnd{0.42} & \ValSecnd{0.42} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 20.83 & 34.70 & 20.42 & 20.51 & 19.05 & 20.43 & \Valbest{36.30} & 35.94 & \ValSecnd{36.08} \\
		%			& HS image
		%			& MSSIM & 0.7734 & 0.9716 & 0.7412 & 0.7435 & 0.7610 & 0.7429 & \Valbest{0.9830} & 0.9804 & \ValSecnd{0.9820} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 5} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 11.17 & 11.83 & 6.95 & 7.39 & 5.79 & 7.65 & \Valbest{16.37} & 15.91 & \ValSecnd{15.93} \\
		%			& & RMSE & 0.1188 & 0.1102 & 0.1932 & 0.1837 & 0.2207 & 0.1801 & \Valbest{0.0653} & 0.0688 & \ValSecnd{0.0687} \\
		%			& & Ps   & 0.33 & 0.36 & 0.31 & 0.31 & 0.28 & 0.32 & \Valbest{0.42} & \Valbest{0.42} & \Valbest{0.42} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 25.09 & 32.19 & 24.47 & 24.65 & 20.87 & 24.50 & \Valbest{34.98} & 34.51 & \ValSecnd{34.86} \\
		%			& HS image
		%			& MSSIM & 0.8613 & 0.9559 & 0.8347 & 0.8381 & 0.8001 & 0.8363 & \Valbest{0.9795} & 0.9759 & \ValSecnd{0.9788} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 6} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 10.60 & 9.36 & 6.36 & 6.62 & 3.28 & 6.99 & \Valbest{14.06} & 13.56 & \ValSecnd{13.59} \\
		%			& & RMSE & 0.1268 & 0.1463 & 0.2068 & 0.2006 & 0.2947 & 0.1955 & \Valbest{0.0852} & 0.0902 & \ValSecnd{0.0899} \\
		%			& & Ps   & 0.31 & 0.32 & 0.29 & 0.29 & 0.18 & 0.30 & \Valbest{0.39} & \Valbest{0.39} & \Valbest{0.39} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 24.46 & 28.75 & 23.81 & 23.96 & 18.83 & 23.84 & \Valbest{31.45} & 30.79 & \ValSecnd{31.24} \\
		%			& HS image
		%			& MSSIM & 0.8407 & 0.9102 & 0.8106 & 0.8136 & 0.7317 & 0.8115 & \Valbest{0.9566} & 0.9459 & \ValSecnd{0.9550} \\
		%			\bottomrule
		%		\end{tabular}
	%	}
%\end{table*}


\begin{table*}[!h]
	\color{blue}
	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM in the Experiments Using \textit{Jasper Ridge}.}
	\vspace{-1mm}
	\label{tab:result_jasper}
	\centering
	%	\scriptsize
	\scalebox{0.75}{
		\begin{tabular}{ccccccccccccc} \toprule
			\multirow{3}{*}{ Noise } & \multirow{3}{*}{Metrics}& \multicolumn{11}{c}{Methods}\\ 
			\cmidrule(lr){3-13}
			& & CLSUnSAL & JSTV & RSSUn-TV & LGSU & UnDIP & EGU-Net & RDSWSU & MdLRR & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
			& & \cite{iordache2014collaborative} & \cite{aggarwal2016hyperspectral} & \cite{wang2019row} & \cite{shen2022superpixel} & \cite{UnDIP_RastiB_2022} & \cite{hong2022endmember} & \cite{rs_Deng_RobustDual_2023} & \cite{MDLRR_WuLing_2023} & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
			%			& & $\lambda$ & $\lambda_{1},\lambda_{2},\lambda_{3}$ & $\lambda, \lambda_{TV}$ & $\lambda_{g}, \lambda_{l}$ & - & - & $\lambda$ & $\lambda, \tau$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ \\ 
			\midrule
			
			\multirow{6}{*}{Case 1} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   \ValSecnd{20.24} &   15.99 &   20.12 &   19.45 &    3.59 &   -1.42 &   20.13 &   \Valbest{20.48} &   19.07 &   19.33 &   19.06 \\ 
			& RMSE &   \ValSecnd{0.0256} &   0.0412 &   0.0263 &   0.0286 &   0.1518 &   0.2002 &   0.0270 &   \Valbest{0.0252} &   0.0294 &   0.0286 &   0.0295 \\ 
			& Ps   &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   0.64 &   0.07 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   45.22 &   35.09 &   45.50 &   45.60 &   32.81 &   18.56 &   \Valbest{45.78} &   \ValSecnd{45.65} &   45.45 &   45.47 &   45.45 \\ 
			& MSSIM &   0.9877 &   0.9234 &   0.9878 &   0.9871 &   0.9330 &   0.4523 &   0.9877 &   0.9876 &   \Valbest{0.9882} &   0.9881 &   \Valbest{0.9882} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 2} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   14.81 &   10.14 &   13.91 &   13.93 &   -0.13 &   -3.23 &   15.35 &   14.32 &   \ValSecnd{15.49} &   \Valbest{15.53} &   15.37 \\ 
			& RMSE &   0.0468 &   0.0743 &   0.0535 &   0.0527 &   0.2247 &   0.2664 &   0.0470 &   0.0510 &   \ValSecnd{0.0436} &   \Valbest{0.0432} &   0.0441 \\ 
			& Ps   &   \Valbest{0.99} &   0.96 &   0.98 &   0.98 &   0.58 &   0.00 &   \Valbest{0.99} &   \Valbest{0.99} &   \Valbest{0.99} &   \Valbest{0.99} &   \Valbest{0.99} \\ 
			& MPSNR &   39.53 &   32.25 &   39.45 &   39.77 &   27.85 &   17.65 &   40.15 &   39.46 &   \Valbest{40.97} &   40.31 &   \ValSecnd{40.36} \\ 
			& MSSIM &   0.9582 &   0.8809 &   0.9533 &   0.9541 &   0.8343 &   0.4552 &   0.9569 &   0.9512 &   \Valbest{0.9732} &   0.9634 &   \ValSecnd{0.9641} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 3} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   10.14 &   15.82 &    9.06 &    8.78 &   -1.88 &   -1.89 &   10.25 &    8.87 &   \ValSecnd{18.76} &   \Valbest{18.98} &   18.75 \\ 
			& RMSE &   0.0751 &   0.0419 &   0.0961 &   0.0948 &   0.2327 &   0.1952 &   0.0872 &   0.0969 &   \ValSecnd{0.0304} &   \Valbest{0.0296} &   \ValSecnd{0.0304} \\ 
			& Ps   &   0.94 &   \Valbest{1.00} &   0.88 &   0.89 &   0.35 &   0.33 &   0.92 &   0.88 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   32.74 &   34.89 &   32.66 &   32.74 &   24.90 &   19.56 &   33.50 &   32.54 &   \Valbest{44.47} &   \Valbest{44.47} &   \Valbest{44.47} \\ 
			& MSSIM &   0.8733 &   0.9195 &   0.8628 &   0.8584 &   0.7162 &   0.5420 &   0.8761 &   0.8561 &   \ValSecnd{0.9849} &   0.9848 &   \Valbest{0.9850} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 4} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    6.70 &   13.03 &    5.70 &    5.75 &   -2.60 &   -2.05 &    6.39 &    5.61 &   \Valbest{18.31} &   \ValSecnd{18.29} &   18.26 \\ 
			& RMSE &   0.1005 &   0.0559 &   0.1490 &   0.1377 &   0.2527 &   0.1926 &   0.1420 &   0.1471 &   \Valbest{0.0319} &   \ValSecnd{0.0321} &   \ValSecnd{0.0321} \\ 
			& Ps   &   0.85 &   0.98 &   0.66 &   0.72 &   0.21 &   0.33 &   0.74 &   0.70 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   28.01 &   35.05 &   27.98 &   28.03 &   23.94 &   19.71 &   28.39 &   27.93 &   \Valbest{43.89} &   \ValSecnd{43.39} &   \ValSecnd{43.39} \\ 
			& MSSIM &   0.7871 &   0.9343 &   0.7589 &   0.7560 &   0.7056 &   0.5584 &   0.7704 &   0.7532 &   \Valbest{0.9836} &   \ValSecnd{0.9803} &   0.9802 \\ 
			\midrule 
			
			\multirow{6}{*}{Case 5} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    9.56 &   10.65 &    8.27 &    8.12 &    0.13 &   -0.50 &    9.41 &    8.21 &   \Valbest{16.36} &   16.16 &   \ValSecnd{16.19} \\ 
			& RMSE &   0.0799 &   0.0716 &   0.1054 &   0.1020 &   0.1976 &   0.1761 &   0.0968 &   0.1043 &   \Valbest{0.0394} &   0.0401 &   \ValSecnd{0.0400} \\ 
			& Ps   &   0.92 &   0.96 &   0.84 &   0.86 &   0.50 &   0.37 &   0.89 &   0.85 &   \ValSecnd{0.99} &   \ValSecnd{0.99} &   \Valbest{1.00} \\ 
			& MPSNR &   32.39 &   32.40 &   32.26 &   32.34 &   27.32 &   20.03 &   33.10 &   32.15 &   \Valbest{42.26} &   \ValSecnd{41.63} &   41.49 \\ 
			& MSSIM &   0.8645 &   0.9018 &   0.8529 &   0.8486 &   0.7606 &   0.6114 &   0.8666 &   0.8464 &   \Valbest{0.9791 }&   \ValSecnd{0.9744} &   0.9735 \\ 
			\midrule 
			
			\multirow{6}{*}{Case 6} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    9.16 &    9.13 &    7.26 &    7.87 &    1.51 &   -1.03 &    8.60 &    7.28 &   \Valbest{14.39} &   14.03 &   \ValSecnd{14.19} \\ 
			& RMSE &   0.0807 &   0.0818 &   0.1204 &   0.1070 &   0.1629 &   0.1836 &   0.1075 &   0.1180 &   \Valbest{0.0489} &   0.0507 &   \ValSecnd{0.0500} \\ 
			& Ps   &   0.93 &   0.95 &   0.78 &   0.84 &   0.61 &   0.34 &   0.85 &   0.80 &   \Valbest{0.99} &   \Valbest{0.99} &   \Valbest{0.99} \\ 
			& MPSNR &   31.64 &   30.93 &   31.58 &   31.83 &   26.89 &   20.02 &   32.42 &   31.47 &   \Valbest{38.82} &   37.78 &   \ValSecnd{38.04} \\ 
			& MSSIM &   0.8543 &   0.8573 &   0.8291 &   0.8287 &   0.7650 &   0.5836 &   0.8441 &   0.8224 &   \Valbest{0.9563} &   0.9396 &   \ValSecnd{0.9435} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 7} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   11.51 &    8.85 &    9.75 &   10.24 &   -0.93 &   -1.06 &   11.75 &   10.19 &   \Valbest{13.67} &   13.27 &   \ValSecnd{13.35} \\ 
			& RMSE &   0.0653 &   0.0911 &   0.0870 &   0.0805 &   0.2345 &   0.2025 &   0.0718 &   0.0822 &   \Valbest{0.0531} &   0.0551 &   \ValSecnd{0.0547} \\ 
			& Ps   &   \Valbest{0.98} &   0.91 &   0.90 &   0.92 &   0.47 &   0.35 &   0.94 &   0.91 &   \Valbest{0.98} &   \Valbest{0.98} &   \Valbest{0.98} \\ 
			& MPSNR &   35.46 &   26.18 &   35.69 &   35.83 &   25.69 &   18.70 &   36.49 &   35.68 &   \Valbest{38.22} &   36.94 &   \ValSecnd{37.25} \\ 
			& MSSIM &   0.9131 &   0.6888 &   0.9011 &   0.9000 &   0.7413 &   0.3965 &   0.9110 &   0.8988 &   \Valbest{0.9502} &   0.9250 &   \ValSecnd{0.9310} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 8} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    8.39 &    7.73 &    6.20 &    6.75 &   -0.65 &   -3.94 &    7.34 &    6.14 &   \Valbest{12.46} &   12.12 &   \ValSecnd{12.21} \\ 
			& RMSE &   0.0880 &   0.1014 &   0.1398 &   0.1257 &   0.2172 &   0.2594 &   0.1302 &   0.1387 &   \Valbest{0.0604} &   0.0623 &   \ValSecnd{0.0619} \\ 
			& Ps   &   0.89 &   0.87 &   0.71 &   0.77 &   0.40 &   0.00 &   0.77 &   0.73 &   \Valbest{0.97} &   {0.97} &   {0.97} \\ 
			& MPSNR &   31.05 &   25.28 &   30.86 &   31.08 &   25.74 &   15.92 &   31.74 &   30.74 &   \Valbest{36.93} &   35.67 &   \ValSecnd{35.97} \\ 
			& MSSIM &   0.8282 &   0.6531 &   0.7953 &   0.7949 &   0.7198 &   0.2987 &   0.8119 &   0.7891 &   \Valbest{0.9371} &   0.9055 &   \ValSecnd{0.9124} \\ 
			\bottomrule
		\end{tabular}
	}
\end{table*}


==> tab_tex/tab_result_jasper_pre.tex <==

\begin{table*}[!h]
	\caption{The SRE, RMSE, Ps, MPSNR, and MSSIM Results in the Experiments With the Real HS Image (\textit{Jasper Ridge}).}
	\vspace{2mm}
	\label{tab:result_jasper}
	\centering
%	\scriptsize
	\scalebox{1.0}{
		\begin{tabular}{ccccccccccc} \toprule
			\multirow{3}{*}{ Noise } & \multirow{3}{6em}{\centering Evaluation \\ Target}  & \multirow{3}{*}{Measures}& \multicolumn{8}{c}{Methods}\\ 
			\cmidrule(lr){4-11}
			& & & CLSUnSAL & JSTV & RSSUn-TV & LGSU & UnDIP & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
			& & & \cite{iordache2014collaborative} & \cite{aggarwal2016hyperspectral} & \cite{wang2019row} & \cite{shen2022superpixel} & \cite{UnDIP_RastiB_2022} & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
			
			\midrule
			
			\multirow{5}{*}{Case 1} 
			& \multirow{3}{*}{Abundance}
			& SRE  & 12.04 & 11.58 & 10.99 & \Valbest{19.21} & 5.22 & \ValSecnd{12.51} & 11.74 & 11.80 \\
			& & RMSE & 0.1076 & 0.1134 & 0.1213 & \Valbest{0.0469} & 0.2356 & \ValSecnd{0.1019} & 0.1113 & 0.1106 \\
			& & Ps   & 0.39 & 0.37 & 0.36 & \Valbest{0.45} & 0.33 & \ValSecnd{0.40} & 0.39 & 0.39 \\
			\cmidrule(lr){2-11}
			& Reconstructed
			& MPSNR & 37.78 & 37.15 & 37.02 & \ValSecnd{38.19} & 29.94 & \Valbest{38.26} & 37.94 & 37.99 \\
			& HS image
			& MSSIM & 0.9873 & 0.9840 & 0.9835 & 0.9863 & 0.9409 & \Valbest{0.9900} & 0.9891 & \ValSecnd{0.9898} \\
			\cmidrule(lr){1-11}
			
			\multirow{5}{*}{Case 2} 
			& \multirow{3}{*}{Abundance}
			& SRE  & 8.28 & 7.38 & 7.14 & \Valbest{10.89} & 5.27 & \ValSecnd{10.55} & 10.11 & 10.17 \\
			& & RMSE & 0.1658 & 0.1838 & 0.1889 & \Valbest{0.1190} & 0.2343 & \ValSecnd{0.1277} & 0.1343 & 0.1333 \\
			& & Ps   & 0.34 & 0.32 & 0.31 & \Valbest{0.38} & 0.28 & \ValSecnd{0.35} & 0.34 & \ValSecnd{0.35} \\
			\cmidrule(lr){2-11}
			& Reconstructed
			& MPSNR & 32.25 & 31.53 & 31.47  & 32.08 & 25.95 & \ValSecnd{33.35} & 33.16 & \Valbest{33.50} \\
			& HS image
			& MSSIM & 0.9574 & 0.9459 & 0.9453 & 0.9495 & 0.9031 & \ValSecnd{0.9678} & 0.9659 & \Valbest{0.9697} \\
			\cmidrule(lr){1-11}
			
			\multirow{5}{*}{Case 3} 
			& \multirow{3}{*}{Abundance}
			& SRE  & 4.79 & 9.85 & 2.89 & 3.78 & 3.05 & \Valbest{12.45} & 11.77 & \ValSecnd{11.84} \\
			& & RMSE & 0.2476 & 0.1383 & 0.3082 & 0.2924 & 0.3026 & \Valbest{0.1026} & 0.1109 & \ValSecnd{0.1100} \\
			& & Ps   & 0.25 & 0.35 & 0.26 & 0.27 & 0.17 & \Valbest{0.40} & \ValSecnd{0.39} & \ValSecnd{0.39} \\
			\cmidrule(lr){2-11}
			& Reconstructed
			& MPSNR & 21.45 & 35.12 & 21.06 & 21.09 & 21.05 & \Valbest{36.69} & 36.46 & \ValSecnd{36.63} \\
			& HS image
			& MSSIM & 0.7990 & 0.9745 & 0.7647 & 0.7655 & 0.7742 & \ValSecnd{0.9846} & 0.9836 & \Valbest{0.9849} \\
			\cmidrule(lr){1-11}
			
			\multirow{5}{*}{Case 4} 
			& \multirow{3}{*}{Abundance}
			& SRE  & 6.34 & 10.52 & 4.93 & 6.43 & 4.59 & \Valbest{12.16} & 11.44 & \ValSecnd{11.50} \\
			& & RMSE & 0.2071 & 0.1281 & 0.2438 & 0.2046 & 0.2534 & \Valbest{0.1061} & 0.1152 & \ValSecnd{0.1144} \\
			& & Ps   & 0.31 & 0.36 & 0.29 & 0.33 & 0.28 & \Valbest{0.39} & 0.38 & \Valbest{0.39} \\
			\cmidrule(lr){2-11}
			& Reconstructed
			& MPSNR & 26.04 & 36.00 & 25.55 & 25.68 & 25.19 & \Valbest{37.37} & 37.08 & \ValSecnd{37.16} \\
			& HS image
			& MSSIM & 0.8835 & 0.9793 & 0.8612 & 0.8636 & 0.8819 & \Valbest{0.9876} & 0.9865 & \ValSecnd{0.9875} \\
			\cmidrule(lr){1-11}
			
			\multirow{5}{*}{Case 5} 
			& \multirow{3}{*}{Abundance}
			& SRE  & 6.21 & 8.20 & 4.77 & 5.56 & 4.01 & \Valbest{10.07} & 9.54 & \ValSecnd{9.60} \\
			& & RMSE & 0.2102 & 0.1673 & 0.2482 & 0.2218 & 0.2711 & \Valbest{0.1348} & 0.1433 & \ValSecnd{0.1424} \\
			& & Ps   & 0.30 & 0.33 & 0.29 & 0.31 & 0.23 & \Valbest{0.35} & 0.34 & \Valbest{0.35} \\
			\cmidrule(lr){2-11}
			& Reconstructed
			& MPSNR & 25.77 & 33.01 & 25.31 & 25.41 & 23.46 & \ValSecnd{35.37} & 35.04 & \Valbest{35.46} \\
			& HS image
			& MSSIM & 0.8778 & 0.9624 & 0.8541 & 0.8558 & 0.8600 & \ValSecnd{0.9816} & 0.9797 & \Valbest{0.9826} \\
			\cmidrule(lr){1-11}
			
			\multirow{5}{*}{Case 6} 
			& \multirow{3}{*}{Abundance}
			& SRE  & 5.59 & 5.85 & 4.01 & 4.61 & 4.65 & \Valbest{7.23} & 6.90 & \ValSecnd{6.96} \\
			& & RMSE & 0.2258 & 0.2192 & 0.2711 & 0.2502 & 0.2518 & \Valbest{0.1871} & 0.1943 & \ValSecnd{0.1929} \\
			& & Ps   & 0.28 & 0.29 & 0.27 & 0.28 & 0.21 & \Valbest{0.31} & \Valbest{0.31} & \Valbest{0.31} \\
			\cmidrule(lr){2-11}
			& Reconstructed
			& MPSNR & 25.04 & 29.26 & 24.51 & 24.59 & 23.42 & \Valbest{31.70} & 31.29 & \Valbest{31.70} \\
			& HS image
			& MSSIM & 0.8564 & 0.9167 & 0.8290 & 0.8304 & 0.8295 & \ValSecnd{0.9599} & 0.9540 & \Valbest{0.9614} \\
			\bottomrule
		\end{tabular}
	}
\end{table*}

==> tab_tex/tab_result_samson_colored.tex <==

%\begin{table*}[!h]
%	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM in the Experiments Using \textit{Samson}.}
%	\vspace{-1mm}
%	\label{tab:result_samson}
%	\centering
%%	\scriptsize
%	\scalebox{0.95}{
	%		\begin{tabular}{cccccccccccc} \toprule
		%			\multirow{3}{*}{ Noise } & \multirow{3}{6em}{\centering Evaluation \\ Target}  & \multirow{3}{*}{Measures}& \multicolumn{9}{c}{Methods}\\ 
		%			\cmidrule(lr){4-12}
		%			& & & CLSUnSAL & JSTV & RSSUn-TV & LGSU & UnDIP & MdLRR & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
		%			& & & \cite{iordache2014collaborative} & \cite{aggarwal2016hyperspectral} & \cite{wang2019row} & \cite{shen2022superpixel} & \cite{UnDIP_RastiB_2022} & \cite{MDLRR_WuLing_2023} &  \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
		%			
		%			\midrule
		%			
		%			\multirow{5}{*}{Case 1} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 12.46 & 11.29 & 10.75 & 10.04 & 7.62 & 13.81 & \ValSecnd{14.84} & 14.68 & \Valbest{15.11} \\
		%			& & RMSE & 0.0998 & 0.1166 & 0.1241 & 0.1331 & 0.1909 & 0.0874 & \ValSecnd{0.0761} & 0.0767 & \Valbest{0.0737} \\
		%			& & Ps   & 0.67 & 0.64 & 0.63 & 0.63 & 0.41 & 0.68 & \ValSecnd{0.77} & \ValSecnd{0.77} & \Valbest{0.78} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 35.55 & 35.06 & 34.91 & 35.17 & 22.39 & 35.73 & \ValSecnd{37.85} & 37.23 & \Valbest{37.87} \\
		%			& HS image
		%			& MSSIM & 0.9772 & 0.9733 & 0.9722 & 0.9736 & 0.8705 & 0.9780 & \Valbest{0.9899} & 0.9869 & \ValSecnd{0.9897} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 2} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 7.87 & 6.63 & 6.35 & 6.41 & 2.21 & 7.31 & \ValSecnd{10.22} & 9.98 & \Valbest{10.53} \\
		%			& & RMSE & 0.1602 & 0.1973 & 0.2046 & 0.2024 & 0.3555 & 0.1836 & \ValSecnd{0.1166} & 0.1185 & \Valbest{0.1128} \\
		%			& & Ps   & 0.57 & 0.52 & 0.51 & 0.51 & 0.22 & 0.54 & \Valbest{0.66} & {0.65} & \Valbest{0.66} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 30.00 & 29.45 & 29.36 & 29.67 & 15.74 & 29.55 & \ValSecnd{31.90} & 31.40 & \Valbest{32.03} \\
		%			& HS image
		%			& MSSIM & 0.9271 & 0.9144 & 0.9125 & 0.9165 & 0.7066 & 0.9166 & \ValSecnd{0.9552} & 0.9484 & \Valbest{0.9569} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 3} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 5.52 & 10.32 & 4.53 & 4.73 & 4.59 & 4.70 & \ValSecnd{14.26} & 14.18 & \Valbest{14.63} \\
		%			& & RMSE & 0.1964 & 0.1300 & 0.3022 & 0.2967 & 0.2703 & 0.2925 & \ValSecnd{0.0804} & 0.0806 & \Valbest{0.0774} \\
		%			& & Ps   & 0.49 & 0.62 & 0.43 & 0.43 & 0.29 & 0.45 & \Valbest{0.76} & \Valbest{0.76} & \Valbest{0.76} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 23.14 & 33.91 & 22.66 & 22.83 & 16.30 & 22.51 & \ValSecnd{36.78} & 36.16 & \Valbest{36.82} \\
		%			& HS image
		%			& MSSIM & 0.7912 & 0.9658 & 0.7677 & 0.7717 & 0.6529 & 0.7644 & \Valbest{0.9865} & 0.9827 & \ValSecnd{0.9864} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 4} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 3.17 & 9.17 & 3.31 & 3.44 & 1.76 & 3.34 & \ValSecnd{13.39} & 13.22 & \Valbest{13.60} \\
		%			& & RMSE & 0.2368 & 0.1464 & 0.3990 & 0.3986 & 0.3745 & 0.3905 & \ValSecnd{0.0869} & 0.0877 & \Valbest{0.0847} \\
		%			& & Ps   & 0.41 & 0.59 & 0.35 & 0.35 & 0.24 & 0.36 & \Valbest{0.75} & {0.74} & \Valbest{0.75} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 18.61 & 33.06 & 18.27 & 18.35 & 16.16 & 18.20 & \Valbest{35.85} & 35.24 & \ValSecnd{35.83} \\
		%			& HS image
		%			& MSSIM & 0.6662 & 0.9593 & 0.6365 & 0.6380 & 0.5906 & 0.6351 & \Valbest{0.9824} & 0.9783 & \ValSecnd{0.9821} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 5} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 4.97 & 7.45 & 4.27 & 4.48 & 4.98 & 4.42 & \ValSecnd{10.37} & 10.05 & \Valbest{10.75} \\
		%			& & RMSE & 0.2065 & 0.1801 & 0.3096 & 0.3045 & 0.2584 & 0.2996 & \ValSecnd{0.1144} & 0.1170 & \Valbest{0.1099} \\
		%			& & Ps   & 0.47 & 0.54 & 0.42 & 0.42 & 0.30 & 0.43 & \Valbest{0.69} & 0.68 & \Valbest{0.69} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 22.81 & 30.52 & 22.35 & 22.50 & 20.83 & 22.21 & \ValSecnd{33.70} & 33.11 & \Valbest{33.85} \\
		%			& HS image
		%			& MSSIM & 0.7822 & 0.9364 & 0.7587 & 0.7626 & 0.7465 & 0.7561 & \ValSecnd{0.9725} & 0.9673 & \Valbest{0.9735} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 6} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 4.55 & 5.36 & 3.87 & 4.02 & 3.63 & 3.98 & \ValSecnd{9.76} & 9.31 & \Valbest{10.29} \\
		%			& & RMSE & 0.2157 & 0.2433 & 0.3398 & 0.3369 & 0.3021 & 0.3319 & \ValSecnd{0.1212} & 0.1257 & \Valbest{0.1156} \\
		%			& & Ps   & 0.47 & 0.48 & 0.40 & 0.40 & 0.25 & 0.41 & \ValSecnd{0.69} & 0.68 & \Valbest{0.70} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 22.30 & 27.07 & 21.79 & 21.93 & 18.14 & 21.68 & \ValSecnd{30.63} & 29.86 & \Valbest{30.83} \\
		%			& HS image
		%			& MSSIM & 0.7559 & 0.8700 & 0.7299 & 0.7333 & 0.6863 & 0.7277 & \ValSecnd{0.9471} & 0.9330 & \Valbest{0.9500} \\
		%			\bottomrule
		%		\end{tabular}
	%	}
%\end{table*}


\begin{table*}[!h]
	\color{blue}
	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM in the Experiments Using \textit{Samson}.}
	\vspace{-1mm}
	\label{tab:result_samson}
	\centering
	%	\scriptsize
	\scalebox{0.75}{
		\begin{tabular}{ccccccccccccc} \toprule
			\multirow{3}{*}{ Noise } & \multirow{3}{*}{Metrics}& \multicolumn{11}{c}{Methods}\\ 
			\cmidrule(lr){3-13}
			& & CLSUnSAL & JSTV & RSSUn-TV & LGSU & UnDIP & EGU-Net & RDSWSU & MdLRR & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
			& & \cite{iordache2014collaborative} & \cite{aggarwal2016hyperspectral} & \cite{wang2019row} & \cite{shen2022superpixel} & \cite{UnDIP_RastiB_2022} & \cite{hong2022endmember} & \cite{rs_Deng_RobustDual_2023} & \cite{MDLRR_WuLing_2023} & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
			%			& & $\lambda$ & $\lambda_{1},\lambda_{2},\lambda_{3}$ & $\lambda, \lambda_{TV}$ & $\lambda_{g}, \lambda_{l}$ & - & - & $\lambda$ & $\lambda, \tau$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ \\
			\midrule
			
			\multirow{6}{*}{Case 1} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-4}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-3}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   16.82 &    0.01 &   17.52 &   10.89 &    2.52 &    7.27 &   13.37 &   13.96 &   \Valbest{19.51} &   16.48 &   \ValSecnd{18.03} \\ 
			& RMSE &   0.0338 &   4.0921 &   0.0309 &   0.0678 &   0.1491 &   0.0940 &   0.0539 &   0.0474 &   \Valbest{0.0254} &   0.0345 &   \ValSecnd{0.0296} \\ 
			& Ps   &   \Valbest{1.00} &   0.97 &   \Valbest{1.00} &   0.94 &   0.56 &   0.80 &   0.97 &   0.99 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   34.42 &  -11.99 &   45.31 &   43.54 &   28.92 &   24.85 &   44.90 &   44.01 &   43.75 &   45.52 &   46.74 \\ 
			& MSSIM &   0.9218 &   0.9600 &   0.9839 &   0.9731 &   0.8409 &   0.7107 &   0.9772 &   0.9774 &   0.9836 &   0.9855 &   0.9907 \\ 
			\midrule 
			
			\multirow{6}{*}{Case 2} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-4}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   \Valbest{18.36} &    6.79 &   11.64 &    6.46 &   -1.91 &    6.42 &    8.60 &    7.12 &   \ValSecnd{14.51} &   11.09 &   12.86 \\ 
			& RMSE &   \Valbest{0.0291} &   0.0902 &   0.0576 &   0.1120 &   0.2408 &   0.0976 &   0.0960 &   0.1032 &   \ValSecnd{0.0435} &   0.0590 &   0.0504 \\ 
			& Ps   &   \Valbest{1.00} &   0.97 &   \ValSecnd{0.99} &   0.74 &   0.31 &   0.77 &   0.83 &   0.78 &   \ValSecnd{0.99} &   \ValSecnd{0.99} &   \ValSecnd{0.99} \\ 
			& MPSNR &   38.12 &   29.09 &   39.23 &   38.01 &   23.33 &   25.39 &   39.20 &   37.96 &   \Valbest{40.84} &   \ValSecnd{40.45} &   40.44 \\ 
			& MSSIM &   0.9402 &   0.6970 &   0.9387 &   0.9147 &   0.6756 &   0.6802 &   0.9255 &   0.9166 &   \Valbest{0.9719} &   0.9561 &   \ValSecnd{0.9725} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 3} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-3}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   14.35 &   10.96 &    8.78 &    4.48 &   -2.66 &    4.13 &    6.49 &    4.31 &   \Valbest{18.16} &   15.61 &   \ValSecnd{16.74} \\ 
			& RMSE &   0.0446 &   0.0624 &   0.0913 &   0.1695 &   0.2501 &   0.1159 &   0.1660 &   0.1715 &   \Valbest{0.0294} &   0.0378 &   \ValSecnd{0.0341} \\ 
			& Ps   &   \Valbest{1.00} &   0.99 &   0.88 &   0.53 &   0.14 &   0.58 &   0.62 &   0.51 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   31.57 &   32.84 &   31.68 &   31.21 &   23.22 &   21.63 &   32.82 &   30.89 &   43.09 &   \ValSecnd{44.34} &   \Valbest{45.45} \\ 
			& MSSIM &   0.8178 &   0.8224 &   0.8019 &   0.7713 &   0.6394 &   0.5828 &   0.8190 &   0.7644 &   \ValSecnd{0.9812} &   0.9807 &   \Valbest{0.9868} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 4} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-3}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   10.51 &    0.02 &    5.16 &    3.10 &   -1.86 &   -1.41 &    3.97 &    2.90 &   \Valbest{16.09} &   14.57 &   \ValSecnd{15.24} \\ 
			& RMSE &   0.0653 &   3.0269 &   0.1542 &   0.2343 &   0.2358 &   0.1998 &   0.2263 &   0.2362 &   \Valbest{0.0364} &   0.0417 &   \ValSecnd{0.0390} \\ 
			& Ps   &   0.96 &   0.95 &   0.60 &   0.33 &   0.19 &   0.18 &   0.35 &   0.32 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   27.06 &   -8.81 &   27.00 &   26.74 &   24.75 &   16.26 &   27.47 &   26.59 &   42.80 &   \ValSecnd{43.41} &   \Valbest{44.25} \\ 
			& MSSIM &   0.6876 &   0.9504 &   0.6646 &   0.6377 &   0.6187 &   0.2036 &   0.6772 &   0.6351 &   \ValSecnd{0.9805} &   0.9761 &   \Valbest{0.9815} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 5} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-3}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   \Valbest{13.60} &    7.85 &    7.63 &    4.19 &   -0.17 &    3.94 &    6.34 &    4.01 &   \ValSecnd{12.91} &   10.04 &   12.12 \\ 
			& RMSE &   \Valbest{0.0478} &   0.0816 &   0.1031 &   0.1754 &   0.1974 &   0.1176 &   0.1667 &   0.1770 &   \ValSecnd{0.0489} &   0.0648 &   0.0532 \\ 
			& Ps   &   0.99 &   0.98 &   0.82 &   0.50 &   0.36 &   0.59 &   0.61 &   0.49 &   \Valbest{1.00} &   0.99 &   \Valbest{1.00} \\ 
			& MPSNR &   31.31 &   30.73 &   31.35 &   30.90 &   29.99 &   22.42 &   32.49 &   30.60 &   \Valbest{42.74} &   40.95 &   \ValSecnd{42.48} \\ 
			& MSSIM &   0.8107 &   0.7485 &   0.7920 &   0.7622 &   0.7643 &   0.6111 &   0.8128 &   0.7561 &   \Valbest{0.9811} &   0.9625 &   \ValSecnd{0.9759} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 6} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-3}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   \Valbest{13.59} &    5.51 &    6.56 &    3.78 &   -2.24 &    4.30 &    5.63 &    3.67 &   \ValSecnd{12.49} &    9.33 &   11.97 \\ 
			& RMSE &   \Valbest{0.0484} &   0.0993 &   0.1219 &   0.1929 &   0.2439 &   0.1156 &   0.1898 &   0.1932 &   \ValSecnd{0.0525} &   0.0689 &   0.0543 \\ 
			& Ps   &   \ValSecnd{0.99} &   0.98 &   0.74 &   0.46 &   0.26 &   0.59 &   0.56 &   0.44 &   \ValSecnd{0.99} &   0.98 &   \Valbest{1.00} \\ 
			& MPSNR &   30.84 &   30.86 &   30.77 &   30.33 &   25.92 &   22.21 &   31.85 &   30.07 &   \ValSecnd{38.41} &   37.76 &   \Valbest{39.70} \\ 
			& MSSIM &   0.7877 &   0.7506 &   0.7611 &   0.7326 &   0.6786 &   0.5919 &   0.7804 &   0.7277 &   0.9559 &   0.9222 &   0.9573 \\ 
			\midrule 
			
			\multirow{6}{*}{Case 7} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-3}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  & \Valbest{  16.71} &    4.71 &    7.68 &    4.59 &   -2.67 &   -0.10 &    6.43 &    4.83 & \ValSecnd{  13.61} &    8.38 &   11.28 \\ 
			& RMSE & \Valbest{  0.0350} &   0.1076 &   0.0892 &   0.1420 &   0.2622 &   0.1946 &   0.1197 &   0.1382 & \ValSecnd{  0.0466} &   0.0759 &   0.0588 \\ 
			& Ps   & \Valbest{  1.00} &   0.93 &   0.87 &   0.61 &   0.14 &   0.23 &   0.67 &   0.62 & \Valbest{  1.00} &   0.98 & \ValSecnd{  0.99} \\ 
			& MPSNR &   35.59 &   27.13 &   35.75 &   34.90 &   26.96 &   17.60 &   36.39 &   34.79 & \Valbest{  39.74} &   37.62 & \ValSecnd{  38.83} \\ 
			& MSSIM &   0.8968 &   0.6114 &   0.8757 &   0.8482 &   0.7173 &   0.2423 &   0.8831 &   0.8475 & \Valbest{  0.9651} &   0.9317 & \ValSecnd{  0.9612} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 8} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-3}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  & \Valbest{  11.52} &    2.72 &    5.16 &    3.30 &   -2.20 &   -1.28 &    5.23 &    3.23 & \ValSecnd{  10.39} &    6.26 &    9.40 \\ 
			& RMSE & \Valbest{  0.0589} &   0.1208 &   0.1400 &   0.2047 &   0.2283 &   0.1958 &   0.1979 &   0.2037 & \ValSecnd{  0.0630} &   0.0922 &   0.0714 \\ 
			& Ps   & \ValSecnd{  0.97} &   0.76 &   0.63 &   0.40 &   0.12 &   0.23 &   0.53 &   0.39 & \Valbest{  0.99} &   0.84 &   0.96 \\ 
			& MPSNR &   30.31 &   29.70 &   30.13 &   29.70 &   23.63 &   16.86 &   31.25 &   29.52 & \ValSecnd{  37.22} &   35.18 & \Valbest{  37.76} \\ 
			& MSSIM &   0.7595 &   0.7024 &   0.7230 &   0.6970 &   0.5958 &   0.2474 &   0.7493 &   0.6943 & \Valbest{  0.9447} &   0.8707 & \ValSecnd{  0.9405} \\ 
			\bottomrule
		\end{tabular}
	}
\end{table*}





==> tab_tex/tab_result_synth_Legendre200_colored.tex <==
%\begin{table*}[!h]
%	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM in the Experiments Using \textit{Synth 2}.}
%	\vspace{-1mm}
%	\label{tab:result_synth}
%	\centering
%%	\scriptsize
%	\scalebox{0.95}{
	%		\begin{tabular}{cccccccccccc} \toprule
		%			\multirow{3}{*}{ Noise } & \multirow{3}{6em}{\centering Evaluation \\ Target}  & \multirow{3}{*}{Measures}& \multicolumn{9}{c}{Methods}\\ 
		%			\cmidrule(lr){4-12}
		%			& & & CLSUnSAL & JSTV & RSSUn-TV & LGSU & UnDIP & MdLRR & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
		%			& & & \cite{iordache2014collaborative} & \cite{aggarwal2016hyperspectral} & \cite{wang2019row} & \cite{shen2022superpixel} & \cite{UnDIP_RastiB_2022} & \cite{MDLRR_WuLing_2023} & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
		%			
		%			\midrule
		%			
		%			\multirow{5}{*}{Case 1} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & \Valbest{10.57} & 9.39 & 8.70  & 6.50 & 5.89 & 6.45 & 9.95 & \ValSecnd{9.98} & 9.96 \\
		%			& & RMSE & \Valbest{0.1081} & 0.1239 & 0.1342 & 0.1694 & {0.1853} & 0.1681 & 0.1162 & \ValSecnd{0.1158} & 0.1160 \\
		%			& & Ps   & 0.60 & 0.52 & 0.49 & 0.54 & 0.35 & 0.55 & 0.78 & \Valbest{0.79} & \Valbest{0.79} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 40.41 & 39.58 & 39.38 & 40.45 & 21.80 & 40.80 & \ValSecnd{42.12} & 41.69 & \Valbest{42.16} \\
		%			& HS image
		%			& MSSIM & 0.9870 & 0.9841 & 0.9833 & 0.9875 & 0.8409 & 0.9891 & \Valbest{0.9926} & 0.9912 & \ValSecnd{0.9925} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 2} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 7.97& 6.00 & 5.64 & 5.74 & 5.55 & 5.92 & 8.39 & \ValSecnd{8.45} & \Valbest{8.48} \\
		%			& & RMSE & 0.1459 & 0.1829 & 0.1907 & 0.1837 & 0.1928 & 0.1789 & 0.1390 & \ValSecnd{0.1381} & \Valbest{0.1376} \\
		%			& & Ps   & 0.49 & 0.39 & 0.38 & 0.45 & 0.34 & 0.46 & 0.61 & \ValSecnd{0.62} & \Valbest{0.63} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 35.10 & 34.10 & 34.01 & 34.88 & 22.02 & 35.32 & \ValSecnd{36.25} & 36.01 & \Valbest{36.51} \\
		%			& HS image
		%			& MSSIM & 0.9593 & 0.9485 & 0.9477 & 0.9562 & 0.8005 & 0.9612 & \ValSecnd{0.9715} & 0.9693 & \Valbest{0.9732} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 3} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 7.19 & 8.67 & 4.27 & 5.11 & 2.95 & 5.19 & \ValSecnd{9.73} & \Valbest{9.74} & 9.72 \\
		%			& & RMSE & 0.1596 & 0.1346 & 0.2233 & 0.1986 & 0.2601 & 0.1938 & \ValSecnd{0.1192} & \Valbest{0.1190} & \ValSecnd{0.1192} \\
		%			& & Ps   & 0.47 & 0.50 & 0.34 & 0.42 & 0.35 & 0.42 & 0.78 & \Valbest{0.79} & \ValSecnd{0.78} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 32.88 & 38.63 & 31.60 & 32.24 & 21.17 & 32.56 & \ValSecnd{41.30} & 40.89 & \Valbest{41.40} \\
		%			& HS image
		%			& MSSIM & 0.9423 & 0.9806 & 0.9235 & 0.9331 & 0.8355 & 0.9387 & \Valbest{0.9914} & 0.9898 & \Valbest{0.9914} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 4} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 6.22 & 8.43 & 3.02 & 3.73 & 2.28 & 5.00 & 9.70 & \Valbest{9.77} & \ValSecnd{9.76} \\
		%			& & RMSE & 0.1785 & 0.1384 & 0.2579 & 0.2465 & 0.2810 & 0.1997 & 0.1195 & \Valbest{0.1186} & \ValSecnd{0.1187} \\
		%			& & Ps   & 0.43 & 0.48 & 0.29 & 0.36 & 0.28 & 0.38 & 0.77 & \Valbest{0.78} & \Valbest{0.78} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 29.97 & 37.94 & 28.63 & 28.98 & 20.97 & 29.20 & \ValSecnd{40.63} & 40.20 & \Valbest{40.75} \\
		%			& HS image
		%			& MSSIM & 0.9093 & 0.9773 & 0.8775 & 0.8876 & 0.7972 & 0.8936 & \ValSecnd{0.9898} & 0.9880 & \Valbest{0.9899} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 5} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 6.84 & 6.36 & 4.01 & 4.77 & 2.77 & 5.42 & \ValSecnd{9.00} & \Valbest{9.02} & 8.99 \\
		%			& & RMSE & 0.1661 & 0.1756 & 0.2301 & 0.2108 & 0.2654 & 0.1880 & \ValSecnd{0.1295} & \Valbest{0.1293} & 0.1297 \\
		%			& & Ps   & 0.45 & 0.41 & 0.32 & 0.40 & 0.21 & 0.41 & \ValSecnd{0.74} & \Valbest{0.75} & \ValSecnd{0.74} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 32.34 & 35.46 & 31.00 & 31.55 & 19.63 & 31.80 & \ValSecnd{39.10} & 38.40 & \Valbest{39.32} \\
		%			& HS image
		%			& MSSIM & 0.9368 & 0.9640 & 0.9150 & 0.9242 & 0.7990 & 0.9295 & \ValSecnd{0.9880} & 0.9850 & \Valbest{0.9885} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 6} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 6.46 & 4.62 & 3.37 & 4.16 & 4.16 & 5.27 & \ValSecnd{7.94} & \Valbest{7.97} & 7.92 \\
		%			& & RMSE & 0.1736 & 0.2146 & 0.2477 & 0.2298 & 0.2261 & 0.1917 & \ValSecnd{0.1464} & \Valbest{0.1459} & 0.1468 \\
		%			& & Ps   & 0.43 & 0.34 & 0.30 & 0.37 & 0.30 & 0.40 & \ValSecnd{0.68} & \Valbest{0.69} & \ValSecnd{0.68} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 31.18 & 32.12 & 29.95 & 30.38 & 21.76 & 30.61 & \ValSecnd{35.97} & 35.09 & \Valbest{36.11} \\
		%			& HS image
		%			& MSSIM & 0.9175 & 0.9246 & 0.8926 & 0.9012 & 0.8032 & 0.9066 & \ValSecnd{0.9735} & 0.9641 & \Valbest{0.9737} \\
		%			\bottomrule
		%		\end{tabular}
	%	}
%%\end{table*}

\begin{table*}[!h]
	\color{blue}
	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM in the Experiments Using \textit{Synth 3}.}
	\vspace{-1mm}
	\label{tab:result_synth_3}
	\centering
	%	\scriptsize
	\scalebox{0.75}{
		\begin{tabular}{ccccccccccccc} \toprule
			\multirow{3}{*}{ Noise } & \multirow{3}{*}{Metrics}& \multicolumn{11}{c}{Methods}\\ 
			\cmidrule(lr){3-13}
			& & CLSUnSAL & JSTV & RSSUn-TV & LGSU & UnDIP & EGU-Net & RDSWSU & MdLRR & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
			& & \cite{iordache2014collaborative} & \cite{aggarwal2016hyperspectral} & \cite{wang2019row} & \cite{shen2022superpixel} & \cite{UnDIP_RastiB_2022} & \cite{hong2022endmember} & \cite{rs_Deng_RobustDual_2023} & \cite{MDLRR_WuLing_2023} & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
			%			& & $\lambda$ & $\lambda_{1},\lambda_{2},\lambda_{3}$ & $\lambda, \lambda_{TV}$ & $\lambda_{g}, \lambda_{l}$ & - & - & $\lambda$ & $\lambda, \tau$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ \\
			\midrule 
			
			\multirow{6}{*}{Case 1} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   21.68 &   -0.00 &   23.03 &   22.90 &   -0.49 &   -3.64 &   25.54 &   24.21 & \Valbest{  30.26} &   26.38 & \ValSecnd{  27.58} \\ 
			& RMSE &   0.0045 &   1.8879 &   0.0039 &   0.0040 &   0.0380 &   0.0520 &   0.0030 &   0.0034 & \Valbest{  0.0017} &   0.0026 & \ValSecnd{  0.0023} \\ 
			& Ps   & \Valbest{  1.00} &   0.00 & \Valbest{  1.00} & \Valbest{  1.00} & {  0.52} &   0.02 & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR &   42.76 &  -44.42 &   42.72 &   43.14 &   18.91 &   12.43 &   45.54 &   43.10 & \Valbest{  56.00} &   46.05 & \ValSecnd{  46.49} \\ 
			& MSSIM &   0.9614 &   0.7841 &   0.9556 &   0.9587 &   0.6812 &   0.6928 &   0.9721 &   0.9647 & \Valbest{  0.9997} &   0.9822 & \ValSecnd{  0.9834} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 2} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   16.96 &   -0.00 &   15.10 &   16.82 &   -3.02 &   -0.35 &   20.97 &   18.83 & \Valbest{  28.67} &   22.34 & \ValSecnd{  22.72} \\ 
			& RMSE &   0.0076 &   1.6608 &   0.0095 &   0.0080 &   0.0410 &   0.0346 &   0.0050 &   0.0063 & \Valbest{  0.0020} &   0.0041 & \ValSecnd{  0.0040} \\ 
			& Ps   & \Valbest{  1.00} &   0.00 & \Valbest{  1.00} & \Valbest{  1.00} &   0.02 & {  0.53} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR &   37.22 &  -43.74 &   36.07 &   36.67 &   18.26 &   15.57 &   40.13 &   35.15 & \Valbest{  52.34} &   40.45 & \ValSecnd{  42.56} \\ 
			& MSSIM &   0.8721 &   0.4809 &   0.8288 &   0.8415 &   0.7765 &   0.8055 &   0.9052 &   0.8377 & \Valbest{  0.9991} &   0.9361 & \ValSecnd{  0.9624} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 3} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-1}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   13.12 &   -0.00 &   10.65 &   13.66 &   -3.83 &   -4.33 &   15.63 &   13.97 & \Valbest{  29.66} &   25.91 & \ValSecnd{  26.93} \\ 
			& RMSE &   0.0111 &   2.1084 &   0.0152 &   0.0112 &   0.0429 &   0.0479 &   0.0090 &   0.0105 & \Valbest{  0.0018} &   0.0028 & \ValSecnd{  0.0025} \\ 
			& Ps   & \ValSecnd{  0.99} &   0.00 &   0.98 &   0.97 &   0.02 &   0.02 & \Valbest{  1.00} & {  0.99} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR &   32.00 &  -45.39 &   31.33 &   32.49 &   20.44 &   12.87 &   34.41 &   29.86 & \Valbest{  55.27} &   45.23 & \ValSecnd{  47.14} \\ 
			& MSSIM &   0.7730 &   0.5410 &   0.7136 &   0.7836 &   0.5486 &   0.6956 &   0.8264 &   0.6874 & \Valbest{  0.9996} &   0.9783 & \ValSecnd{  0.9870} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 4} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-1}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    9.59 &   -0.00 &    6.88 &    9.73 &   -6.48 &   -3.74 &   10.14 &    9.44 & \Valbest{  30.92} &   25.52 & \ValSecnd{  26.68} \\ 
			& RMSE &   0.0156 &   2.0454 &   0.0225 &   0.0161 &   0.0489 &   0.0432 &   0.0167 &   0.0169 & \Valbest{  0.0016} &   0.0029 & \ValSecnd{  0.0025} \\ 
			& Ps   & {  0.96} &   0.00 &   0.87 &   0.94 &   0.00 &   0.04 &   0.92 &   0.95 & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR &   27.91 &  -45.13 &   27.34 &   28.16 &   16.13 &   15.71 &   30.11 &   25.25 & \Valbest{  55.21} &   44.34 & \ValSecnd{  45.62} \\ 
			& MSSIM &   0.6530 &   0.4900 &   0.5783 &   0.6521 &   0.4271 &   0.7979 &   0.8082 &   0.5151 & \Valbest{  0.9996} &   0.9730 & \ValSecnd{  0.9803} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 5} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-1}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   12.80 &   -0.00 &   10.15 &   13.66 &   -5.29 &   -4.01 &   15.24 &   13.47 & \Valbest{  24.96} &   21.46 & \ValSecnd{  21.54} \\ 
			& RMSE &   0.0115 &   1.7139 &   0.0161 &   0.0111 &   0.0461 &   0.0470 &   0.0094 &   0.0112 & \Valbest{  0.0031} &   0.0046 & \ValSecnd{  0.0045} \\ 
			& Ps   & \ValSecnd{  0.99} &   0.00 &   0.97 &   0.97 &   0.00 &   0.04 & \Valbest{  1.00} & {  0.99} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR &   31.76 &  -44.03 &   31.01 &   32.21 &   15.25 &   13.15 &   34.15 &   29.38 & \Valbest{  47.52} &   41.18 & \ValSecnd{  41.51} \\ 
			& MSSIM &   0.7597 &   0.4738 &   0.6970 &   0.7688 &   0.4620 &   0.7016 &   0.8153 &   0.6696 & \Valbest{  0.9980} &   0.9507 & \ValSecnd{  0.9550} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 6} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-1}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   11.84 &   -0.00 &    8.75 &   12.21 &   -6.97 &   -4.64 &   14.26 &   11.85 & \Valbest{  24.39} & \ValSecnd{  20.38} &   20.36 \\ 
			& RMSE &   0.0127 &   1.5402 &   0.0188 &   0.0126 &   0.0530 &   0.0520 &   0.0105 &   0.0134 & \Valbest{  0.0033} & \ValSecnd{  0.0051} & \ValSecnd{  0.0051} \\ 
			& Ps   & {  0.98} &   0.00 &   0.93 &   0.96 &   0.00 &   0.01 & \Valbest{  1.00} & {  0.98} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR &   30.96 &  -43.10 &   30.01 &   31.31 &   17.37 &   12.17 &   33.31 &   27.65 & \Valbest{  47.02} &   38.23 & \ValSecnd{  38.86} \\ 
			& MSSIM &   0.7132 &   0.2564 &   0.6349 &   0.7118 &   0.4976 &   0.6436 &   0.7763 &   0.5911 & \Valbest{  0.9956} &   0.9029 & \ValSecnd{  0.9176} \\ 
			\midrule 
			
			
			\multirow{6}{*}{Case 7} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   14.14 &   -0.00 &   10.63 &   13.86 &   -4.27 &   -4.21 &   17.18 &   14.05 & \Valbest{  25.57} & \ValSecnd{  20.01} &   20.00 \\ 
			& RMSE &   0.0103 &   1.4475 &   0.0158 &   0.0113 &   0.0464 &   0.0527 &   0.0077 &   0.0109 & \Valbest{  0.0029} & \ValSecnd{  0.0054} & \ValSecnd{  0.0054} \\ 
			& Ps   & \ValSecnd{  0.99} &   0.00 &   0.97 &   0.97 &   0.01 &   0.01 & \Valbest{  1.00} & \ValSecnd{  0.99} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR &   33.96 &  -42.56 &   32.28 &   33.57 &   19.63 &   12.39 &   36.47 &   29.24 & \Valbest{  48.64} &   37.09 & \ValSecnd{  38.06} \\ 
			& MSSIM &   0.7684 &   0.2893 &   0.6830 &   0.7356 &   0.4921 &   0.6608 &   0.8178 &   0.6416 & \Valbest{  0.9969} &   0.8716 & \ValSecnd{  0.8980} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 8} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-3}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   10.67 &   -0.00 &    6.95 &    9.74 &   -6.72 &   -3.78 &   12.74 &    9.49 & \Valbest{  21.12} &   18.67 & \ValSecnd{  18.69} \\ 
			& RMSE &   0.0144 &   1.0417 &   0.0234 &   0.0167 &   0.0517 &   0.0474 &   0.0126 &   0.0176 & \Valbest{  0.0047} & \ValSecnd{  0.0062} & \ValSecnd{  0.0062} \\ 
			& Ps   &   0.96 &   0.01 &   0.84 &   0.94 &   0.00 &   0.04 & \ValSecnd{  0.99} &   0.94 & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR &   29.84 &  -39.41 &   28.58 &   29.37 &   14.55 &   13.37 &   32.13 &   24.96 & \Valbest{  43.66} &   35.56 & \ValSecnd{  36.44} \\ 
			& MSSIM &   0.6476 &   0.4875 &   0.5494 &   0.5894 &   0.4098 &   0.7328 &   0.7146 &   0.4711 & \Valbest{  0.9925} &   0.8375 & \ValSecnd{  0.8696} \\ 
			\bottomrule
		\end{tabular}
	}
\end{table*}



==> tab_tex/tab_result_synth_Legendre_colored.tex <==
%\begin{table*}[t]
%	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM in the Experiments Using \textit{Synth 1}.}
%	\vspace{-1mm}
%	\label{tab:result_synth_Legendre}
%	\centering
%%	\scriptsize
%	\scalebox{0.95}{
	%		\begin{tabular}{cccccccccccc} \toprule
		%			\multirow{3}{*}{ Noise } & \multirow{3}{6em}{\centering Evaluation \\ Target}  & \multirow{3}{*}{Measures}& \multicolumn{9}{c}{Methods}\\ 
		%			\cmidrule(lr){4-12}
		%			& & & CLSUnSAL & JSTV & RSSUn-TV & LGSU & UnDIP & MdLRR & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
		%			& & & \cite{iordache2014collaborative} & \cite{aggarwal2016hyperspectral} & \cite{wang2019row} & \cite{shen2022superpixel} & \cite{UnDIP_RastiB_2022} & \cite{MDLRR_WuLing_2023} & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
		%			
		%			\midrule
		%			
		%			\multirow{5}{*}{Case 1} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 16.50 & 12.95 & 11.39  & 16.59 & 0.58 & 17.98 & \Valbest{27.22} & \ValSecnd{27.02} & 26.99 \\
		%			& & RMSE & 0.0590 & 0.0840 & 0.0992 & 0.0608 & 0.3414 & 0.0524 & \Valbest{0.0173} & \ValSecnd{0.0177} & \ValSecnd{0.0177} \\
		%			& & Ps   & 0.68 & 0.56 & 0.53 & 0.64 & 0.18 & 0.66 & \Valbest{0.92} & \Valbest{0.92} & \Valbest{0.92} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 41.26 & 39.94 & 39.70 & 41.19 & 11.80 & 41.90 & \ValSecnd{46.09} & 44.49 & \Valbest{46.26} \\
		%			& HS image
		%			& MSSIM & 0.9771 & 0.9706 & 0.9693 & 0.9754 & 0.4659 & 0.9821 & \ValSecnd{0.9936} & 0.9906 & \Valbest{0.9940} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 2} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 12.81 & 7.83 & 7.13 & 12.73 & 0.88 & 16.71 & \ValSecnd{21.85} & 21.84 & \Valbest{22.12} \\
		%			& & RMSE & 0.0889 & 0.1424 & 0.1530 & 0.0923 & 0.3302 & 0.0588 & \ValSecnd{0.0318} & \ValSecnd{0.0318} & \Valbest{0.0308} \\
		%			& & Ps   & 0.55 & 0.41 & 0.40 & 0.52 & 0.19 & 0.63 & \ValSecnd{0.80} & \ValSecnd{0.80} & \Valbest{0.81} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 36.13 & 34.51 & 34.42 & 35.39 & 12.68 & 36.07 & \ValSecnd{38.86} & 37.91 & \Valbest{39.19} \\
		%			& HS image
		%			& MSSIM & 0.9322 & 0.9114 & 0.9101 & 0.9213 & 0.4138 & 0.9327 & \ValSecnd{0.9660} & 0.9585 & \Valbest{0.9692} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 3} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 11.42 & 11.97 & 5.72 & 10.72 & 0.87 & 13.84 & \Valbest{26.40} & {26.04} & \ValSecnd{26.07} \\
		%			& & RMSE & 0.1018 & 0.0931 & 0.1720 & 0.1138 & 0.3305 & 0.0802 & \Valbest{0.0190} & {0.0197} & \ValSecnd{0.0196} \\
		%			& & Ps   & 0.53 & 0.53 & 0.36 & 0.49 & 0.18 & 0.58 & \Valbest{0.91} & \ValSecnd{0.90} & \Valbest{0.91} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 33.82 & 39.02 & 31.94 & 32.73 & 13.36 & 33.25 & \ValSecnd{45.43} & 43.64 & \Valbest{45.58} \\
		%			& HS image
		%			& MSSIM & 0.9026 & 0.9641 & 0.8688 & 0.8821 & 0.3607 & 0.8943 & \ValSecnd{0.9926} & 0.9885 & \Valbest{0.9930} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 4} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 9.20 & 10.87 & 3.47 & 7.18 & 0.68 & 9.79 & \ValSecnd{25.76} & {25.61} & \Valbest{25.81} \\
		%			& & RMSE & 0.1275 & 0.1045 & 0.2088 & 0.1614 & 0.3378 & 0.1232 & \ValSecnd{0.0205} & {0.0208} & \Valbest{0.0203} \\
		%			& & Ps   & 0.46 & 0.51 & 0.29 & 0.39 & 0.21 & 0.47 & \Valbest{0.89} & \Valbest{0.89} & \Valbest{0.90} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 30.73 & 38.20 & 28.88 & 29.28 & 13.11 & 29.75 & \ValSecnd{43.69} & 42.38 & \Valbest{43.97} \\
		%			& HS image
		%			& MSSIM & 0.8505 & 0.9573 & 0.8003 & 0.8115 & 0.3799 & 0.8259 & \ValSecnd{0.9884} & 0.9844 & \Valbest{0.9894} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 5} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 10.68 & 7.86 & 4.85 & 9.61 & 0.56 & 12.04 & \ValSecnd{23.85} & {23.71} & \Valbest{24.00} \\
		%			& & RMSE & 0.1096 & 0.1418 & 0.1860 & 0.1264 & 0.3424 & 0.0965 & \ValSecnd{0.0252} & {0.0255} & \Valbest{0.0247} \\
		%			& & Ps   & 0.50 & 0.43 & 0.34 & 0.46 & 0.16 & 0.53 & \ValSecnd{0.82} & \ValSecnd{0.82} & \Valbest{0.84} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 32.93 & 35.52 & 31.16 & 31.81 & 11.64 & 32.37 & \ValSecnd{41.33} & 40.13 & \Valbest{41.76} \\
		%			& HS image
		%			& MSSIM & 0.8908 & 0.9338 & 0.8534 & 0.8649 & 0.4211 & 0.8790 & \ValSecnd{0.9850} & 0.9792 & \Valbest{0.9870} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 6} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 9.79 & 5.83 & 4.16 & 8.10 & 0.99 & 11.05 & \Valbest{20.13} & \ValSecnd{19.72} & 19.63 \\
		%			& & RMSE & 0.1209 & 0.1720 & 0.1981 & 0.1471 & 0.3259 & 0.1075 & \Valbest{0.0377} & \ValSecnd{0.0393} & 0.0396 \\
		%			& & Ps   & 0.47 & 0.36 & 0.31 & 0.42 & 0.23 & 0.50 & \ValSecnd{0.79} & \Valbest{0.80} & \ValSecnd{0.82} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 31.85 & 32.35 & 30.13 & 30.62 & 13.87 & 31.19 & \ValSecnd{38.85} & 36.95 & \Valbest{39.44} \\
		%			& HS image
		%			& MSSIM & 0.8615 & 0.8702 & 0.8191 & 0.8294 & 0.4129 & 0.8442 & \ValSecnd{0.9702} & 0.9527 & \Valbest{0.9753} \\
		%			\bottomrule
		%		\end{tabular}
	%	}
%\end{table*}


%\begin{table*}[!h]
%	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM in the Experiments Using \textit{Synth 1}.}
%	\vspace{-1mm}
%	\label{tab:result_synth_Legendre}
%	\centering
%	%	\scriptsize
%	\scalebox{0.85}{
	%		\begin{tabular}{ccccccccccccc} \toprule
		%			\multirow{3}{*}{ Noise } & \multirow{3}{*}{Metrics}& \multicolumn{11}{c}{Methods}\\ 
		%			\cmidrule(lr){3-13}
		%			& & CLSUnSAL & JSTV & RSSUn-TV & LGSU & UnDIP & EGU-Net & RDSWSU & MdLRR & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
		%			& & \cite{iordache2014collaborative} & \cite{aggarwal2016hyperspectral} & \cite{wang2019row} & \cite{shen2022superpixel} & \cite{UnDIP_RastiB_2022} & \cite{hong2022endmember} & \cite{rs_Deng_RobustDual_2023} & \cite{MDLRR_WuLing_2023} & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
		%%			& & $\lambda$ & $\lambda_{1},\lambda_{2},\lambda_{3}$ & $\lambda, \lambda_{TV}$ & $\lambda_{g}, \lambda_{l}$ & - & - & $\lambda$ & $\lambda, \tau$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ \\ 
		%			
		%			\midrule
		%			
		%			\multirow{6}{*}{Case 1} 
		%			& Setup & \begin{tabular}{c}
			%				\hspace{-4mm} $\lambda = 1 * 10^{-2}$ \hspace{-4mm}
			%			\end{tabular} & \begin{tabular}{c}
			%				\hspace{-4mm}$\lambda_{1} = 1 * 10^{-2}$\hspace{-4mm}, \\ \hspace{-4mm}$\lambda_{2} = 0.001$\hspace{-4mm}, \\ \hspace{-4mm}$\lambda_{3} = 0.1$\hspace{-4mm}
			%			\end{tabular} &  &  &  &  &  &  &  &  &  \\
		%			& SRE  & 16.50 & 12.95 & 11.39  & 16.59 & 0.58 & & & 17.98 & \Valbest{27.22} & \ValSecnd{27.02} & 26.99 \\
		%			& RMSE & 0.0590 & 0.0840 & 0.0992 & 0.0608 & 0.3414 & & & 0.0524 & \Valbest{0.0173} & \ValSecnd{0.0177} & \ValSecnd{0.0177} \\
		%			& Ps   & 0.68 & 0.56 & 0.53 & 0.64 & 0.18 & & & 0.66 & \Valbest{0.92} & \Valbest{0.92} & \Valbest{0.92} \\
		%			
		%			& MPSNR & 41.26 & 39.94 & 39.70 & 41.19 & 11.80 & & & 41.90 & \ValSecnd{46.09} & 44.49 & \Valbest{46.26} \\
		%			& MSSIM & 0.9771 & 0.9706 & 0.9693 & 0.9754 & 0.4659 & & & 0.9821 & \ValSecnd{0.9936} & 0.9906 & \Valbest{0.9940} \\
		%			\cmidrule(lr){1-13}
		%			
		%			\multirow{5}{*}{Case 2} 
		%			& Setup & & \begin{tabular}{c}
			%				0.001, \\ 0.001, \\ 0.1
			%			\end{tabular} &  &  &  &  &  &  &  &  &  \\
		%			& SRE  & 12.81 & 7.83 & 7.13 & 12.73 & 0.88 & & & 16.71 & \ValSecnd{21.85} & 21.84 & \Valbest{22.12} \\
		%			& RMSE & 0.0889 & 0.1424 & 0.1530 & 0.0923 & 0.3302 & & & 0.0588 & \ValSecnd{0.0318} & \ValSecnd{0.0318} & \Valbest{0.0308} \\
		%			& Ps   & 0.55 & 0.41 & 0.40 & 0.52 & 0.19 & & & 0.63 & \ValSecnd{0.80} & \ValSecnd{0.80} & \Valbest{0.81} \\
		%			
		%			& MPSNR & 36.13 & 34.51 & 34.42 & 35.39 & 12.68 & & & 36.07 & \ValSecnd{38.86} & 37.91 & \Valbest{39.19} \\
		%			& MSSIM & 0.9322 & 0.9114 & 0.9101 & 0.9213 & 0.4138 & & & 0.9327 & \ValSecnd{0.9660} & 0.9585 & \Valbest{0.9692} \\
		%			\cmidrule(lr){1-13}
		%			
		%			\multirow{5}{*}{Case 3} 
		%			& Setup & & \begin{tabular}{c}
			%				0.001, \\ 0.001, \\ 0.1
			%			\end{tabular} &  &  &  &  &  &  &  &  &  \\
		%			& SRE  & 11.42 & 11.97 & 5.72 & 10.72 & 0.87 & & & 13.84 & \Valbest{26.40} & {26.04} & \ValSecnd{26.07} \\
		%			& RMSE & 0.1018 & 0.0931 & 0.1720 & 0.1138 & 0.3305 & & & 0.0802 & \Valbest{0.0190} & {0.0197} & \ValSecnd{0.0196} \\
		%			& Ps   & 0.53 & 0.53 & 0.36 & 0.49 & 0.18 & & & 0.58 & \Valbest{0.91} & \ValSecnd{0.90} & \Valbest{0.91} \\
		%			
		%			& MPSNR & 33.82 & 39.02 & 31.94 & 32.73 & 13.36 & & & 33.25 & \ValSecnd{45.43} & 43.64 & \Valbest{45.58} \\
		%			& MSSIM & 0.9026 & 0.9641 & 0.8688 & 0.8821 & 0.3607 & & & 0.8943 & \ValSecnd{0.9926} & 0.9885 & \Valbest{0.9930} \\
		%			\cmidrule(lr){1-13}
		%			
		%			\multirow{5}{*}{Case 4} 
		%			& Setup & & \begin{tabular}{c}
			%				0.001, \\ 0.001, \\ 0.1
			%			\end{tabular} &  &  &  &  &  &  &  &  &  \\
		%			& SRE  & 9.20 & 10.87 & 3.47 & 7.18 & 0.68 & & & 9.79 & \ValSecnd{25.76} & {25.61} & \Valbest{25.81} \\
		%			& RMSE & 0.1275 & 0.1045 & 0.2088 & 0.1614 & 0.3378 & & & 0.1232 & \ValSecnd{0.0205} & {0.0208} & \Valbest{0.0203} \\
		%			& Ps   & 0.46 & 0.51 & 0.29 & 0.39 & 0.21 & & & 0.47 & \Valbest{0.89} & \Valbest{0.89} & \Valbest{0.90} \\
		%			
		%			& MPSNR & 30.73 & 38.20 & 28.88 & 29.28 & 13.11 & & & 29.75 & \ValSecnd{43.69} & 42.38 & \Valbest{43.97} \\
		%			& HMSSIM & 0.8505 & 0.9573 & 0.8003 & 0.8115 & 0.3799 & & & 0.8259 & \ValSecnd{0.9884} & 0.9844 & \Valbest{0.9894} \\
		%			\cmidrule(lr){1-13}
		%			
		%			\multirow{5}{*}{Case 5} 
		%			& Setup & & \begin{tabular}{c}
			%				0.001, \\ 0.001, \\ 0.1
			%			\end{tabular} &  &  &  &  &  &  &  &  &  \\
		%			& SRE  & 10.68 & 7.86 & 4.85 & 9.61 & 0.56 & & & 12.04 & \ValSecnd{23.85} & {23.71} & \Valbest{24.00} \\
		%			& RMSE & 0.1096 & 0.1418 & 0.1860 & 0.1264 & 0.3424 & & & 0.0965 & \ValSecnd{0.0252} & {0.0255} & \Valbest{0.0247} \\
		%			& Ps   & 0.50 & 0.43 & 0.34 & 0.46 & 0.16 & & & 0.53 & \ValSecnd{0.82} & \ValSecnd{0.82} & \Valbest{0.84} \\
		%			
		%			& MPSNR & 32.93 & 35.52 & 31.16 & 31.81 & 11.64 & & & 32.37 & \ValSecnd{41.33} & 40.13 & \Valbest{41.76} \\
		%			& MSSIM & 0.8908 & 0.9338 & 0.8534 & 0.8649 & 0.4211 & & & 0.8790 & \ValSecnd{0.9850} & 0.9792 & \Valbest{0.9870} \\
		%			\cmidrule(lr){1-13}
		%			
		%			\multirow{5}{*}{Case 6} 
		%			& Setup & & \begin{tabular}{c}
			%				0.001, \\ 0.001, \\ 0.1
			%			\end{tabular} &  &  &  &  &  &  &  &  &  \\
		%			& SRE  & 9.79 & 5.83 & 4.16 & 8.10 & 0.99 & & & 11.05 & \Valbest{20.13} & \ValSecnd{19.72} & 19.63 \\
		%			& RMSE & 0.1209 & 0.1720 & 0.1981 & 0.1471 & 0.3259 & & & 0.1075 & \Valbest{0.0377} & \ValSecnd{0.0393} & 0.0396 \\
		%			& Ps   & 0.47 & 0.36 & 0.31 & 0.42 & 0.23 & & & 0.50 & \ValSecnd{0.79} & \Valbest{0.80} & \ValSecnd{0.82} \\
		%			
		%			& MPSNR & 31.85 & 32.35 & 30.13 & 30.62 & 13.87 & & & 31.19 & \ValSecnd{38.85} & 36.95 & \Valbest{39.44} \\
		%			& MSSIM & 0.8615 & 0.8702 & 0.8191 & 0.8294 & 0.4129 & & & 0.8442 & \ValSecnd{0.9702} & 0.9527 & \Valbest{0.9753} \\
		%			\cmidrule(lr){1-13}
		%			
		%			\multirow{5}{*}{Case 6} 
		%			& Setup & & \begin{tabular}{c}
			%				0.001, \\ 0.001, \\ 0.1
			%			\end{tabular} &  &  &  &  &  &  &  &  & \\
		%			& SRE  & 9.79 & 5.83 & 4.16 & 8.10 & 0.99 & & & 11.05 & \Valbest{20.13} & \ValSecnd{19.72} & 19.63 \\
		%			& RMSE & 0.1209 & 0.1720 & 0.1981 & 0.1471 & 0.3259 & & & 0.1075 & \Valbest{0.0377} & \ValSecnd{0.0393} & 0.0396 \\
		%			& Ps   & 0.47 & 0.36 & 0.31 & 0.42 & 0.23 & & & 0.50 & \ValSecnd{0.79} & \Valbest{0.80} & \ValSecnd{0.82} \\
		%			
		%			& MPSNR & 31.85 & 32.35 & 30.13 & 30.62 & 13.87 & & & 31.19 & \ValSecnd{38.85} & 36.95 & \Valbest{39.44} \\
		%			& MSSIM & 0.8615 & 0.8702 & 0.8191 & 0.8294 & 0.4129 & & & 0.8442 & \ValSecnd{0.9702} & 0.9527 & \Valbest{0.9753} \\
		%			\cmidrule(lr){1-13}
		%			
		%			\multirow{5}{*}{Case 6} 
		%			& Setup & & \begin{tabular}{c}
			%				0.001, \\ $10^{-2}$, \\ 0.1
			%			\end{tabular} &  &  &  &  &  &  &  &  & \\
		%			& SRE  & 9.79 & 5.83 & 4.16 & 8.10 & 0.99 & & & 11.05 & \Valbest{20.13} & \ValSecnd{19.72} & 19.63 \\
		%			& RMSE & 0.1209 & 0.1720 & 0.1981 & 0.1471 & 0.3259 & & & 0.1075 & \Valbest{0.0377} & \ValSecnd{0.0393} & 0.0396 \\
		%			& Ps   & 0.47 & 0.36 & 0.31 & 0.42 & 0.23 & & & 0.50 & \ValSecnd{0.79} & \Valbest{0.80} & \ValSecnd{0.82} \\
		%			
		%			& MPSNR & 31.85 & 32.35 & 30.13 & 30.62 & 13.87 & & & 31.19 & \ValSecnd{38.85} & 36.95 & \Valbest{39.44} \\
		%			& MSSIM & 0.8615 & 0.8702 & 0.8191 & 0.8294 & 0.4129 & & & 0.8442 & \ValSecnd{0.9702} & 0.9527 & \Valbest{0.9753} \\
		%			\bottomrule
		%		\end{tabular}
	%	}
%\end{table*}


\begin{table*}[!h]
	\color{blue}
	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM in the Experiments Using \textit{Synth 1}.}
	\vspace{-1mm}
	\label{tab:result_synth_Legendre}
	\centering
	%	\scriptsize
	\scalebox{0.75}{
		\begin{tabular}{ccccccccccccc} \toprule
			\multirow{3}{*}{ Noise } & \multirow{3}{*}{Metrics}& \multicolumn{11}{c}{Methods}\\ 
			\cmidrule(lr){3-13}
			& & CLSUnSAL & JSTV & RSSUn-TV & LGSU & UnDIP & EGU-Net & RDSWSU & MdLRR & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
			& & \cite{iordache2014collaborative} & \cite{aggarwal2016hyperspectral} & \cite{wang2019row} & \cite{shen2022superpixel} & \cite{UnDIP_RastiB_2022} & \cite{hong2022endmember} & \cite{rs_Deng_RobustDual_2023} & \cite{MDLRR_WuLing_2023} & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
			%			& & $\lambda$ & $\lambda_{1},\lambda_{2},\lambda_{3}$ & $\lambda, \lambda_{TV}$ & $\lambda_{g}, \lambda_{l}$ & - & - & $\lambda$ & $\lambda, \tau$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ \\ 
			
			\midrule
			\multirow{6}{*}{Case 1} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-3}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   16.22 &   15.73 &   22.15 &   16.73 &    2.88 &   -5.52 &   16.38 &   18.96 &   \Valbest{24.31} &   21.84 &   \ValSecnd{23.52} \\ 
			& RMSE &   0.0385 &   0.0388 &   0.0197 &   0.0391 &   0.1417 &   0.2489 &   0.0398 &   0.0284 &   \Valbest{0.0153} &   0.0200 &   \ValSecnd{0.0167} \\ 
			& Ps   &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   0.59 &   0.01 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   45.23 &   38.35 &   46.53 &   45.09 &   23.92 &   15.32 &   45.17 &   45.59 &   \Valbest{54.23} &   \ValSecnd{49.34} &   47.74 \\ 
			& MSSIM &   0.9775 &   0.9164 &   0.9840 &   0.9768 &   0.8096 &   0.4255 &   0.9766 &   0.9804 &   \Valbest{0.9988} &   \ValSecnd{0.9937} &   0.9886 \\ 
			\midrule 
			
			\multirow{6}{*}{Case 2} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-1}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   12.57 &   11.35 &   14.22 &   14.91 &    0.42 &   -5.59 &   13.12 &   16.24 &   \Valbest{21.64} &   20.19 &   \ValSecnd{20.84} \\ 
			& RMSE &   0.0569 &   0.0615 &   0.0485 &   0.0484 &   0.1892 &   0.2510 &   0.0567 &   0.0393 &   \Valbest{0.0206} &   0.0240 &   \ValSecnd{0.0226} \\ 
			& Ps   &   0.98 &   \Valbest{1.00} &   \Valbest{1.00} &   0.99 &   0.50 &   0.01 &   0.97 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   40.17 &   34.04 &   39.90 &   39.74 &   19.76 &   15.25 &   39.67 &   39.91 &   \Valbest{49.20} &   \ValSecnd{43.39} &   41.70 \\ 
			& MSSIM &   0.9356 &   0.8270 &   0.9338 &   0.9298 &   0.6906 &   0.3899 &   0.9261 &   0.9327 &   \Valbest{0.9959} &   \ValSecnd{0.9735} &   0.9572 \\ 
			\midrule 
			
			\multirow{6}{*}{Case 3} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-1}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   11.28 &   15.18 &    7.63 &   13.13 &   -1.03 &   -5.62 &   11.58 &   14.64 &   \Valbest{23.92} &   21.06 &   \ValSecnd{23.73} \\ 
			& RMSE &   0.0646 &   0.0411 &   0.1051 &   0.0583 &   0.2085 &   0.2512 &   0.0790 &   0.0494 &   \Valbest{0.0159} &   0.0218 &   \ValSecnd{0.0162} \\ 
			& Ps   &   0.97 &   \Valbest{1.00} &   0.85 &   0.98 &   0.32 &   0.01 &   0.96 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   37.77 &   38.32 &   37.09 &   37.30 &   17.82 &   15.24 &   36.15 &   37.82 &   \Valbest{50.54} &   \ValSecnd{48.43} &   46.82 \\ 
			& MSSIM &   0.9066 &   0.9204 &   0.8957 &   0.8919 &   0.6237 &   0.3827 &   0.9239 &   0.9087 &   \Valbest{0.9949} &   \ValSecnd{0.9922} &   0.9860 \\ 
			\midrule 
			
			\multirow{6}{*}{Case 4} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-1}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    9.10 &   14.79 &    4.45 &   10.19 &   -1.62 &   -5.66 &   10.25 &   12.23 &   \Valbest{23.59} &   21.89 &   \ValSecnd{23.31} \\ 
			& RMSE &   0.0809 &   0.0429 &   0.1558 &   0.0797 &   0.2123 &   0.2526 &   0.0918 &   0.0636 &   \Valbest{0.0166} &   0.0199 &   \ValSecnd{0.0172} \\ 
			& Ps   &   0.93 &   \Valbest{1.00} &   0.48 &   0.94 &   0.31 &   0.01 &   0.91 &   0.98 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   34.66 &   37.77 &   33.63 &   33.94 &   19.02 &   15.23 &   33.82 &   34.27 &   \Valbest{47.92} &   \ValSecnd{47.58 }&   45.63 \\ 
			& MSSIM &   0.8556 &   0.9084 &   0.8286 &   0.8275 &   0.6136 &   0.3774 &   0.8746 &   0.8448 &   \ValSecnd{0.9893} &   \Valbest{0.9900} &   0.9810 \\ 
			\midrule 
			
			\multirow{6}{*}{Case 5} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-1}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   10.48 &   13.43 &    8.03 &   12.19 &   -1.11 &   -5.61 &   11.28 &   13.96 &   \Valbest{21.38} &   \ValSecnd{21.02} &   19.96 \\ 
			& RMSE &   0.0703 &   0.0507 &   0.0964 &   0.0641 &   0.2058 &   0.2522 &   0.0819 &   0.0527 &   \Valbest{0.0211} &   \ValSecnd{0.0218} &   0.0244 \\ 
			& Ps   &   0.96 &   \Valbest{1.00} &   0.86 &   0.97 &   0.31 &   0.01 &   0.95 &   0.99 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   36.97 &   36.20 &   36.18 &   36.53 &   18.10 &   15.22 &   35.62 &   36.98 &   \Valbest{50.17} &   45.92 &   \ValSecnd{45.99} \\ 
			& MSSIM &   0.8951 &   0.9374 &   0.8800 &   0.8778 &   0.6443 &   0.3822 &   0.9151 &   0.8939 &   \Valbest{0.9983} &   0.9886 &   \ValSecnd{0.9893} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 6} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-1}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    9.72 &   10.91 &    6.50 &   12.21 &    0.22 &   -5.65 &   11.21 &   13.31 &   \Valbest{17.14} &   14.86 &   \ValSecnd{16.80} \\ 
			& RMSE &   0.0764 &   0.0670 &   0.1173 &   0.0656 &   0.1763 &   0.2521 &   0.0812 &   0.0563 &   \Valbest{0.0339} &   0.0425 &   \ValSecnd{0.0350} \\ 
			& Ps   &   0.93 &   \Valbest{1.00} &   0.71 &   0.97 &   0.37 &   0.01 &   0.95 &   0.99 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   35.82 &   31.08 &   35.01 &   35.58 &   19.28 &   15.23 &   35.23 &   35.76 &   41.22 &   \Valbest{42.52} &   \ValSecnd{42.03} \\ 
			& MSSIM &   0.8661 &   0.8674 &   0.8454 &   0.8515 &   0.5572 &   0.3818 &   0.8849 &   0.8610 &   0.9560 &   \Valbest{0.9741} &   \ValSecnd{0.9660} \\ 
			\midrule 
			
			
			\multirow{6}{*}{Case 7} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-1}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   10.49 &   10.68 &    9.73 &   12.92 &   -0.87 &   -5.63 &   12.19 &   14.60 &   \ValSecnd{16.71} &   16.66 &   \Valbest{17.48} \\ 
			& RMSE &   0.0715 &   0.0700 &   0.0803 &   0.0607 &   0.1991 &   0.2516 &   0.0734 &   0.0493 &   0.0357 &   \ValSecnd{0.0351} &   \Valbest{0.0323} \\ 
			& Ps   &   0.94 &   0.99 &   0.93 &   0.98 &   0.34 &   0.01 &   0.97 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   36.88 &   30.34 &   35.99 &   36.31 &   20.45 &   15.28 &   35.56 &   36.73 &   \ValSecnd{39.64} &   39.58 &   \Valbest{39.78} \\ 
			& MSSIM &   0.8779 &   0.8063 &   0.8578 &   0.8612 &   0.5501 &   0.3838 &   0.9005 &   0.8740 &   0.9339 &   \ValSecnd{0.9378} &   \Valbest0.9406 \\ 
			\midrule 
			
			\multirow{6}{*}{Case 8} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-1}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    8.78 &    8.81 &    5.53 &   11.15 &   -1.87 &   -5.64 &   11.01 &   12.05 &   \Valbest{14.96} &   11.89 &   \ValSecnd{14.08} \\ 
			& RMSE &   0.0851 &   0.0798 &   0.1314 &   0.0732 &   0.2121 &   0.2527 &   0.0839 &   0.0642 &   \Valbest{0.0427} &   0.0592 &   \ValSecnd{0.0468} \\ 
			& Ps   &   0.91 &   0.99 &   0.65 &   0.96 &   0.23 &   0.01 &   0.94 &   0.98 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   34.38 &   31.16 &   33.42 &   34.02 &   19.49 &   15.25 &   34.03 &   34.15 &   \ValSecnd{40.36} &   37.76 &   \Valbest{41.30} \\ 
			& MSSIM &   0.8292 &   0.7416 &   0.7969 &   0.8067 &   0.6387 &   0.3791 &   0.8517 &   0.8148 &   \ValSecnd{0.9518} &   0.9118 &   \Valbest0.9653 \\ 
			\bottomrule
		\end{tabular}
	}
\end{table*}






==> tab_tex/tab_result_synth_colored.tex <==
%\begin{table*}[!h]
%	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM in the Experiments Using \textit{Synth 2}.}
%	\vspace{-1mm}
%	\label{tab:result_synth}
%	\centering
%%	\scriptsize
%	\scalebox{0.95}{
	%		\begin{tabular}{cccccccccccc} \toprule
		%			\multirow{3}{*}{ Noise } & \multirow{3}{6em}{\centering Evaluation \\ Target}  & \multirow{3}{*}{Measures}& \multicolumn{9}{c}{Methods}\\ 
		%			\cmidrule(lr){4-12}
		%			& & & CLSUnSAL & JSTV & RSSUn-TV & LGSU & UnDIP & MdLRR & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
		%			& & & \cite{iordache2014collaborative} & \cite{aggarwal2016hyperspectral} & \cite{wang2019row} & \cite{shen2022superpixel} & \cite{UnDIP_RastiB_2022} & \cite{MDLRR_WuLing_2023} & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
		%			
		%			\midrule
		%			
		%			\multirow{5}{*}{Case 1} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & \Valbest{10.57} & 9.39 & 8.70  & 6.50 & 5.89 & 6.45 & 9.95 & \ValSecnd{9.98} & 9.96 \\
		%			& & RMSE & \Valbest{0.1081} & 0.1239 & 0.1342 & 0.1694 & {0.1853} & 0.1681 & 0.1162 & \ValSecnd{0.1158} & 0.1160 \\
		%			& & Ps   & 0.60 & 0.52 & 0.49 & 0.54 & 0.35 & 0.55 & 0.78 & \Valbest{0.79} & \Valbest{0.79} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 40.41 & 39.58 & 39.38 & 40.45 & 21.80 & 40.80 & \ValSecnd{42.12} & 41.69 & \Valbest{42.16} \\
		%			& HS image
		%			& MSSIM & 0.9870 & 0.9841 & 0.9833 & 0.9875 & 0.8409 & 0.9891 & \Valbest{0.9926} & 0.9912 & \ValSecnd{0.9925} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 2} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 7.97& 6.00 & 5.64 & 5.74 & 5.55 & 5.92 & 8.39 & \ValSecnd{8.45} & \Valbest{8.48} \\
		%			& & RMSE & 0.1459 & 0.1829 & 0.1907 & 0.1837 & 0.1928 & 0.1789 & 0.1390 & \ValSecnd{0.1381} & \Valbest{0.1376} \\
		%			& & Ps   & 0.49 & 0.39 & 0.38 & 0.45 & 0.34 & 0.46 & 0.61 & \ValSecnd{0.62} & \Valbest{0.63} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 35.10 & 34.10 & 34.01 & 34.88 & 22.02 & 35.32 & \ValSecnd{36.25} & 36.01 & \Valbest{36.51} \\
		%			& HS image
		%			& MSSIM & 0.9593 & 0.9485 & 0.9477 & 0.9562 & 0.8005 & 0.9612 & \ValSecnd{0.9715} & 0.9693 & \Valbest{0.9732} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 3} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 7.19 & 8.67 & 4.27 & 5.11 & 2.95 & 5.19 & \ValSecnd{9.73} & \Valbest{9.74} & 9.72 \\
		%			& & RMSE & 0.1596 & 0.1346 & 0.2233 & 0.1986 & 0.2601 & 0.1938 & \ValSecnd{0.1192} & \Valbest{0.1190} & \ValSecnd{0.1192} \\
		%			& & Ps   & 0.47 & 0.50 & 0.34 & 0.42 & 0.35 & 0.42 & 0.78 & \Valbest{0.79} & \ValSecnd{0.78} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 32.88 & 38.63 & 31.60 & 32.24 & 21.17 & 32.56 & \ValSecnd{41.30} & 40.89 & \Valbest{41.40} \\
		%			& HS image
		%			& MSSIM & 0.9423 & 0.9806 & 0.9235 & 0.9331 & 0.8355 & 0.9387 & \Valbest{0.9914} & 0.9898 & \Valbest{0.9914} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 4} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 6.22 & 8.43 & 3.02 & 3.73 & 2.28 & 5.00 & 9.70 & \Valbest{9.77} & \ValSecnd{9.76} \\
		%			& & RMSE & 0.1785 & 0.1384 & 0.2579 & 0.2465 & 0.2810 & 0.1997 & 0.1195 & \Valbest{0.1186} & \ValSecnd{0.1187} \\
		%			& & Ps   & 0.43 & 0.48 & 0.29 & 0.36 & 0.28 & 0.38 & 0.77 & \Valbest{0.78} & \Valbest{0.78} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 29.97 & 37.94 & 28.63 & 28.98 & 20.97 & 29.20 & \ValSecnd{40.63} & 40.20 & \Valbest{40.75} \\
		%			& HS image
		%			& MSSIM & 0.9093 & 0.9773 & 0.8775 & 0.8876 & 0.7972 & 0.8936 & \ValSecnd{0.9898} & 0.9880 & \Valbest{0.9899} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 5} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 6.84 & 6.36 & 4.01 & 4.77 & 2.77 & 5.42 & \ValSecnd{9.00} & \Valbest{9.02} & 8.99 \\
		%			& & RMSE & 0.1661 & 0.1756 & 0.2301 & 0.2108 & 0.2654 & 0.1880 & \ValSecnd{0.1295} & \Valbest{0.1293} & 0.1297 \\
		%			& & Ps   & 0.45 & 0.41 & 0.32 & 0.40 & 0.21 & 0.41 & \ValSecnd{0.74} & \Valbest{0.75} & \ValSecnd{0.74} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 32.34 & 35.46 & 31.00 & 31.55 & 19.63 & 31.80 & \ValSecnd{39.10} & 38.40 & \Valbest{39.32} \\
		%			& HS image
		%			& MSSIM & 0.9368 & 0.9640 & 0.9150 & 0.9242 & 0.7990 & 0.9295 & \ValSecnd{0.9880} & 0.9850 & \Valbest{0.9885} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 6} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 6.46 & 4.62 & 3.37 & 4.16 & 4.16 & 5.27 & \ValSecnd{7.94} & \Valbest{7.97} & 7.92 \\
		%			& & RMSE & 0.1736 & 0.2146 & 0.2477 & 0.2298 & 0.2261 & 0.1917 & \ValSecnd{0.1464} & \Valbest{0.1459} & 0.1468 \\
		%			& & Ps   & 0.43 & 0.34 & 0.30 & 0.37 & 0.30 & 0.40 & \ValSecnd{0.68} & \Valbest{0.69} & \ValSecnd{0.68} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 31.18 & 32.12 & 29.95 & 30.38 & 21.76 & 30.61 & \ValSecnd{35.97} & 35.09 & \Valbest{36.11} \\
		%			& HS image
		%			& MSSIM & 0.9175 & 0.9246 & 0.8926 & 0.9012 & 0.8032 & 0.9066 & \ValSecnd{0.9735} & 0.9641 & \Valbest{0.9737} \\
		%			\bottomrule
		%		\end{tabular}
	%	}
%%\end{table*}

\begin{table*}[!h]
	\color{blue}
	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM in the Experiments Using \textit{Synth 2}.}
	\vspace{-1mm}
	\label{tab:result_synth}
	\centering
	%	\scriptsize
	\scalebox{0.75}{
		\begin{tabular}{ccccccccccccc} \toprule
			\multirow{3}{*}{ Noise } & \multirow{3}{*}{Metrics}& \multicolumn{11}{c}{Methods}\\ 
			\cmidrule(lr){3-13}
			& & CLSUnSAL & JSTV & RSSUn-TV & LGSU & UnDIP & EGU-Net & RDSWSU & MdLRR & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
			& & \cite{iordache2014collaborative} & \cite{aggarwal2016hyperspectral} & \cite{wang2019row} & \cite{shen2022superpixel} & \cite{UnDIP_RastiB_2022} & \cite{hong2022endmember} & \cite{rs_Deng_RobustDual_2023} & \cite{MDLRR_WuLing_2023} & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
			%			& & $\lambda$ & $\lambda_{1},\lambda_{2},\lambda_{3}$ & $\lambda, \lambda_{TV}$ & $\lambda_{g}, \lambda_{l}$ & - & - & $\lambda$ & $\lambda, \tau$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ \\
			\midrule 
			
			\multirow{6}{*}{Case 1} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-3}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   18.06 &   16.65 &   19.03 &   19.78 &    1.88 &   -5.02 &   20.80 &   19.81 &   \Valbest{21.11} &   20.78 &   \ValSecnd{20.99} \\ 
			& RMSE &   0.0270 &   0.0318 &   0.0252 &   0.0236 &   0.1518 &   0.2272 &   0.0212 &   0.0235 &   \Valbest{0.0198} &   0.0206 &   \ValSecnd{0.0201} \\ 
			& Ps   &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   0.55 &   0.00 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   41.37 &   32.54 &   41.80 &   41.60 &   27.09 &   15.79 &   41.90 &   41.71 &   \Valbest{42.84} &   42.39 &   \ValSecnd{42.55} \\ 
			& MSSIM &   0.9889 &   0.9435 &   0.9870 &   0.9864 &   0.8702 &   0.3498 &   0.9871 &   0.9876 &   \Valbest{0.9911} &   0.9891 &   \ValSecnd{0.9897} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 2} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-4}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   15.49 &   13.97 &   13.99 &   16.01 &    0.60 &   -5.08 &   16.68 &   15.62 &   \Valbest{17.50} &   17.23 &   \ValSecnd{17.38} \\ 
			& RMSE &   0.0358 &   0.0425 &   0.0449 &   0.0365 &   0.1760 &   0.2308 &   0.0342 &   0.0377 &   \Valbest{0.0297} &   0.0308 &   \ValSecnd{0.0302} \\ 
			& Ps   &   \Valbest{1.00} &   0.99 &   \Valbest{1.00} &   \Valbest{1.00} &   0.48 &   0.00 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   38.11 &   30.06 &   37.29 &   37.46 &   24.74 &   15.25 &   37.58 &   37.52 &   \Valbest{39.00} &   38.35 &   \ValSecnd{38.51} \\ 
			& MSSIM &   0.9735 &   0.8983 &   0.9645 &   0.9654 &   0.8380 &   0.2937 &   0.9667 &   0.9665 &   \Valbest{0.9787} &   0.9731 &   \ValSecnd{0.9743} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 3} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   11.62 &   16.37 &   10.81 &   12.36 &    1.69 &   -5.08 &   14.32 &   12.50 &   \Valbest{20.80} &   20.46 &   \ValSecnd{20.71} \\ 
			& RMSE &   0.0529 &   0.0326 &   0.0620 &   0.0529 &   0.1586 &   0.2319 &   0.0436 &   0.0514 &   \Valbest{0.0204} &   0.0213 &   \ValSecnd{0.0207} \\ 
			& Ps   &   \Valbest{1.00} &   \Valbest{1.00} &   0.97 &   0.98 &   0.62 &   0.00 &   \Valbest{1.00} &   0.99 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   33.78 &   32.31 &   33.71 &   33.78 &   27.65 &   14.98 &   34.19 &   33.89 &   \Valbest{42.24} &   41.90 &   \ValSecnd{42.06} \\ 
			& MSSIM &   0.9525 &   0.9444 &   0.9419 &   0.9421 &   0.8395 &   0.2635 &   0.9477 &   0.9445 &   \Valbest{0.9902} &   0.9883 &   \ValSecnd{0.9889} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 4} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    8.49 &   15.93 &    7.29 &    9.18 &   -0.08 &   -5.08 &   11.89 &    9.17 &   \Valbest{19.02} &   18.65 &   \ValSecnd{18.92} \\ 
			& RMSE &   0.0723 &   0.0344 &   0.0910 &   0.0732 &   0.1784 &   0.2332 &   0.0565 &   0.0722 &   \Valbest{0.0251} &   0.0262 &   \ValSecnd{0.0254} \\ 
			& Ps   &   0.97 &   \Valbest{1.00} &   0.88 &   0.94 &   0.43 &   0.00 &   0.98 &   0.95 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   30.06 &   31.42 &   29.91 &   30.03 &   24.84 &   14.71 &   30.48 &   30.07 &   \Valbest{41.30} &   40.80 &   \ValSecnd{40.97} \\ 
			& MSSIM &   0.9143 &   0.9299 &   0.8993 &   0.9001 &   0.7894 &   0.2472 &   0.9096 &   0.9025 &   \Valbest{0.9871} &   0.9844 &   \ValSecnd{0.9852} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 5} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   11.95 &   17.36 &   11.27 &   12.68 &    1.63 &   -5.09 &   14.25 &   12.86 &   \Valbest{21.52} &   21.27 &   \ValSecnd{21.42} \\ 
			& RMSE &   0.0513 &   0.0294 &   0.0590 &   0.0512 &   0.1553 &   0.2323 &   0.0439 &   0.0495 &   \Valbest{0.0189} &   0.0195 &   \ValSecnd{0.0191} \\ 
			& Ps   &   \Valbest{1.00} &   \Valbest{1.00} &   0.98 &   0.99 &   0.53 &   0.00 &   \Valbest{1.00} &   0.99 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   33.88 &   32.87 &   33.84 &   33.90 &   25.62 &   14.95 &   34.24 &   34.02 &   \Valbest{42.83} &   42.51 &   \ValSecnd{42.65} \\ 
			& MSSIM &   0.9530 &   0.9509 &   0.9428 &   0.9429 &   0.8397 &   0.2607 &   0.9484 &   0.9453 &   \Valbest{0.9909} &   0.9890 &   \ValSecnd{0.9895} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 6} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-1}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   11.08 &   13.75 &    9.03 &   11.44 &   -0.74 &   -5.10 &   13.62 &   11.43 &   \Valbest{17.96} &   17.55 &   \ValSecnd{17.81} \\ 
			& RMSE &   0.0564 &   0.0434 &   0.0776 &   0.0599 &   0.1962 &   0.2331 &   0.0477 &   0.0584 &   \Valbest{0.0282} &   0.0296 &   \ValSecnd{0.0288} \\ 
			& Ps   &   0.99 &   0.99 &   0.92 &   0.97 &   0.39 &   0.00 &   0.99 &   0.98 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   33.06 &   29.63 &   32.71 &   32.84 &   26.02 &   14.78 &   33.28 &   32.93 &   \Valbest{38.55} &   38.14 &   \ValSecnd{38.24} \\ 
			& MSSIM &   0.9401 &   0.8945 &   0.9254 &   0.9282 &   0.8051 &   0.2515 &   0.9327 &   0.9284 &   \Valbest{0.9798} &   0.9724 &   \ValSecnd{0.9732} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 7} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   12.85 &   11.74 &   10.75 &   13.58 &    0.68 &   -5.10 &   14.65 &   13.25 &   15.49 &   \ValSecnd{15.68} &   \Valbest{16.05} \\ 
			& RMSE &   0.0477 &   0.0531 &   0.0649 &   0.0483 &   0.1714 &   0.2326 &   0.0437 &   0.0495 &   0.0370 &   \ValSecnd{0.0362} &   \Valbest{0.0348} \\ 
			& Ps   &   \Valbest{1.00} &   0.99 &   0.96 &   0.99 &   0.46 &   0.00 &   0.99 &   0.99 &   \Valbest{1.00} &   \Valbest{1.00} &   \Valbest{1.00} \\ 
			& MPSNR &   35.24 &   27.62 &   34.22 &   34.53 &   25.30 &   14.92 &   34.93 &   34.63 &   \Valbest{36.76} &   35.77 &   \ValSecnd{36.11} \\ 
			& MSSIM &   0.9488 &   0.8577 &   0.9334 &   0.9365 &   0.8282 &   0.2464 &   0.9425 &   0.9382 &   \Valbest{0.9664} &   0.9531 &   \ValSecnd{0.9570} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 8} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-1}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    9.67 &   10.96 &    7.13 &   10.72 &    3.34 &   -5.09 &   12.50 &   10.12 &   12.99 &   \ValSecnd{14.26} &   \Valbest{14.60} \\ 
			& RMSE &   0.0655 &   0.0576 &   0.0976 &   0.0650 &   0.1275 &   0.2333 &   0.0547 &   0.0682 &   0.0471 &   \ValSecnd{0.0415} &   \Valbest{0.0405} \\ 
			& Ps   &   0.98 &   0.98 &   0.85 &   0.96 &   0.66 &   0.00 &   0.98 &   0.95 &   0.98 &   0.99 &   0.99 \\ 
			& MPSNR &   31.72 &   26.70 &   31.17 &   31.50 &   27.93 &   14.73 &   32.01 &   31.48 &   34.17 &   \ValSecnd{35.12} &   \Valbest{35.21} \\ 
			& MSSIM &   0.9172 &   0.8258 &   0.8977 &   0.9054 &   0.8409 &   0.2389 &   0.9102 &   0.9029 &   \Valbest{0.9575} &   0.9517 &   \ValSecnd{0.9525} \\ 
			\bottomrule
		\end{tabular}
	}
\end{table*}



==> tab_tex/tab_result_urban_colored.tex <==
%\begin{table*}[t]
%	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM in the Experiments Using \textit{Synth 1}.}
%	\vspace{-1mm}
%	\label{tab:result_synth_Legendre}
%	\centering
%%	\scriptsize
%	\scalebox{0.95}{
	%		\begin{tabular}{cccccccccccc} \toprule
		%			\multirow{3}{*}{ Noise } & \multirow{3}{6em}{\centering Evaluation \\ Target}  & \multirow{3}{*}{Measures}& \multicolumn{9}{c}{Methods}\\ 
		%			\cmidrule(lr){4-12}
		%			& & & CLSUnSAL & JSTV & RSSUn-TV & LGSU & UnDIP & MdLRR & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
		%			& & & \cite{iordache2014collaborative} & \cite{aggarwal2016hyperspectral} & \cite{wang2019row} & \cite{shen2022superpixel} & \cite{UnDIP_RastiB_2022} & \cite{MDLRR_WuLing_2023} & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
		%			
		%			\midrule
		%			
		%			\multirow{5}{*}{Case 1} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 16.50 & 12.95 & 11.39  & 16.59 & 0.58 & 17.98 & \Valbest{27.22} & \ValSecnd{27.02} & 26.99 \\
		%			& & RMSE & 0.0590 & 0.0840 & 0.0992 & 0.0608 & 0.3414 & 0.0524 & \Valbest{0.0173} & \ValSecnd{0.0177} & \ValSecnd{0.0177} \\
		%			& & Ps   & 0.68 & 0.56 & 0.53 & 0.64 & 0.18 & 0.66 & \Valbest{0.92} & \Valbest{0.92} & \Valbest{0.92} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 41.26 & 39.94 & 39.70 & 41.19 & 11.80 & 41.90 & \ValSecnd{46.09} & 44.49 & \Valbest{46.26} \\
		%			& HS image
		%			& MSSIM & 0.9771 & 0.9706 & 0.9693 & 0.9754 & 0.4659 & 0.9821 & \ValSecnd{0.9936} & 0.9906 & \Valbest{0.9940} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 2} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 12.81 & 7.83 & 7.13 & 12.73 & 0.88 & 16.71 & \ValSecnd{21.85} & 21.84 & \Valbest{22.12} \\
		%			& & RMSE & 0.0889 & 0.1424 & 0.1530 & 0.0923 & 0.3302 & 0.0588 & \ValSecnd{0.0318} & \ValSecnd{0.0318} & \Valbest{0.0308} \\
		%			& & Ps   & 0.55 & 0.41 & 0.40 & 0.52 & 0.19 & 0.63 & \ValSecnd{0.80} & \ValSecnd{0.80} & \Valbest{0.81} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 36.13 & 34.51 & 34.42 & 35.39 & 12.68 & 36.07 & \ValSecnd{38.86} & 37.91 & \Valbest{39.19} \\
		%			& HS image
		%			& MSSIM & 0.9322 & 0.9114 & 0.9101 & 0.9213 & 0.4138 & 0.9327 & \ValSecnd{0.9660} & 0.9585 & \Valbest{0.9692} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 3} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 11.42 & 11.97 & 5.72 & 10.72 & 0.87 & 13.84 & \Valbest{26.40} & {26.04} & \ValSecnd{26.07} \\
		%			& & RMSE & 0.1018 & 0.0931 & 0.1720 & 0.1138 & 0.3305 & 0.0802 & \Valbest{0.0190} & {0.0197} & \ValSecnd{0.0196} \\
		%			& & Ps   & 0.53 & 0.53 & 0.36 & 0.49 & 0.18 & 0.58 & \Valbest{0.91} & \ValSecnd{0.90} & \Valbest{0.91} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 33.82 & 39.02 & 31.94 & 32.73 & 13.36 & 33.25 & \ValSecnd{45.43} & 43.64 & \Valbest{45.58} \\
		%			& HS image
		%			& MSSIM & 0.9026 & 0.9641 & 0.8688 & 0.8821 & 0.3607 & 0.8943 & \ValSecnd{0.9926} & 0.9885 & \Valbest{0.9930} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 4} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 9.20 & 10.87 & 3.47 & 7.18 & 0.68 & 9.79 & \ValSecnd{25.76} & {25.61} & \Valbest{25.81} \\
		%			& & RMSE & 0.1275 & 0.1045 & 0.2088 & 0.1614 & 0.3378 & 0.1232 & \ValSecnd{0.0205} & {0.0208} & \Valbest{0.0203} \\
		%			& & Ps   & 0.46 & 0.51 & 0.29 & 0.39 & 0.21 & 0.47 & \Valbest{0.89} & \Valbest{0.89} & \Valbest{0.90} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 30.73 & 38.20 & 28.88 & 29.28 & 13.11 & 29.75 & \ValSecnd{43.69} & 42.38 & \Valbest{43.97} \\
		%			& HS image
		%			& MSSIM & 0.8505 & 0.9573 & 0.8003 & 0.8115 & 0.3799 & 0.8259 & \ValSecnd{0.9884} & 0.9844 & \Valbest{0.9894} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 5} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 10.68 & 7.86 & 4.85 & 9.61 & 0.56 & 12.04 & \ValSecnd{23.85} & {23.71} & \Valbest{24.00} \\
		%			& & RMSE & 0.1096 & 0.1418 & 0.1860 & 0.1264 & 0.3424 & 0.0965 & \ValSecnd{0.0252} & {0.0255} & \Valbest{0.0247} \\
		%			& & Ps   & 0.50 & 0.43 & 0.34 & 0.46 & 0.16 & 0.53 & \ValSecnd{0.82} & \ValSecnd{0.82} & \Valbest{0.84} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 32.93 & 35.52 & 31.16 & 31.81 & 11.64 & 32.37 & \ValSecnd{41.33} & 40.13 & \Valbest{41.76} \\
		%			& HS image
		%			& MSSIM & 0.8908 & 0.9338 & 0.8534 & 0.8649 & 0.4211 & 0.8790 & \ValSecnd{0.9850} & 0.9792 & \Valbest{0.9870} \\
		%			\cmidrule(lr){1-12}
		%			
		%			\multirow{5}{*}{Case 6} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 9.79 & 5.83 & 4.16 & 8.10 & 0.99 & 11.05 & \Valbest{20.13} & \ValSecnd{19.72} & 19.63 \\
		%			& & RMSE & 0.1209 & 0.1720 & 0.1981 & 0.1471 & 0.3259 & 0.1075 & \Valbest{0.0377} & \ValSecnd{0.0393} & 0.0396 \\
		%			& & Ps   & 0.47 & 0.36 & 0.31 & 0.42 & 0.23 & 0.50 & \ValSecnd{0.79} & \Valbest{0.80} & \ValSecnd{0.82} \\
		%			\cmidrule(lr){2-12}
		%			& Reconstructed
		%			& MPSNR & 31.85 & 32.35 & 30.13 & 30.62 & 13.87 & 31.19 & \ValSecnd{38.85} & 36.95 & \Valbest{39.44} \\
		%			& HS image
		%			& MSSIM & 0.8615 & 0.8702 & 0.8191 & 0.8294 & 0.4129 & 0.8442 & \ValSecnd{0.9702} & 0.9527 & \Valbest{0.9753} \\
		%			\bottomrule
		%		\end{tabular}
	%	}
%\end{table*}


%\begin{table*}[!h]
%	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM in the Experiments Using \textit{Synth 1}.}
%	\vspace{-1mm}
%	\label{tab:result_synth_Legendre}
%	\centering
%	%	\scriptsize
%	\scalebox{0.85}{
	%		\begin{tabular}{ccccccccccccc} \toprule
		%			\multirow{3}{*}{ Noise } & \multirow{3}{*}{Metrics}& \multicolumn{11}{c}{Methods}\\ 
		%			\cmidrule(lr){3-13}
		%			& & CLSUnSAL & JSTV & RSSUn-TV & LGSU & UnDIP & EGU-Net & RDSWSU & MdLRR & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
		%			& & \cite{iordache2014collaborative} & \cite{aggarwal2016hyperspectral} & \cite{wang2019row} & \cite{shen2022superpixel} & \cite{UnDIP_RastiB_2022} & \cite{hong2022endmember} & \cite{rs_Deng_RobustDual_2023} & \cite{MDLRR_WuLing_2023} & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
		%%			& & $\lambda$ & $\lambda_{1},\lambda_{2},\lambda_{3}$ & $\lambda, \lambda_{TV}$ & $\lambda_{g}, \lambda_{l}$ & - & - & $\lambda$ & $\lambda, \tau$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ \\ 
		%			
		%			\midrule
		%			
		%			\multirow{6}{*}{Case 1} 
		%			& Setup & \begin{tabular}{c}
			%				\hspace{-4mm} $\lambda = 1 * 10^{-2}$ \hspace{-4mm}
			%			\end{tabular} & \begin{tabular}{c}
			%				\hspace{-4mm}$\lambda_{1} = 1 * 10^{-2}$\hspace{-4mm}, \\ \hspace{-4mm}$\lambda_{2} = 0.001$\hspace{-4mm}, \\ \hspace{-4mm}$\lambda_{3} = 0.1$\hspace{-4mm}
			%			\end{tabular} &  &  &  &  &  &  &  &  &  \\
		%			& SRE  & 16.50 & 12.95 & 11.39  & 16.59 & 0.58 & & & 17.98 & \Valbest{27.22} & \ValSecnd{27.02} & 26.99 \\
		%			& RMSE & 0.0590 & 0.0840 & 0.0992 & 0.0608 & 0.3414 & & & 0.0524 & \Valbest{0.0173} & \ValSecnd{0.0177} & \ValSecnd{0.0177} \\
		%			& Ps   & 0.68 & 0.56 & 0.53 & 0.64 & 0.18 & & & 0.66 & \Valbest{0.92} & \Valbest{0.92} & \Valbest{0.92} \\
		%			
		%			& MPSNR & 41.26 & 39.94 & 39.70 & 41.19 & 11.80 & & & 41.90 & \ValSecnd{46.09} & 44.49 & \Valbest{46.26} \\
		%			& MSSIM & 0.9771 & 0.9706 & 0.9693 & 0.9754 & 0.4659 & & & 0.9821 & \ValSecnd{0.9936} & 0.9906 & \Valbest{0.9940} \\
		%			\cmidrule(lr){1-13}
		%			
		%			\multirow{5}{*}{Case 2} 
		%			& Setup & & \begin{tabular}{c}
			%				0.001, \\ 0.001, \\ 0.1
			%			\end{tabular} &  &  &  &  &  &  &  &  &  \\
		%			& SRE  & 12.81 & 7.83 & 7.13 & 12.73 & 0.88 & & & 16.71 & \ValSecnd{21.85} & 21.84 & \Valbest{22.12} \\
		%			& RMSE & 0.0889 & 0.1424 & 0.1530 & 0.0923 & 0.3302 & & & 0.0588 & \ValSecnd{0.0318} & \ValSecnd{0.0318} & \Valbest{0.0308} \\
		%			& Ps   & 0.55 & 0.41 & 0.40 & 0.52 & 0.19 & & & 0.63 & \ValSecnd{0.80} & \ValSecnd{0.80} & \Valbest{0.81} \\
		%			
		%			& MPSNR & 36.13 & 34.51 & 34.42 & 35.39 & 12.68 & & & 36.07 & \ValSecnd{38.86} & 37.91 & \Valbest{39.19} \\
		%			& MSSIM & 0.9322 & 0.9114 & 0.9101 & 0.9213 & 0.4138 & & & 0.9327 & \ValSecnd{0.9660} & 0.9585 & \Valbest{0.9692} \\
		%			\cmidrule(lr){1-13}
		%			
		%			\multirow{5}{*}{Case 3} 
		%			& Setup & & \begin{tabular}{c}
			%				0.001, \\ 0.001, \\ 0.1
			%			\end{tabular} &  &  &  &  &  &  &  &  &  \\
		%			& SRE  & 11.42 & 11.97 & 5.72 & 10.72 & 0.87 & & & 13.84 & \Valbest{26.40} & {26.04} & \ValSecnd{26.07} \\
		%			& RMSE & 0.1018 & 0.0931 & 0.1720 & 0.1138 & 0.3305 & & & 0.0802 & \Valbest{0.0190} & {0.0197} & \ValSecnd{0.0196} \\
		%			& Ps   & 0.53 & 0.53 & 0.36 & 0.49 & 0.18 & & & 0.58 & \Valbest{0.91} & \ValSecnd{0.90} & \Valbest{0.91} \\
		%			
		%			& MPSNR & 33.82 & 39.02 & 31.94 & 32.73 & 13.36 & & & 33.25 & \ValSecnd{45.43} & 43.64 & \Valbest{45.58} \\
		%			& MSSIM & 0.9026 & 0.9641 & 0.8688 & 0.8821 & 0.3607 & & & 0.8943 & \ValSecnd{0.9926} & 0.9885 & \Valbest{0.9930} \\
		%			\cmidrule(lr){1-13}
		%			
		%			\multirow{5}{*}{Case 4} 
		%			& Setup & & \begin{tabular}{c}
			%				0.001, \\ 0.001, \\ 0.1
			%			\end{tabular} &  &  &  &  &  &  &  &  &  \\
		%			& SRE  & 9.20 & 10.87 & 3.47 & 7.18 & 0.68 & & & 9.79 & \ValSecnd{25.76} & {25.61} & \Valbest{25.81} \\
		%			& RMSE & 0.1275 & 0.1045 & 0.2088 & 0.1614 & 0.3378 & & & 0.1232 & \ValSecnd{0.0205} & {0.0208} & \Valbest{0.0203} \\
		%			& Ps   & 0.46 & 0.51 & 0.29 & 0.39 & 0.21 & & & 0.47 & \Valbest{0.89} & \Valbest{0.89} & \Valbest{0.90} \\
		%			
		%			& MPSNR & 30.73 & 38.20 & 28.88 & 29.28 & 13.11 & & & 29.75 & \ValSecnd{43.69} & 42.38 & \Valbest{43.97} \\
		%			& HMSSIM & 0.8505 & 0.9573 & 0.8003 & 0.8115 & 0.3799 & & & 0.8259 & \ValSecnd{0.9884} & 0.9844 & \Valbest{0.9894} \\
		%			\cmidrule(lr){1-13}
		%			
		%			\multirow{5}{*}{Case 5} 
		%			& Setup & & \begin{tabular}{c}
			%				0.001, \\ 0.001, \\ 0.1
			%			\end{tabular} &  &  &  &  &  &  &  &  &  \\
		%			& SRE  & 10.68 & 7.86 & 4.85 & 9.61 & 0.56 & & & 12.04 & \ValSecnd{23.85} & {23.71} & \Valbest{24.00} \\
		%			& RMSE & 0.1096 & 0.1418 & 0.1860 & 0.1264 & 0.3424 & & & 0.0965 & \ValSecnd{0.0252} & {0.0255} & \Valbest{0.0247} \\
		%			& Ps   & 0.50 & 0.43 & 0.34 & 0.46 & 0.16 & & & 0.53 & \ValSecnd{0.82} & \ValSecnd{0.82} & \Valbest{0.84} \\
		%			
		%			& MPSNR & 32.93 & 35.52 & 31.16 & 31.81 & 11.64 & & & 32.37 & \ValSecnd{41.33} & 40.13 & \Valbest{41.76} \\
		%			& MSSIM & 0.8908 & 0.9338 & 0.8534 & 0.8649 & 0.4211 & & & 0.8790 & \ValSecnd{0.9850} & 0.9792 & \Valbest{0.9870} \\
		%			\cmidrule(lr){1-13}
		%			
		%			\multirow{5}{*}{Case 6} 
		%			& Setup & & \begin{tabular}{c}
			%				0.001, \\ 0.001, \\ 0.1
			%			\end{tabular} &  &  &  &  &  &  &  &  &  \\
		%			& SRE  & 9.79 & 5.83 & 4.16 & 8.10 & 0.99 & & & 11.05 & \Valbest{20.13} & \ValSecnd{19.72} & 19.63 \\
		%			& RMSE & 0.1209 & 0.1720 & 0.1981 & 0.1471 & 0.3259 & & & 0.1075 & \Valbest{0.0377} & \ValSecnd{0.0393} & 0.0396 \\
		%			& Ps   & 0.47 & 0.36 & 0.31 & 0.42 & 0.23 & & & 0.50 & \ValSecnd{0.79} & \Valbest{0.80} & \ValSecnd{0.82} \\
		%			
		%			& MPSNR & 31.85 & 32.35 & 30.13 & 30.62 & 13.87 & & & 31.19 & \ValSecnd{38.85} & 36.95 & \Valbest{39.44} \\
		%			& MSSIM & 0.8615 & 0.8702 & 0.8191 & 0.8294 & 0.4129 & & & 0.8442 & \ValSecnd{0.9702} & 0.9527 & \Valbest{0.9753} \\
		%			\cmidrule(lr){1-13}
		%			
		%			\multirow{5}{*}{Case 6} 
		%			& Setup & & \begin{tabular}{c}
			%				0.001, \\ 0.001, \\ 0.1
			%			\end{tabular} &  &  &  &  &  &  &  &  & \\
		%			& SRE  & 9.79 & 5.83 & 4.16 & 8.10 & 0.99 & & & 11.05 & \Valbest{20.13} & \ValSecnd{19.72} & 19.63 \\
		%			& RMSE & 0.1209 & 0.1720 & 0.1981 & 0.1471 & 0.3259 & & & 0.1075 & \Valbest{0.0377} & \ValSecnd{0.0393} & 0.0396 \\
		%			& Ps   & 0.47 & 0.36 & 0.31 & 0.42 & 0.23 & & & 0.50 & \ValSecnd{0.79} & \Valbest{0.80} & \ValSecnd{0.82} \\
		%			
		%			& MPSNR & 31.85 & 32.35 & 30.13 & 30.62 & 13.87 & & & 31.19 & \ValSecnd{38.85} & 36.95 & \Valbest{39.44} \\
		%			& MSSIM & 0.8615 & 0.8702 & 0.8191 & 0.8294 & 0.4129 & & & 0.8442 & \ValSecnd{0.9702} & 0.9527 & \Valbest{0.9753} \\
		%			\cmidrule(lr){1-13}
		%			
		%			\multirow{5}{*}{Case 6} 
		%			& Setup & & \begin{tabular}{c}
			%				0.001, \\ $10^{-2}$, \\ 0.1
			%			\end{tabular} &  &  &  &  &  &  &  &  & \\
		%			& SRE  & 9.79 & 5.83 & 4.16 & 8.10 & 0.99 & & & 11.05 & \Valbest{20.13} & \ValSecnd{19.72} & 19.63 \\
		%			& RMSE & 0.1209 & 0.1720 & 0.1981 & 0.1471 & 0.3259 & & & 0.1075 & \Valbest{0.0377} & \ValSecnd{0.0393} & 0.0396 \\
		%			& Ps   & 0.47 & 0.36 & 0.31 & 0.42 & 0.23 & & & 0.50 & \ValSecnd{0.79} & \Valbest{0.80} & \ValSecnd{0.82} \\
		%			
		%			& MPSNR & 31.85 & 32.35 & 30.13 & 30.62 & 13.87 & & & 31.19 & \ValSecnd{38.85} & 36.95 & \Valbest{39.44} \\
		%			& MSSIM & 0.8615 & 0.8702 & 0.8191 & 0.8294 & 0.4129 & & & 0.8442 & \ValSecnd{0.9702} & 0.9527 & \Valbest{0.9753} \\
		%			\bottomrule
		%		\end{tabular}
	%	}
%\end{table*}


\begin{table*}[!h]
	\color{blue}
	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM in the Experiments Using \textit{Urban}.}
	\vspace{-1mm}
	\label{tab:result_real_Urban}
	\centering
	%	\scriptsize
	\scalebox{0.75}{
		\begin{tabular}{ccccccccccccc} \toprule
			\multirow{3}{*}{ Noise } & \multirow{3}{*}{Metrics}& \multicolumn{11}{c}{Methods}\\ 
			\cmidrule(lr){3-13}
			& & CLSUnSAL & JSTV & RSSUn-TV & LGSU & UnDIP & EGU-Net & RDSWSU & MdLRR & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
			& & \cite{iordache2014collaborative} & \cite{aggarwal2016hyperspectral} & \cite{wang2019row} & \cite{shen2022superpixel} & \cite{UnDIP_RastiB_2022} & \cite{hong2022endmember} & \cite{rs_Deng_RobustDual_2023} & \cite{MDLRR_WuLing_2023} & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
			%			& & $\lambda$ & $\lambda_{1},\lambda_{2},\lambda_{3}$ & $\lambda, \lambda_{TV}$ & $\lambda_{g}, \lambda_{l}$ & - & - & $\lambda$ & $\lambda, \tau$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ & $\lambda_{1},\lambda_{2},\alpha$ \\ 
			
			\midrule
			\multirow{6}{*}{Case 1} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-3}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &   13.07 &   -0.00 &   15.62 & \ValSecnd{  20.91} &    0.42 &   -2.81 & \Valbest{  24.94} &   18.28 &   15.92 &   14.49 &   14.74 \\ 
			& RMSE &   0.0105 &   2.1963 &   0.0081 & \ValSecnd{  0.0047} &   0.0336 &   0.0409 & \Valbest{  0.0029} &   0.0062 &   0.0078 &   0.0090 &   0.0088 \\ 
			& Ps   & \ValSecnd{  0.99} &   0.11 & \Valbest{  1.00} & \Valbest{  1.00} &   0.53 &   0.07 & \Valbest{  1.00} & \Valbest{  1.00} & \ValSecnd{  0.99} & \ValSecnd{  0.99} & \ValSecnd{  0.99} \\ 
			& MPSNR &   40.67 &  -45.31 &   40.88 & \ValSecnd{  42.44} &   24.71 &   15.70 & \Valbest{  43.78} &   40.05 &   37.93 &   41.74 &   41.91 \\ 
			& MSSIM &   0.9813 &   0.6266 &   0.9806 &   0.9859 &   0.8480 &   0.2748 & \Valbest{  0.9894} &   0.9791 &   0.9741 &   0.9854 & \ValSecnd{  0.9863} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 2} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-4}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    7.33 &   -0.00 &    8.91 &   12.88 &   -2.49 &   -7.34 & \Valbest{  19.15} & \ValSecnd{  12.98} &   12.62 &   10.90 &   11.37 \\ 
			& RMSE &   0.0191 &   2.1447 &   0.0165 &   0.0111 &   0.0389 &   0.0569 & \Valbest{  0.0057} &   0.0113 & \ValSecnd{  0.0110} &   0.0131 &   0.0126 \\ 
			& Ps   &   0.81 &   0.12 &   0.92 & \ValSecnd{  0.98} &   0.29 &   0.00 & \Valbest{  1.00} &   0.96 & \ValSecnd{  0.98} & \ValSecnd{  0.98} & \ValSecnd{  0.98} \\ 
			& MPSNR &   34.87 &  -45.10 &   34.39 &   35.69 &   21.98 &   13.21 & \Valbest{  37.83} &   33.83 &   35.25 &   35.77 & \ValSecnd{  36.05} \\ 
			& MSSIM &   0.9360 &   0.5726 &   0.9232 &   0.9382 &   0.7388 &   0.3409 & \Valbest{  0.9607} &   0.9306 & \ValSecnd{  0.9571} &   0.9448 &   0.9483 \\ 
			\midrule 
			
			\multirow{6}{*}{Case 3} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-3}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    5.06 &   -0.00 &    5.46 &   10.01 &   -5.38 &   -7.92 & \Valbest{  15.64} &    9.47 & \ValSecnd{  15.29} &   13.79 &   14.11 \\ 
			& RMSE &   0.0233 &   1.6567 &   0.0235 &   0.0149 &   0.0463 &   0.0561 & \ValSecnd{  0.0085} &   0.0161 & \Valbest{  0.0083} &   0.0097 &   0.0094 \\ 
			& Ps   &   0.72 &   0.23 &   0.74 & \ValSecnd{  0.93} &   0.02 &   0.00 & \Valbest{  0.99} &   0.90 & \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} \\ 
			& MPSNR &   31.03 &  -42.73 &   30.72 &   31.73 &   20.09 &   13.05 &   33.91 &   29.55 &   37.38 & \ValSecnd{  40.78} & \Valbest{  40.98} \\ 
			& MSSIM &   0.8842 &   0.8106 &   0.8656 &   0.8876 &   0.7273 &   0.3206 &   0.9320 &   0.8551 &   0.9712 & \ValSecnd{  0.9819} & \Valbest{  0.9831} \\ 
			\midrule 
			
			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			\multirow{6}{*}{Case 4} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{-1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    2.56 &    0.00 &    2.08 &    6.05 &   -5.08 &   -8.40 &   12.42 &    5.33 & \Valbest{  14.95} &   13.76 & \ValSecnd{  14.05} \\ 
			& RMSE &   0.0290 &   8.8367 &   0.0339 &   0.0219 &   0.0437 &   0.0555 &   0.0119 &   0.0243 & \Valbest{  0.0086} &   0.0097 & \ValSecnd{  0.0095} \\ 
			& Ps   &   0.60 &   0.72 &   0.43 &   0.79 &   0.11 &   0.00 & \ValSecnd{  0.97} &   0.72 & \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} \\ 
			& MPSNR &   27.58 &  -57.72 &   27.20 &   28.08 &   19.23 &   13.01 &   29.85 &   25.67 &   37.34 & \ValSecnd{  39.87} & \Valbest{  40.12} \\ 
			& MSSIM &   0.8119 &   0.5146 &   0.7824 &   0.8139 &   0.6811 &   0.2982 &   0.8767 &   0.7507 &   0.9713 & \ValSecnd{  0.9776} & \Valbest{  0.9792} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 5} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-3}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    4.47 &    0.00 &    4.44 &    8.99 &   -5.94 &   -8.13 & \Valbest{  15.21} &    8.34 & \ValSecnd{  10.38} &    9.59 &    9.59 \\ 
			& RMSE &   0.0247 &   9.6721 &   0.0262 &   0.0170 &   0.0466 &   0.0558 & \Valbest{  0.0089} &   0.0181 & \ValSecnd{  0.0138} &   0.0149 &   0.0148 \\ 
			& Ps   &   0.69 &   0.62 &   0.65 &   0.89 &   0.01 &   0.00 & \Valbest{  0.99} &   0.86 & \ValSecnd{  0.96} &   0.94 &   0.94 \\ 
			& MPSNR &   30.57 &  -58.27 &   30.16 &   31.14 &   17.69 &   13.03 &   33.48 &   28.88 &   30.36 & \ValSecnd{  37.42} & \Valbest{  37.43} \\ 
			& MSSIM &   0.8743 &   0.7935 &   0.8522 &   0.8736 &   0.6354 &   0.3098 &   0.9244 &   0.8400 &   0.8906 & \ValSecnd{  0.9677} & \Valbest{  0.9679} \\ 
			\midrule 
			
			\multirow{6}{*}{Case 6} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-3}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    3.65 &    0.00 &    3.20 &    7.48 &   -5.80 &   -8.10 & \Valbest{  14.37} &    6.85 & \ValSecnd{  10.02} &    8.59 &    8.69 \\ 
			& RMSE &   0.0269 &   9.5123 &   0.0303 &   0.0199 &   0.0484 &   0.0559 & \Valbest{  0.0098} &   0.0212 & \ValSecnd{  0.0144} &   0.0166 &   0.0165 \\ 
			& Ps   &   0.64 &   0.47 &   0.53 &   0.83 &   0.06 &   0.00 & \Valbest{  0.98} &   0.79 & \ValSecnd{  0.95} &   0.93 &   0.93 \\ 
			& MPSNR &   29.63 &  -58.13 &   29.08 &   30.01 &   18.89 &   13.26 &   32.55 &   27.29 & \Valbest{  34.34} &   33.87 & \ValSecnd{  34.18} \\ 
			& MSSIM &   0.8490 &   0.7094 &   0.8194 &   0.8423 &   0.6723 &   0.3455 &   0.9066 &   0.7968 & \Valbest{  0.9496} &   0.9227 & \ValSecnd{  0.9294} \\ 
			\midrule
			%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
			
			\multirow{6}{*}{Case 7} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-3}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    4.61 &   -0.00 &    4.46 &    9.06 &   -6.68 &   -7.88 & \Valbest{  16.19} &    8.43 & \ValSecnd{  10.55} &    7.97 &    8.32 \\ 
			& RMSE &   0.0253 &   2.0093 &   0.0270 &   0.0171 &   0.0582 &   0.0561 & \Valbest{  0.0082} &   0.0184 & \ValSecnd{  0.0136} &   0.0177 &   0.0171 \\ 
			& Ps   &   0.67 &   0.09 &   0.61 &   0.88 &   0.00 &   0.00 & \Valbest{  0.99} &   0.85 & \ValSecnd{  0.96} &   0.91 &   0.92 \\ 
			& MPSNR &   31.60 &  -44.48 &   30.64 &   31.88 &   12.53 &   12.99 & \Valbest{  34.67} &   28.67 &   32.38 &   32.70 & \ValSecnd{  33.19} \\ 
			& MSSIM &   0.8806 &   0.4875 &   0.8485 &   0.8723 &   0.1260 &   0.3170 & \Valbest{  0.9295} &   0.8358 & \ValSecnd{  0.9250} &   0.8999 &   0.9117 \\ 
			\midrule 
			
			\multirow{6}{*}{Case 8} 
			& Setup & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{3} = 10^{1}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{TV} = 10^{-2}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{g} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{l} = 10^{-2}$ \hspace{-4mm}\end{tabular} &  --  &  --  & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\tau = 10^{0}$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  &    2.55 &   -0.00 &    1.55 &    5.20 &   -6.84 &   -8.13 & \Valbest{  13.14} &    4.47 & \ValSecnd{   8.92} &    6.64 &    7.32 \\ 
			& RMSE &   0.0302 &   2.1167 &   0.0380 &   0.0246 &   0.0578 &   0.0559 & \Valbest{  0.0113} &   0.0274 & \ValSecnd{  0.0160} &   0.0199 &   0.0186 \\ 
			& Ps   &   0.58 &   0.06 &   0.38 &   0.71 &   0.00 &   0.00 & \Valbest{  0.97} &   0.65 & \ValSecnd{  0.92} &   0.85 &   0.88 \\ 
			& MPSNR &   28.26 &  -44.97 &   27.45 &   28.50 &   13.55 &   13.19 &   31.20 &   25.12 & \Valbest{  31.82} &   31.34 & \ValSecnd{  31.62} \\ 
			& MSSIM &   0.8057 &   0.3782 &   0.7635 &   0.7943 &   0.1835 &   0.3380 &   0.8736 &   0.7267 & \Valbest{  0.9192} &   0.8727 & \ValSecnd{  0.8796} \\
			
			\bottomrule
		\end{tabular}
	}
\end{table*}






==> tab_tex/tab_results_ablation.tex <==
%\begin{table}[t]
%	\caption{RSE, RMSE, Ps, MPSNR, and MSSIM of Ablation Experiments.}
%	\vspace{-1mm}
%	\label{tab:results_ablation}
%	\centering
%	%	\scriptsize
%	\scalebox{0.775}{
%		\begin{tabular}{ccccccc} \toprule
%			\multirow{3}{*}{ Image } & \multirow{3}{6em}{\centering Evaluation \\ Target}  & \multirow{3}{*}{Measures}& \multicolumn{4}{c}{Methods}\\ 
%			\cmidrule(lr){4-7}
%			& & & \Ours & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
%			& & & -- & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
%			
%			\midrule
%			
%			\multirow{5}{*}{\textit{Synth 1}} 
%			& \multirow{3}{*}{Abundance}
%			& SRE  & 19.88 & \Valbest{20.13} & \ValSecnd{19.72} & 19.63 \\
%			& & RMSE & 0.0390 & \Valbest{0.0377} & \ValSecnd{0.0393} & 0.0396 \\
%			& & Ps   & 0.76 & \ValSecnd{0.79} & \Valbest{0.80} & \ValSecnd{0.82} \\
%			\cmidrule(lr){2-7}
%			& Reconstructed
%			& MPSNR & 36.21 & \ValSecnd{38.85} & 36.95 & \Valbest{39.44} \\
%			& HS image
%			& MSSIM & 0.9420 & \ValSecnd{0.9702} & 0.9527 & \Valbest{0.9753} \\
%			\cmidrule(lr){1-7}
%			
%			\multirow{5}{*}{\textit{Synth 2}} 
%			& \multirow{3}{*}{Abundance}
%			& SRE  & 6.83 & \ValSecnd{7.94} & \Valbest{7.97} & 7.92 \\
%			& & RMSE & 0.1464 & \ValSecnd{0.1464} & \Valbest{0.1459} & 0.1468 \\
%			& & Ps   & 0.67 & \ValSecnd{0.68} & \Valbest{0.69} & \ValSecnd{0.68} \\
%			\cmidrule(lr){2-7}
%			& Reconstructed
%			& MPSNR & 34.92 & \ValSecnd{35.97} & 35.09 & \Valbest{36.11} \\
%			& HS image
%			& MSSIM & 0.9626 & \ValSecnd{0.9735} & 0.9641 & \Valbest{0.9737} \\
%			\cmidrule(lr){1-7}
%			
%			\multirow{5}{3em}{\centering \textit{Jasper \\ Ridge}} 
%			& \multirow{3}{*}{Abundance}
%			& SRE  & 13.42 & \Valbest{14.06} & 13.56 & \ValSecnd{13.59} \\
%			& & RMSE & \Valbest{0.0843} & \ValSecnd{0.0852} & 0.0902 & {0.0899} \\
%			& & Ps   & \Valbest{0.39} & \Valbest{0.39} & \Valbest{0.39} & \Valbest{0.39} \\
%			\cmidrule(lr){2-7}
%			& Reconstructed
%			& MPSNR & 30.86 & \Valbest{31.45} & 30.79 & \ValSecnd{31.24} \\
%			& HS image
%			& MSSIM & 0.9450 & \Valbest{0.9566} & 0.9459 & \ValSecnd{0.9550} \\
%			\cmidrule(lr){1-7}
%			
%			\multirow{5}{*}{\centering \textit{Samson}} 
%			& \multirow{3}{*}{Abundance}
%			& SRE  & 9.13 & \ValSecnd{9.76} & 9.31 & \Valbest{10.29} \\
%			& & RMSE & 0.1280 & \ValSecnd{0.1212} & 0.1257 & \Valbest{0.1156} \\
%			& & Ps   & 0.67 & \ValSecnd{0.69} & 0.68 & \Valbest{0.70} \\
%			\cmidrule(lr){2-7}
%			& Reconstructed
%			& MPSNR & 29.49 & \ValSecnd{30.63} & 29.86 & \Valbest{30.83} \\
%			& HS image
%			& MSSIM & 0.9253 & \ValSecnd{0.9471} & 0.9330 & \Valbest{0.9500} \\
%			\bottomrule
%		\end{tabular}
%	}
%\end{table}

\begin{table*}[t]
	\caption{RSE, RMSE, Ps, MPSNR, and MSSIM of Ablation Experiments.}
	\vspace{-1mm}
	\label{tab:results_ablation}
	\centering
	%	\scriptsize
	\scalebox{0.775}{
		\begin{tabular}{cccccccccccccc} \toprule
			\multirow{3}{*}{ Image }  & \multirow{3}{*}{Measures} & \multicolumn{4}{c}{Methods} & \multicolumn{4}{c}{Methods} & \multicolumn{4}{c}{Methods} \\ 
			\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			& & \Ours & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} & \Ours & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} & \Ours & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
			& & -- & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} & -- & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} & -- & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
			
			\midrule
			
			\multirow{5}{*}{\textit{Synth 1}} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  & 19.88 & \Valbest{20.13} & \ValSecnd{19.72} & 19.63 \\
			& RMSE & 0.0390 & \Valbest{0.0377} & \ValSecnd{0.0393} & 0.0396 \\
			& Ps   & 0.76 & \ValSecnd{0.79} & \Valbest{0.80} & \ValSecnd{0.82} \\
			& MPSNR & 36.21 & \ValSecnd{38.85} & 36.95 & \Valbest{39.44} \\
			& MSSIM & 0.9420 & \ValSecnd{0.9702} & 0.9527 & \Valbest{0.9753} \\
			\cmidrule(lr){1-7}
			
			\multirow{5}{*}{\textit{Synth 2}} 
			& SRE  & 6.83 & \ValSecnd{7.94} & \Valbest{7.97} & 7.92 \\
			& RMSE & 0.1464 & \ValSecnd{0.1464} & \Valbest{0.1459} & 0.1468 \\
			& Ps   & 0.67 & \ValSecnd{0.68} & \Valbest{0.69} & \ValSecnd{0.68} \\
			& MPSNR & 34.92 & \ValSecnd{35.97} & 35.09 & \Valbest{36.11} \\
			& MSSIM & 0.9626 & \ValSecnd{0.9735} & 0.9641 & \Valbest{0.9737} \\
			\cmidrule(lr){1-7}
			
			\multirow{5}{3em}{\centering \textit{Jasper \\ Ridge}} 
			& SRE  & 13.42 & \Valbest{14.06} & 13.56 & \ValSecnd{13.59} \\
			& RMSE & \Valbest{0.0843} & \ValSecnd{0.0852} & 0.0902 & {0.0899} \\
			& Ps   & \Valbest{0.39} & \Valbest{0.39} & \Valbest{0.39} & \Valbest{0.39} \\
			& MPSNR & 30.86 & \Valbest{31.45} & 30.79 & \ValSecnd{31.24} \\
			& MSSIM & 0.9450 & \Valbest{0.9566} & 0.9459 & \ValSecnd{0.9550} \\
			\cmidrule(lr){1-7}
			
			\multirow{5}{*}{\centering \textit{Samson}} 
			& SRE  & 9.13 & \ValSecnd{9.76} & 9.31 & \Valbest{10.29} \\
			& RMSE & 0.1280 & \ValSecnd{0.1212} & 0.1257 & \Valbest{0.1156} \\
			& Ps   & 0.67 & \ValSecnd{0.69} & 0.68 & \Valbest{0.70} \\
			& MPSNR & 29.49 & \ValSecnd{30.63} & 29.86 & \Valbest{30.83} \\
			& MSSIM & 0.9253 & \ValSecnd{0.9471} & 0.9330 & \Valbest{0.9500} \\
			\bottomrule
		\end{tabular}
	}
\end{table*}



==> tab_tex/tab_results_ablation_colored.tex <==
\begin{table}[t]
	\color{blue}
	\caption{RSE, RMSE, Ps, MPSNR, and MSSIM Results of Ablation Experiments.}
	\vspace{-1mm}
	\label{tab:results_ablation}
	\centering
	%	\scriptsize
	\scalebox{0.8}{
		\begin{tabular}{ccccccc} \toprule
			\multirow{3}{*}{ Image } & \multirow{3}{6em}{\centering Evaluation \\ Target}  & \multirow{3}{*}{Measures}& \multicolumn{4}{c}{Methods}\\ 
			\cmidrule(lr){4-7}
			& & & \Ours & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
			& & & -- & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
			
			\midrule
			
			\multirow{5}{6em}{\centering Synthetic \\ HS Image 1} 
			& \multirow{3}{*}{Abundance}
			& SRE  & 19.88 & \Valbest{20.13} & \ValSecnd{19.72} & 19.63 \\
			& & RMSE & 0.0390 & \Valbest{0.0377} & \ValSecnd{0.0393} & 0.0396 \\
			& & Ps   & 0.76 & \ValSecnd{0.79} & \Valbest{0.80} & \ValSecnd{0.82} \\
			\cmidrule(lr){2-7}
			& Reconstructed
			& MPSNR & 36.21 & \ValSecnd{38.85} & 36.95 & \Valbest{39.44} \\
			& HS image
			& MSSIM & 0.9420 & \ValSecnd{0.9702} & 0.9527 & \Valbest{0.9753} \\
			\cmidrule(lr){1-7}
			
			\multirow{5}{6em}{\centering Synthetic \\ HS Image 2} 
			& \multirow{3}{*}{Abundance}
			& SRE  & 6.83 & \ValSecnd{7.94} & \Valbest{7.97} & 7.92 \\
			& & RMSE & 0.1464 & \ValSecnd{0.1464} & \Valbest{0.1459} & 0.1468 \\
			& & Ps   & 0.67 & \ValSecnd{0.68} & \Valbest{0.69} & \ValSecnd{0.68} \\
			\cmidrule(lr){2-7}
			& Reconstructed
			& MPSNR & 34.92 & \ValSecnd{35.97} & 35.09 & \Valbest{36.11} \\
			& HS image
			& MSSIM & 0.9626 & \ValSecnd{0.9735} & 0.9641 & \Valbest{0.9737} \\
			\cmidrule(lr){1-7}
			
			\multirow{5}{6em}{\centering \textit{Jasper \\ Ridge}} 
			& \multirow{3}{*}{Abundance}
			& SRE  & 13.42 & \Valbest{14.06} & 13.56 & \ValSecnd{13.59} \\
			& & RMSE & \Valbest{0.0843} & \ValSecnd{0.0852} & 0.0902 & {0.0899} \\
			& & Ps   & \Valbest{0.39} & \Valbest{0.39} & \Valbest{0.39} & \Valbest{0.39} \\
			\cmidrule(lr){2-7}
			& Reconstructed
			& MPSNR & 30.86 & \Valbest{31.45} & 30.79 & \ValSecnd{31.24} \\
			& HS image
			& MSSIM & 0.9450 & \Valbest{0.9566} & 0.9459 & \ValSecnd{0.9550} \\
			\cmidrule(lr){1-7}
			
			\multirow{5}{6em}{\centering \textit{Samson}} 
			& \multirow{3}{*}{Abundance}
			& SRE  & 9.13 & \ValSecnd{9.76} & 9.31 & \Valbest{10.29} \\
			& & RMSE & 0.1280 & \ValSecnd{0.1212} & 0.1257 & \Valbest{0.1156} \\
			& & Ps   & 0.67 & \ValSecnd{0.69} & 0.68 & \Valbest{0.70} \\
			\cmidrule(lr){2-7}
			& Reconstructed
			& MPSNR & 29.49 & \ValSecnd{30.63} & 29.86 & \Valbest{30.83} \\
			& HS image
			& MSSIM & 0.9253 & \ValSecnd{0.9471} & 0.9330 & \Valbest{0.9500} \\
			\bottomrule
		\end{tabular}
	}
	\color{black}
\end{table}



==> tab_tex/tab_results_ablation_real_colored.tex <==
%\begin{table}[t]
%	\caption{RSE, RMSE, Ps, MPSNR, and MSSIM of Ablation Experiments.}
%	\vspace{-1mm}
%	\label{tab:results_ablation}
%	\centering
%	%	\scriptsize
%	\scalebox{0.775}{
	%		\begin{tabular}{ccccccc} \toprule
		%			\multirow{3}{*}{ Image } & \multirow{3}{6em}{\centering Evaluation \\ Target}  & \multirow{3}{*}{Measures}& \multicolumn{4}{c}{Methods}\\ 
		%			\cmidrule(lr){4-7}
		%			& & & \Ours & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
		%			& & & -- & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
		%			
		%			\midrule
		%			
		%			\multirow{5}{*}{\textit{Synth 1}} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 19.88 & \Valbest{20.13} & \ValSecnd{19.72} & 19.63 \\
		%			& & RMSE & 0.0390 & \Valbest{0.0377} & \ValSecnd{0.0393} & 0.0396 \\
		%			& & Ps   & 0.76 & \ValSecnd{0.79} & \Valbest{0.80} & \ValSecnd{0.82} \\
		%			\cmidrule(lr){2-7}
		%			& Reconstructed
		%			& MPSNR & 36.21 & \ValSecnd{38.85} & 36.95 & \Valbest{39.44} \\
		%			& HS image
		%			& MSSIM & 0.9420 & \ValSecnd{0.9702} & 0.9527 & \Valbest{0.9753} \\
		%			\cmidrule(lr){1-10}
		%			
		%			\multirow{5}{*}{\textit{Synth 2}} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 6.83 & \ValSecnd{7.94} & \Valbest{7.97} & 7.92 \\
		%			& & RMSE & 0.1464 & \ValSecnd{0.1464} & \Valbest{0.1459} & 0.1468 \\
		%			& & Ps   & 0.67 & \ValSecnd{0.68} & \Valbest{0.69} & \ValSecnd{0.68} \\
		%			\cmidrule(lr){2-7}
		%			& Reconstructed
		%			& MPSNR & 34.92 & \ValSecnd{35.97} & 35.09 & \Valbest{36.11} \\
		%			& HS image
		%			& MSSIM & 0.9626 & \ValSecnd{0.9735} & 0.9641 & \Valbest{0.9737} \\
		%			\cmidrule(lr){1-10}
		%			
		%			\multirow{5}{3em}{\centering \textit{Jasper \\ Ridge}} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 13.42 & \Valbest{14.06} & 13.56 & \ValSecnd{13.59} \\
		%			& & RMSE & \Valbest{0.0843} & \ValSecnd{0.0852} & 0.0902 & {0.0899} \\
		%			& & Ps   & \Valbest{0.39} & \Valbest{0.39} & \Valbest{0.39} & \Valbest{0.39} \\
		%			\cmidrule(lr){2-7}
		%			& Reconstructed
		%			& MPSNR & 30.86 & \Valbest{31.45} & 30.79 & \ValSecnd{31.24} \\
		%			& HS image
		%			& MSSIM & 0.9450 & \Valbest{0.9566} & 0.9459 & \ValSecnd{0.9550} \\
		%			\cmidrule(lr){1-10}
		%			
		%			\multirow{5}{*}{\centering \textit{Samson}} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 9.13 & \ValSecnd{9.76} & 9.31 & \Valbest{10.29} \\
		%			& & RMSE & 0.1280 & \ValSecnd{0.1212} & 0.1257 & \Valbest{0.1156} \\
		%			& & Ps   & 0.67 & \ValSecnd{0.69} & 0.68 & \Valbest{0.70} \\
		%			\cmidrule(lr){2-7}
		%			& Reconstructed
		%			& MPSNR & 29.49 & \ValSecnd{30.63} & 29.86 & \Valbest{30.83} \\
		%			& HS image
		%			& MSSIM & 0.9253 & \ValSecnd{0.9471} & 0.9330 & \Valbest{0.9500} \\
		%			\bottomrule
		%		\end{tabular}
	%	}
%\end{table}

\begin{table*}[t]
	\color{blue}
	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM of the Ablation Experiments Using Real Datasets.}
	\vspace{-1mm}
	\label{tab:results_ablation_real}
	\centering
	%	\scriptsize
	\scalebox{0.775}{
		\begin{tabular}{cccccccccccccc} \toprule
			\multirow{3}{*}{ Image }  & \multirow{3}{*}{Metrics} & \multicolumn{4}{c}{\textit{Jasper Ridge}} & \multicolumn{4}{c}{Samson} & \multicolumn{4}{c}{Urban} \\ 
			\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			& & \Ours & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} & \Ours & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} & \Ours & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
			& & -- & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} & -- & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} & -- & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
			
			\midrule
			
			\multirow{6}{*}{Case 1} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			& \ValSecnd{  19.08} &   19.07 & \Valbest{  19.33} &   19.06 
			&   15.90 & \Valbest{  19.51} &   16.48 & \ValSecnd{  18.03} 
			& \ValSecnd{  15.00} & \Valbest{  15.92} &   14.49 &   14.74 \\ 
			& RMSE 
			& \ValSecnd{  0.0294} & \ValSecnd{  0.0294} & \Valbest{  0.0286} &   0.0295 
			&   0.0368 & \Valbest{  0.0254} &   0.0345 & \ValSecnd{  0.0296} 
			& \ValSecnd{  0.0086} & \Valbest{  0.0078} &   0.0090 &   0.0088 \\ 
			& Ps   
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} \\ 
			& MPSNR 
			&   45.44 & \ValSecnd{  45.45} & \Valbest{  45.47} & \ValSecnd{  45.45} 
			&   45.27 &   43.75 & \ValSecnd{  45.52} & \Valbest{  46.74} 
			& \ValSecnd{  41.84} &   37.93 &   41.74 & \Valbest{  41.91} \\ 
			& MSSIM 
			& \Valbest{  0.9882} & \Valbest{  0.9882} & \ValSecnd{  0.9881} & \Valbest{  0.9882} 
			&   0.9842 &   0.9836 & \ValSecnd{  0.9855} & \Valbest{  0.9907} 
			& \ValSecnd{  0.9857} &   0.9741 &   0.9854 & \Valbest{  0.9863} \\ 
			%			\midrule 
			\cmidrule(lr){1-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			
			\multirow{6}{*}{Case 2} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			&   15.38 & \ValSecnd{  15.49} & \Valbest{  15.53} &   15.37 
			&   11.02 & \Valbest{  14.51} &   11.09 & \ValSecnd{  12.86} 
			&   11.36 & \Valbest{  12.62} &   10.90 & \ValSecnd{  11.37} \\ 
			& RMSE 
			&   0.0441 & \ValSecnd{  0.0436} & \Valbest{  0.0432} &   0.0441 
			&   0.0597 & \Valbest{  0.0435} &   0.0590 & \ValSecnd{  0.0504} 
			& \ValSecnd{  0.0126} & \Valbest{  0.0110} &   0.0131 & \ValSecnd{  0.0126} \\ 
			& Ps   
			& \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} 
			& \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} 
			& \Valbest{  0.98} & \Valbest{  0.98} & \Valbest{  0.98} & \Valbest{  0.98} \\ 
			& MPSNR 
			&   40.34 & \Valbest{  40.97} &   40.31 & \ValSecnd{  40.36} 
			&   40.10 & \Valbest{  40.84} & \ValSecnd{  40.45} &   40.44 
			& \ValSecnd{  35.89} &   35.25 &   35.77 & \Valbest{  36.05} \\ 
			& MSSIM 
			&   0.9639 & \Valbest{  0.9732} &   0.9634 & \ValSecnd{  0.9641} 
			&   0.9513 & \ValSecnd{  0.9719} &   0.9561 & \Valbest{  0.9725} 
			&   0.9459 & \Valbest{  0.9571} &   0.9448 & \ValSecnd{  0.9483} \\ 
			%			\midrule 
			\cmidrule(lr){1-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			
			\multirow{6}{*}{Case 3} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			& \ValSecnd{  18.76} & \ValSecnd{  18.76} & \Valbest{  18.98} &   18.75 
			&   15.24 & \Valbest{  18.16} &   15.61 & \ValSecnd{  16.74} 
			& \ValSecnd{  14.33} & \Valbest{  15.29} &   13.79 &   14.11 \\ 
			& RMSE 
			& \ValSecnd{  0.0303} &   0.0304 & \Valbest{  0.0296} &   0.0304 
			&   0.0393 & \Valbest{  0.0294} &   0.0378 & \ValSecnd{  0.0341} 
			& \ValSecnd{  0.0092} & \Valbest{  0.0083} &   0.0097 &   0.0094 \\ 
			& Ps   
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} \\ 
			& MPSNR 
			& \ValSecnd{  44.46} & \Valbest{  44.47} & \Valbest{  44.47} & \Valbest{  44.47} 
			&   44.12 &   43.09 & \ValSecnd{  44.34} & \Valbest{  45.45} 
			& \ValSecnd{  40.89} &   37.38 &   40.78 & \Valbest{  40.98} \\ 
			& MSSIM 
			& \ValSecnd{  0.9849} & \ValSecnd{  0.9849} &   0.9848 & \Valbest{  0.9850} 
			&   0.9791 & \ValSecnd{  0.9812} &   0.9807 & \Valbest{  0.9868} 
			& \ValSecnd{  0.9823} &   0.9712 &   0.9819 & \Valbest{  0.9831} \\ 
			%			\midrule 
			\cmidrule(lr){1-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			
			\multirow{6}{*}{Case 4} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			&   18.26 & \Valbest{  18.31} & \ValSecnd{  18.29} &   18.26 
			&   14.09 & \Valbest{  16.09} &   14.57 & \ValSecnd{  15.24} 
			& \ValSecnd{  14.22} & \Valbest{  14.95} &   13.76 &   14.05 \\ 
			& RMSE 
			& \ValSecnd{  0.0321} & \Valbest{  0.0319} & \ValSecnd{  0.0321} & \ValSecnd{  0.0321} 
			&   0.0439 & \Valbest{  0.0364} &   0.0417 & \ValSecnd{  0.0390} 
			& \ValSecnd{  0.0093} & \Valbest{  0.0086} &   0.0097 &   0.0095 \\ 
			& Ps   
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} \\ 
			& MPSNR 
			&   43.37 & \Valbest{  43.89} & \ValSecnd{  43.39} & \ValSecnd{  43.39} 
			&   43.18 &   42.80 & \ValSecnd{  43.41} & \Valbest{  44.25} 
			& \ValSecnd{  40.00} &   37.34 &   39.87 & \Valbest{  40.12} \\ 
			& MSSIM 
			&   0.9801 & \Valbest{  0.9836} & \ValSecnd{  0.9803} &   0.9802 
			&   0.9742 & \ValSecnd{  0.9805} &   0.9761 & \Valbest{  0.9815} 
			& \ValSecnd{  0.9782} &   0.9713 &   0.9776 & \Valbest{  0.9792} \\ 
			%			\midrule 
			\cmidrule(lr){1-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			
			\multirow{6}{*}{Case 5} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			& \ValSecnd{  16.19} & \Valbest{  16.36} &   16.16 & \ValSecnd{  16.19} 
			&   10.75 & \Valbest{  12.91} &   10.04 & \ValSecnd{  12.12} 
			& \ValSecnd{   9.61} & \Valbest{  10.38} &    9.59 &    9.59 \\ 
			& RMSE 
			&   0.0401 & \Valbest{  0.0394} &   0.0401 & \ValSecnd{  0.0400} 
			&   0.0607 & \Valbest{  0.0489} &   0.0648 & \ValSecnd{  0.0532} 
			& \ValSecnd{  0.0148} & \Valbest{  0.0138} &   0.0149 & \ValSecnd{  0.0148} \\ 
			& Ps   
			& \Valbest{  1.00} & \ValSecnd{  0.99} & \ValSecnd{  0.99} & \Valbest{  1.00} 
			& \ValSecnd{  0.99} & \Valbest{  1.00} & \ValSecnd{  0.99} & \Valbest{  1.00} 
			& \ValSecnd{  0.94} & \Valbest{  0.96} & \ValSecnd{  0.94} & \ValSecnd{  0.94} \\ 
			& MPSNR 
			&   41.47 & \Valbest{  42.26} & \ValSecnd{  41.63} &   41.49 
			&   41.05 & \Valbest{  42.74} &   40.95 & \ValSecnd{  42.48} 
			& \ValSecnd{  37.42} &   30.36 & \ValSecnd{  37.42} & \Valbest{  37.43} \\ 
			& MSSIM 
			&   0.9734 & \Valbest{  0.9791} & \ValSecnd{  0.9744} &   0.9735 
			&   0.9631 & \Valbest{  0.9811} &   0.9625 & \ValSecnd{  0.9759} 
			& \ValSecnd{  0.9677} &   0.8906 & \ValSecnd{  0.9677} & \Valbest{  0.9679} \\ 
			%			\midrule 
			\cmidrule(lr){1-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			
			\multirow{6}{*}{Case 6} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			&   14.17 & \Valbest{  14.39} &   14.03 & \ValSecnd{  14.19} 
			&    9.92 & \Valbest{  12.49} &    9.33 & \ValSecnd{  11.97} 
			&    8.13 & \Valbest{  10.02} &    8.59 & \ValSecnd{   8.69} \\ 
			& RMSE 
			& \ValSecnd{  0.0500} & \Valbest{  0.0489} &   0.0507 & \ValSecnd{  0.0500} 
			&   0.0655 & \Valbest{  0.0525} &   0.0689 & \ValSecnd{  0.0543} 
			&   0.0175 & \Valbest{  0.0144} &   0.0166 & \ValSecnd{  0.0165} \\ 
			& Ps   
			& \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} 
			& \ValSecnd{  0.99} & \ValSecnd{  0.99} &   0.98 & \Valbest{  1.00} 
			&   0.90 & \Valbest{  0.95} & \ValSecnd{  0.93} & \ValSecnd{  0.93} \\ 
			& MPSNR 
			&   37.86 & \Valbest{  38.82} &   37.78 & \ValSecnd{  38.04} 
			&   37.76 & \ValSecnd{  38.41} &   37.76 & \Valbest{  39.70} 
			&   33.25 & \Valbest{  34.34} &   33.87 & \ValSecnd{  34.18} \\ 
			& MSSIM 
			&   0.9407 & \Valbest{  0.9563} &   0.9396 & \ValSecnd{  0.9435} 
			&   0.9219 & \ValSecnd{  0.9559} &   0.9222 & \Valbest{  0.9573} 
			&   0.9109 & \Valbest{  0.9496} &   0.9227 & \ValSecnd{  0.9294} \\ 
			%			\midrule 
			\cmidrule(lr){1-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			
			\multirow{6}{*}{Case 7} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			&   13.34 & \Valbest{  13.67} &   13.27 & \ValSecnd{  13.35} 
			&    8.26 & \Valbest{  13.61} &    8.38 & \ValSecnd{  11.28} 
			&    8.12 & \Valbest{  10.55} &    7.97 & \ValSecnd{   8.32} \\ 
			& RMSE 
			&   0.0548 & \Valbest{  0.0531} &   0.0551 & \ValSecnd{  0.0547} 
			&   0.0767 & \Valbest{  0.0466} &   0.0759 & \ValSecnd{  0.0588} 
			&   0.0173 & \Valbest{  0.0136} &   0.0177 & \ValSecnd{  0.0171} \\ 
			& Ps   
			& \Valbest{  0.98} & \Valbest{  0.98} & \Valbest{  0.98} & \Valbest{  0.98} 
			&   0.95 & \Valbest{  1.00} &   0.98 & \ValSecnd{  0.99} 
			&   0.91 & \Valbest{  0.96} &   0.91 & \ValSecnd{  0.92} \\ 
			& MPSNR 
			&   37.02 & \Valbest{  38.22} &   36.94 & \ValSecnd{  37.25} 
			&   36.88 & \Valbest{  39.74} &   37.62 & \ValSecnd{  38.83} 
			& \Valbest{  33.51} &   32.38 &   32.70 & \ValSecnd{  33.19} \\ 
			& MSSIM 
			&   0.9265 & \Valbest{  0.9502} &   0.9250 & \ValSecnd{  0.9310} 
			&   0.9036 & \Valbest{  0.9651} &   0.9317 & \ValSecnd{  0.9612} 
			& \ValSecnd{  0.9141} & \Valbest{  0.9250} &   0.8999 &   0.9117 \\ 
			%			\midrule 
			\cmidrule(lr){1-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			
			\multirow{6}{*}{Case 8} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			&   12.20 & \Valbest{  12.46} &   12.12 & \ValSecnd{  12.21} 
			&    7.43 & \Valbest{  10.39} &    6.26 & \ValSecnd{   9.40} 
			&    7.25 & \Valbest{   8.92} &    6.64 & \ValSecnd{   7.32} \\ 
			& RMSE 
			&   0.0621 & \Valbest{  0.0604} &   0.0623 & \ValSecnd{  0.0619} 
			&   0.0827 & \Valbest{  0.0630} &   0.0922 & \ValSecnd{  0.0714} 
			&   0.0188 & \Valbest{  0.0160} &   0.0199 & \ValSecnd{  0.0186} \\ 
			& Ps   
			& \Valbest{  0.97} & \Valbest{  0.97} & \Valbest{  0.97} & \Valbest{  0.97} 
			&   0.90 & \Valbest{  0.99} &   0.84 & \ValSecnd{  0.96} 
			& \ValSecnd{  0.88} & \Valbest{  0.92} &   0.85 & \ValSecnd{  0.88} \\ 
			& MPSNR 
			&   35.74 & \Valbest{  36.93} &   35.67 & \ValSecnd{  35.97} 
			&   35.82 & \ValSecnd{  37.22} &   35.18 & \Valbest{  37.76} 
			&   31.41 & \Valbest{  31.82} &   31.34 & \ValSecnd{  31.62} \\ 
			& MSSIM 
			&   0.9067 & \Valbest{  0.9371} &   0.9055 & \ValSecnd{  0.9124} 
			&   0.8875 & \Valbest{  0.9447} &   0.8707 & \ValSecnd{  0.9405} 
			&   0.8736 & \Valbest{  0.9192} &   0.8727 & \ValSecnd{  0.8796} \\  
			\bottomrule
		\end{tabular}
	}
\end{table*}



==> tab_tex/tab_results_ablation_synth_colored.tex <==
%\begin{table}[t]
%	\caption{RSE, RMSE, Ps, MPSNR, and MSSIM of Ablation Experiments.}
%	\vspace{-1mm}
%	\label{tab:results_ablation}
%	\centering
%	%	\scriptsize
%	\scalebox{0.775}{
	%		\begin{tabular}{ccccccc} \toprule
		%			\multirow{3}{*}{ Image } & \multirow{3}{6em}{\centering Evaluation \\ Target}  & \multirow{3}{*}{Measures}& \multicolumn{4}{c}{Methods}\\ 
		%			\cmidrule(lr){4-7}
		%			& & & \Ours & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
		%			& & & -- & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
		%			
		%			\midrule
		%			
		%			\multirow{5}{*}{\textit{Synth 1}} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 19.88 & \Valbest{20.13} & \ValSecnd{19.72} & 19.63 \\
		%			& & RMSE & 0.0390 & \Valbest{0.0377} & \ValSecnd{0.0393} & 0.0396 \\
		%			& & Ps   & 0.76 & \ValSecnd{0.79} & \Valbest{0.80} & \ValSecnd{0.82} \\
		%			\cmidrule(lr){2-7}
		%			& Reconstructed
		%			& MPSNR & 36.21 & \ValSecnd{38.85} & 36.95 & \Valbest{39.44} \\
		%			& HS image
		%			& MSSIM & 0.9420 & \ValSecnd{0.9702} & 0.9527 & \Valbest{0.9753} \\
		%			\cmidrule(lr){1-7}
		%			
		%			\multirow{5}{*}{\textit{Synth 2}} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 6.83 & \ValSecnd{7.94} & \Valbest{7.97} & 7.92 \\
		%			& & RMSE & 0.1464 & \ValSecnd{0.1464} & \Valbest{0.1459} & 0.1468 \\
		%			& & Ps   & 0.67 & \ValSecnd{0.68} & \Valbest{0.69} & \ValSecnd{0.68} \\
		%			\cmidrule(lr){2-7}
		%			& Reconstructed
		%			& MPSNR & 34.92 & \ValSecnd{35.97} & 35.09 & \Valbest{36.11} \\
		%			& HS image
		%			& MSSIM & 0.9626 & \ValSecnd{0.9735} & 0.9641 & \Valbest{0.9737} \\
		%			\cmidrule(lr){1-7}
		%			
		%			\multirow{5}{3em}{\centering \textit{Jasper \\ Ridge}} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 13.42 & \Valbest{14.06} & 13.56 & \ValSecnd{13.59} \\
		%			& & RMSE & \Valbest{0.0843} & \ValSecnd{0.0852} & 0.0902 & {0.0899} \\
		%			& & Ps   & \Valbest{0.39} & \Valbest{0.39} & \Valbest{0.39} & \Valbest{0.39} \\
		%			\cmidrule(lr){2-7}
		%			& Reconstructed
		%			& MPSNR & 30.86 & \Valbest{31.45} & 30.79 & \ValSecnd{31.24} \\
		%			& HS image
		%			& MSSIM & 0.9450 & \Valbest{0.9566} & 0.9459 & \ValSecnd{0.9550} \\
		%			\cmidrule(lr){1-7}
		%			
		%			\multirow{5}{*}{\centering \textit{Samson}} 
		%			& \multirow{3}{*}{Abundance}
		%			& SRE  & 9.13 & \ValSecnd{9.76} & 9.31 & \Valbest{10.29} \\
		%			& & RMSE & 0.1280 & \ValSecnd{0.1212} & 0.1257 & \Valbest{0.1156} \\
		%			& & Ps   & 0.67 & \ValSecnd{0.69} & 0.68 & \Valbest{0.70} \\
		%			\cmidrule(lr){2-7}
		%			& Reconstructed
		%			& MPSNR & 29.49 & \ValSecnd{30.63} & 29.86 & \Valbest{30.83} \\
		%			& HS image
		%			& MSSIM & 0.9253 & \ValSecnd{0.9471} & 0.9330 & \Valbest{0.9500} \\
		%			\bottomrule
		%		\end{tabular}
	%	}
%\end{table}

\begin{table*}[t]
	\color{blue}
	\caption{SRE, RMSE, Ps, MPSNR, and MSSIM of the Ablation Experiments Using Synthetic Datasets.}
	\vspace{-1mm}
	\label{tab:results_ablation_synth}
	\centering
	%	\scriptsize
	\scalebox{0.775}{
		\begin{tabular}{cccccccccccccc} \toprule
			\multirow{3}{*}{ Image }  & \multirow{3}{*}{Metrics} & \multicolumn{4}{c}{\textit{Synth 1}} & \multicolumn{4}{c}{\textit{Synth 2}} & \multicolumn{4}{c}{\textit{Synth 3}} \\ 
			\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			& & \Ours & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} & \Ours & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} & \Ours & \textbf{\Ours} & \textbf{\Ours} & \textbf{\Ours} \\ 
			& & -- & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} & -- & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} & -- & \textbf{(HTV)} & \textbf{(SSTV)} & \textbf{(HSSTV)} \\ 
			
			\midrule
			
			\multirow{6}{*}{Case 1} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			& \ValSecnd{  23.54} & \Valbest{  24.31} &   21.84 &   23.52 
			&   20.85 & \Valbest{  21.11} &   20.78 & \ValSecnd{  20.99} 
			&   27.08 & \Valbest{  30.26} &   26.38 & \ValSecnd{  27.58} \\ 
			& RMSE 
			& \ValSecnd{  0.0166} & \Valbest{  0.0153} &   0.0200 &   0.0167 
			&   0.0204 & \Valbest{  0.0198} &   0.0206 & \ValSecnd{  0.0201} 
			&   0.0024 & \Valbest{  0.0017} &   0.0026 & \ValSecnd{  0.0023} \\ 
			& Ps   
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR 
			&   47.69 & \Valbest{  54.23} & \ValSecnd{  49.34} &   47.74 
			&   42.38 & \Valbest{  42.84} &   42.39 & \ValSecnd{  42.55} 
			&   46.04 & \Valbest{  56.00} &   46.05 & \ValSecnd{  46.49} \\ 
			& MSSIM 
			&   0.9885 & \Valbest{  0.9988} & \ValSecnd{  0.9937} &   0.9886 
			&   0.9891 & \Valbest{  0.9911} &   0.9891 & \ValSecnd{  0.9897} 
			&   0.9810 & \Valbest{  0.9997} &   0.9822 & \ValSecnd{  0.9834} \\ 
			\cmidrule(lr){1-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			
			\multirow{6}{*}{Case 2} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			&   20.55 & \Valbest{  21.64} &   20.19 & \ValSecnd{  20.84} 
			&   17.15 & \Valbest{  17.50} &   17.23 & \ValSecnd{  17.38} 
			&   21.95 & \Valbest{  28.67} &   22.34 & \ValSecnd{  22.72} \\ 
			& RMSE 
			&   0.0234 & \Valbest{  0.0206} &   0.0240 & \ValSecnd{  0.0226} 
			&   0.0310 & \Valbest{  0.0297} &   0.0308 & \ValSecnd{  0.0302} 
			&   0.0043 & \Valbest{  0.0020} &   0.0041 & \ValSecnd{  0.0040} \\ 
			& Ps   
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR 
			&   41.32 & \Valbest{  49.20} & \ValSecnd{  43.39} &   41.70 
			&   38.29 & \Valbest{  39.00} &   38.35 & \ValSecnd{  38.51} 
			&   40.18 & \Valbest{  52.34} &   40.45 & \ValSecnd{  42.56} \\ 
			& MSSIM 
			&   0.9530 & \Valbest{  0.9959} & \ValSecnd{  0.9735} &   0.9572 
			&   0.9726 & \Valbest{  0.9787} &   0.9731 & \ValSecnd{  0.9743} 
			&   0.9321 & \Valbest{  0.9991} &   0.9361 & \ValSecnd{  0.9624} \\ 
			\cmidrule(lr){1-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			
			\multirow{6}{*}{Case 3} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			& \ValSecnd{  23.75} & \Valbest{  23.92} &   21.06 &   23.73 
			&   20.53 & \Valbest{  20.80} &   20.46 & \ValSecnd{  20.71} 
			&   26.33 & \Valbest{  29.66} &   25.91 & \ValSecnd{  26.93} \\ 
			& RMSE 
			& \ValSecnd{  0.0162} & \Valbest{  0.0159} &   0.0218 & \ValSecnd{  0.0162} 
			&   0.0211 & \Valbest{  0.0204} &   0.0213 & \ValSecnd{  0.0207} 
			&   0.0026 & \Valbest{  0.0018} &   0.0028 & \ValSecnd{  0.0025} \\ 
			& Ps   
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR 
			&   46.76 & \Valbest{  50.54} & \ValSecnd{  48.43} &   46.82 
			&   41.90 & \Valbest{  42.24} &   41.90 & \ValSecnd{  42.06} 
			&   45.07 & \Valbest{  55.27} &   45.23 & \ValSecnd{  47.14} \\ 
			& MSSIM 
			&   0.9858 & \Valbest{  0.9949} & \ValSecnd{  0.9922} &   0.9860 
			&   0.9883 & \Valbest{  0.9902} &   0.9883 & \ValSecnd{  0.9889} 
			&   0.9761 & \Valbest{  0.9996} &   0.9783 & \ValSecnd{  0.9870} \\ 
			\cmidrule(lr){1-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			
			\multirow{6}{*}{Case 4} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			&   23.27 & \Valbest{  23.59} &   21.89 & \ValSecnd{  23.31} 
			&   18.62 & \Valbest{  19.02} &   18.65 & \ValSecnd{  18.92} 
			&   25.52 & \Valbest{  30.92} &   25.52 & \ValSecnd{  26.68} \\ 
			& RMSE 
			& \ValSecnd{  0.0172} & \Valbest{  0.0166} &   0.0199 & \ValSecnd{  0.0172} 
			&   0.0263 & \Valbest{  0.0251} &   0.0262 & \ValSecnd{  0.0254} 
			&   0.0029 & \Valbest{  0.0016} &   0.0029 & \ValSecnd{  0.0025} \\ 
			& Ps   
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR 
			&   45.24 & \Valbest{  47.92} & \ValSecnd{  47.58} &   45.63 
			&   40.78 & \Valbest{  41.30} &   40.80 & \ValSecnd{  40.97} 
			&   43.65 & \Valbest{  55.21} &   44.34 & \ValSecnd{  45.62} \\ 
			& MSSIM 
			&   0.9790 & \ValSecnd{  0.9893} & \Valbest{  0.9900} &   0.9810 
			&   0.9843 & \Valbest{  0.9871} &   0.9844 & \ValSecnd{  0.9852} 
			&   0.9665 & \Valbest{  0.9996} &   0.9730 & \ValSecnd{  0.9803} \\ 
			\cmidrule(lr){1-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			
			\multirow{6}{*}{Case 5} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			&   19.96 & \Valbest{  21.38} & \ValSecnd{  21.02} &   19.96 
			&   21.30 & \Valbest{  21.52} &   21.27 & \ValSecnd{  21.42} 
			&   21.22 & \Valbest{  24.96} &   21.46 & \ValSecnd{  21.54} \\ 
			& RMSE 
			&   0.0244 & \Valbest{  0.0211} & \ValSecnd{  0.0218} &   0.0244 
			&   0.0194 & \Valbest{  0.0189} &   0.0195 & \ValSecnd{  0.0191} 
			&   0.0047 & \Valbest{  0.0031} &   0.0046 & \ValSecnd{  0.0045} \\ 
			& Ps   
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR 
			&   45.97 & \Valbest{  50.17} &   45.92 & \ValSecnd{  45.99} 
			&   42.48 & \Valbest{  42.83} &   42.51 & \ValSecnd{  42.65} 
			&   40.99 & \Valbest{  47.52} &   41.18 & \ValSecnd{  41.51} \\ 
			& MSSIM 
			& \ValSecnd{  0.9893} & \Valbest{  0.9983} &   0.9886 & \ValSecnd{  0.9893} 
			&   0.9890 & \Valbest{  0.9909} &   0.9890 & \ValSecnd{  0.9895} 
			&   0.9484 & \Valbest{  0.9980} &   0.9507 & \ValSecnd{  0.9550} \\ 
			\cmidrule(lr){1-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			
			\multirow{6}{*}{Case 6} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			&   16.28 & \Valbest{  17.14} &   14.86 & \ValSecnd{  16.80} 
			& \ValSecnd{  17.82} & \Valbest{  17.96} &   17.55 &   17.81 
			&   19.98 & \Valbest{  24.39} & \ValSecnd{  20.38} &   20.36 \\ 
			& RMSE 
			&   0.0374 & \Valbest{  0.0339} &   0.0425 & \ValSecnd{  0.0350} 
			& \ValSecnd{  0.0288} & \Valbest{  0.0282} &   0.0296 & \ValSecnd{  0.0288} 
			&   0.0054 & \Valbest{  0.0033} & \ValSecnd{  0.0051} & \ValSecnd{  0.0051} \\ 
			& Ps   
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR 
			&   38.88 &   41.22 & \Valbest{  42.52} & \ValSecnd{  42.03} 
			&   38.21 & \Valbest{  38.55} &   38.14 & \ValSecnd{  38.24} 
			&   37.98 & \Valbest{  47.02} &   38.23 & \ValSecnd{  38.86} \\ 
			& MSSIM 
			&   0.9229 &   0.9560 & \Valbest{  0.9741} & \ValSecnd{  0.9660} 
			&   0.9729 & \Valbest{  0.9798} &   0.9724 & \ValSecnd{  0.9732} 
			&   0.8974 & \Valbest{  0.9956} &   0.9029 & \ValSecnd{  0.9176} \\ 
			\cmidrule(lr){1-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			
			\multirow{6}{*}{Case 7} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			&   17.47 & \Valbest{  17.90} &   16.66 & \ValSecnd{  17.48} 
			&   15.89 & \ValSecnd{  15.95} &   15.68 & \Valbest{  16.05} 
			&   19.53 & \Valbest{  25.57} & \ValSecnd{  20.01} &   20.00 \\ 
			& RMSE 
			& \ValSecnd{  0.0323} & \Valbest{  0.0307} &   0.0351 & \ValSecnd{  0.0323} 
			&   0.0356 & \ValSecnd{  0.0353} &   0.0362 & \Valbest{  0.0348} 
			&   0.0056 & \Valbest{  0.0029} & \ValSecnd{  0.0054} & \ValSecnd{  0.0054} \\ 
			& Ps   
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR 
			&   39.68 & \Valbest{  47.34} &   39.58 & \ValSecnd{  39.78} 
			&   35.80 & \ValSecnd{  35.97} &   35.77 & \Valbest{  36.11} 
			&   36.85 & \Valbest{  48.64} &   37.09 & \ValSecnd{  38.06} \\ 
			& MSSIM 
			&   0.9392 & \Valbest{  0.9957} &   0.9378 & \ValSecnd{  0.9406} 
			&   0.9533 & \ValSecnd{  0.9553} &   0.9531 & \Valbest{  0.9570} 
			&   0.8653 & \Valbest{  0.9969} &   0.8716 & \ValSecnd{  0.8980} \\ 
			\cmidrule(lr){1-2}\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}
			
			\multirow{6}{*}{Case 8} 
			& Setup 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.95$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-2}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} 
			& \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} & \begin{tabular}{c} \hspace{-4mm} $\lambda_{1} = 10^{0}$, \hspace{-4mm} \\\hspace{-4mm} $\lambda_{2} = 10^{-1}$, \hspace{-4mm} \\\hspace{-4mm} $\varepsilon = 0.98$ \hspace{-4mm}\end{tabular} \\ 
			& SRE  
			&   13.84 & \Valbest{  14.96} &   11.89 & \ValSecnd{  14.08} 
			& \ValSecnd{  14.63} & \Valbest{  14.67} &   14.26 &   14.60 
			&   18.29 & \Valbest{  21.12} &   18.67 & \ValSecnd{  18.69} \\ 
			& RMSE 
			&   0.0485 & \Valbest{  0.0427} &   0.0592 & \ValSecnd{  0.0468} 
			& \ValSecnd{  0.0403} & \Valbest{  0.0401} &   0.0415 &   0.0405 
			&   0.0064 & \Valbest{  0.0047} & \ValSecnd{  0.0062} & \ValSecnd{  0.0062} \\ 
			& Ps   
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} 
			& \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} & \Valbest{  0.99} 
			& \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} & \Valbest{  1.00} \\ 
			& MPSNR 
			&   36.73 & \ValSecnd{  40.36} &   37.76 & \Valbest{  41.30} 
			&   35.17 & \Valbest{  35.40} &   35.12 & \ValSecnd{  35.21} 
			&   35.34 & \Valbest{  43.66} &   35.56 & \ValSecnd{  36.44} \\ 
			& MSSIM 
			&   0.8846 & \ValSecnd{  0.9518} &   0.9118 & \Valbest{  0.9653} 
			&   0.9519 & \Valbest{  0.9556} &   0.9517 & \ValSecnd{  0.9525} 
			&   0.8303 & \Valbest{  0.9925} &   0.8375 & \ValSecnd{  0.8696} \\ 
			
			\bottomrule
		\end{tabular}
	}
\end{table*}



==> tab_tex/tab_results_times_colored.tex <==
\begin{table}[t]
	\color{blue}
	\caption{Averages of Running Times [s] in All Noise Cases for Each Dataset.}
	\vspace{-1mm}
	\label{tab:results_times}
	\centering
	\begin{tabular}{cccc}
		\toprule
		Methods &  \textit{Jasper Ridge} & \textit{Samson} & \textit{Urban} \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-4}
		CLSUnSAL~\cite{iordache2014collaborative} & $1.359*10^{0}$ & $9.739*10^{-1}$ & $9.192*10^{1}$ \\ 
		\vspace{0.5mm}
		JSTV~\cite{aggarwal2016hyperspectral} & $7.776*10^{1}$ & $7.787*10^{1}$ & $5.709*10^{2}$ \\ 
		\vspace{0.5mm}
		RSSUn-TV~\cite{wang2019row} & $1.870*10^{0}$ & $1.615*10^{0}$ & $1.111*10^{2}$ \\ 
		\vspace{0.5mm}
		LGSU~\cite{shen2022superpixel} & $2.165*10^{1}$ & $1.720*10^{1}$ & $6.655*10^{2}$ \\ 
		\vspace{0.5mm}
		UnDIP~\cite{UnDIP_RastiB_2022} & $1.436*10^{2}$ & $1.030*10^{2}$ & $2.349*10^{3}$ \\ 
		\vspace{0.5mm}
		EGU-Net~\cite{hong2022endmember} & $1.669*10^{1}$ & $1.420*10^{1}$ & $2.360*10^{2}$ \\ 
		\vspace{0.5mm}
		RDSWSU~\cite{rs_Deng_RobustDual_2023} & $1.239*10^{1}$ & $9.790*10^{0}$ & $4.633*10^{2}$ \\ 
		\vspace{0.5mm}
		MdLRR~\cite{MDLRR_WuLing_2023} & $7.268*10^{0}$ & $6.592*10^{0}$ & $4.776*10^{2}$ \\ 
		\vspace{0.5mm}
		\textbf{\Ours (HTV)} & $2.252*10^{1}$ & $4.674*10^{1}$ & $5.768*10^{2}$ \\ 
		\vspace{0.5mm}
		\textbf{\Ours (SSTV)} & $2.822*10^{1}$ & $5.372*10^{1}$ & $8.269*10^{2}$ \\ 
		\vspace{0.5mm}
		\textbf{\Ours (HSSTV)} & $2.440*10^{1}$ & $5.141*10^{1}$ & $8.265*10^{2}$ \\ 
		\bottomrule
	\end{tabular}
\end{table}


